Search for top squarks decaying to tau sleptons in $pp$ collisions at $\sqrt{s}= 13$ TeV with the ATLAS detector

A search for direct pair production of top squarks in final states with two tau leptons, $b$-jets, and missing transverse momentum is presented. The analysis is based on proton-proton collision data at $\sqrt{s} = 13$ TeV corresponding to an integrated luminosity of 36.1 fb$^{-1}$ recorded with the ATLAS detector at the Large Hadron Collider in 2015 and 2016. Two exclusive channels with either two hadronically decaying tau leptons or one hadronically and one leptonically decaying tau lepton are considered. No significant deviation from the Standard Model predictions is observed in the data. The analysis results are interpreted in terms of model-independent limits and used to derive exclusion limits on the masses of the top squark $\tilde t_1$ and the tau slepton $\tilde \tau_1$ in a simplified model of supersymmetry with a nearly massless gravitino. In this model, masses up to $m(\tilde t_1) = 1.16$ TeV and $m(\tilde \tau_1) = 1.00$ TeV are excluded at 95% confidence level.

==> atlas_authlist.tex <==
% ATLAS Collaboration author list
% Reference date of SUSY-2016-19 is 2017-11-02
% Author list last updated on date 04-SEP-18
% Data extracted on 04-Sep-2018 for paper reference SUSY-2016-19
% at 4:39pm
 
\begin{flushleft}
{\Large The ATLAS Collaboration}

\bigskip

M.~Aaboud$^\textrm{\scriptsize 34d}$,    
G.~Aad$^\textrm{\scriptsize 99}$,    
B.~Abbott$^\textrm{\scriptsize 124}$,    
O.~Abdinov$^\textrm{\scriptsize 13,*}$,    
B.~Abeloos$^\textrm{\scriptsize 128}$,    
S.H.~Abidi$^\textrm{\scriptsize 165}$,    
O.S.~AbouZeid$^\textrm{\scriptsize 143}$,    
N.L.~Abraham$^\textrm{\scriptsize 153}$,    
H.~Abramowicz$^\textrm{\scriptsize 159}$,    
H.~Abreu$^\textrm{\scriptsize 158}$,    
Y.~Abulaiti$^\textrm{\scriptsize 6}$,    
B.S.~Acharya$^\textrm{\scriptsize 64a,64b,p}$,    
S.~Adachi$^\textrm{\scriptsize 161}$,    
L.~Adamczyk$^\textrm{\scriptsize 81a}$,    
J.~Adelman$^\textrm{\scriptsize 119}$,    
M.~Adersberger$^\textrm{\scriptsize 112}$,    
T.~Adye$^\textrm{\scriptsize 141}$,    
A.A.~Affolder$^\textrm{\scriptsize 143}$,    
Y.~Afik$^\textrm{\scriptsize 158}$,    
C.~Agheorghiesei$^\textrm{\scriptsize 27c}$,    
J.A.~Aguilar-Saavedra$^\textrm{\scriptsize 136f,136a}$,    
F.~Ahmadov$^\textrm{\scriptsize 77,ai}$,    
G.~Aielli$^\textrm{\scriptsize 71a,71b}$,    
S.~Akatsuka$^\textrm{\scriptsize 83}$,    
T.P.A.~{\AA}kesson$^\textrm{\scriptsize 94}$,    
E.~Akilli$^\textrm{\scriptsize 52}$,    
A.V.~Akimov$^\textrm{\scriptsize 108}$,    
G.L.~Alberghi$^\textrm{\scriptsize 23b,23a}$,    
J.~Albert$^\textrm{\scriptsize 174}$,    
P.~Albicocco$^\textrm{\scriptsize 49}$,    
M.J.~Alconada~Verzini$^\textrm{\scriptsize 86}$,    
S.~Alderweireldt$^\textrm{\scriptsize 117}$,    
M.~Aleksa$^\textrm{\scriptsize 35}$,    
I.N.~Aleksandrov$^\textrm{\scriptsize 77}$,    
C.~Alexa$^\textrm{\scriptsize 27b}$,    
G.~Alexander$^\textrm{\scriptsize 159}$,    
T.~Alexopoulos$^\textrm{\scriptsize 10}$,    
M.~Alhroob$^\textrm{\scriptsize 124}$,    
B.~Ali$^\textrm{\scriptsize 138}$,    
G.~Alimonti$^\textrm{\scriptsize 66a}$,    
J.~Alison$^\textrm{\scriptsize 36}$,    
S.P.~Alkire$^\textrm{\scriptsize 145}$,    
C.~Allaire$^\textrm{\scriptsize 128}$,    
B.M.M.~Allbrooke$^\textrm{\scriptsize 153}$,    
B.W.~Allen$^\textrm{\scriptsize 127}$,    
P.P.~Allport$^\textrm{\scriptsize 21}$,    
A.~Aloisio$^\textrm{\scriptsize 67a,67b}$,    
A.~Alonso$^\textrm{\scriptsize 39}$,    
F.~Alonso$^\textrm{\scriptsize 86}$,    
C.~Alpigiani$^\textrm{\scriptsize 145}$,    
A.A.~Alshehri$^\textrm{\scriptsize 55}$,    
M.I.~Alstaty$^\textrm{\scriptsize 99}$,    
B.~Alvarez~Gonzalez$^\textrm{\scriptsize 35}$,    
D.~\'{A}lvarez~Piqueras$^\textrm{\scriptsize 172}$,    
M.G.~Alviggi$^\textrm{\scriptsize 67a,67b}$,    
B.T.~Amadio$^\textrm{\scriptsize 18}$,    
Y.~Amaral~Coutinho$^\textrm{\scriptsize 78b}$,    
L.~Ambroz$^\textrm{\scriptsize 131}$,    
C.~Amelung$^\textrm{\scriptsize 26}$,    
D.~Amidei$^\textrm{\scriptsize 103}$,    
S.P.~Amor~Dos~Santos$^\textrm{\scriptsize 136a,136c}$,    
S.~Amoroso$^\textrm{\scriptsize 35}$,    
C.~Anastopoulos$^\textrm{\scriptsize 146}$,    
L.S.~Ancu$^\textrm{\scriptsize 52}$,    
N.~Andari$^\textrm{\scriptsize 21}$,    
T.~Andeen$^\textrm{\scriptsize 11}$,    
C.F.~Anders$^\textrm{\scriptsize 59b}$,    
J.K.~Anders$^\textrm{\scriptsize 20}$,    
K.J.~Anderson$^\textrm{\scriptsize 36}$,    
A.~Andreazza$^\textrm{\scriptsize 66a,66b}$,    
V.~Andrei$^\textrm{\scriptsize 59a}$,    
S.~Angelidakis$^\textrm{\scriptsize 37}$,    
I.~Angelozzi$^\textrm{\scriptsize 118}$,    
A.~Angerami$^\textrm{\scriptsize 38}$,    
A.V.~Anisenkov$^\textrm{\scriptsize 120b,120a}$,    
A.~Annovi$^\textrm{\scriptsize 69a}$,    
C.~Antel$^\textrm{\scriptsize 59a}$,    
M.T.~Anthony$^\textrm{\scriptsize 146}$,    
M.~Antonelli$^\textrm{\scriptsize 49}$,    
A.~Antonov$^\textrm{\scriptsize 110,*}$,    
D.J.A.~Antrim$^\textrm{\scriptsize 169}$,    
F.~Anulli$^\textrm{\scriptsize 70a}$,    
M.~Aoki$^\textrm{\scriptsize 79}$,    
L.~Aperio~Bella$^\textrm{\scriptsize 35}$,    
G.~Arabidze$^\textrm{\scriptsize 104}$,    
Y.~Arai$^\textrm{\scriptsize 79}$,    
J.P.~Araque$^\textrm{\scriptsize 136a}$,    
V.~Araujo~Ferraz$^\textrm{\scriptsize 78b}$,    
R.~Araujo~Pereira$^\textrm{\scriptsize 78b}$,    
A.T.H.~Arce$^\textrm{\scriptsize 47}$,    
R.E.~Ardell$^\textrm{\scriptsize 91}$,    
F.A.~Arduh$^\textrm{\scriptsize 86}$,    
J-F.~Arguin$^\textrm{\scriptsize 107}$,    
S.~Argyropoulos$^\textrm{\scriptsize 75}$,    
A.J.~Armbruster$^\textrm{\scriptsize 35}$,    
L.J.~Armitage$^\textrm{\scriptsize 90}$,    
O.~Arnaez$^\textrm{\scriptsize 165}$,    
H.~Arnold$^\textrm{\scriptsize 118}$,    
M.~Arratia$^\textrm{\scriptsize 31}$,    
O.~Arslan$^\textrm{\scriptsize 24}$,    
A.~Artamonov$^\textrm{\scriptsize 109,*}$,    
G.~Artoni$^\textrm{\scriptsize 131}$,    
S.~Artz$^\textrm{\scriptsize 97}$,    
S.~Asai$^\textrm{\scriptsize 161}$,    
N.~Asbah$^\textrm{\scriptsize 44}$,    
A.~Ashkenazi$^\textrm{\scriptsize 159}$,    
L.~Asquith$^\textrm{\scriptsize 153}$,    
K.~Assamagan$^\textrm{\scriptsize 29}$,    
R.~Astalos$^\textrm{\scriptsize 28a}$,    
R.J.~Atkin$^\textrm{\scriptsize 32a}$,    
M.~Atkinson$^\textrm{\scriptsize 171}$,    
N.B.~Atlay$^\textrm{\scriptsize 148}$,    
K.~Augsten$^\textrm{\scriptsize 138}$,    
G.~Avolio$^\textrm{\scriptsize 35}$,    
R.~Avramidou$^\textrm{\scriptsize 58a}$,    
B.~Axen$^\textrm{\scriptsize 18}$,    
M.K.~Ayoub$^\textrm{\scriptsize 15a}$,    
G.~Azuelos$^\textrm{\scriptsize 107,ax}$,    
A.E.~Baas$^\textrm{\scriptsize 59a}$,    
M.J.~Baca$^\textrm{\scriptsize 21}$,    
H.~Bachacou$^\textrm{\scriptsize 142}$,    
K.~Bachas$^\textrm{\scriptsize 65a,65b}$,    
M.~Backes$^\textrm{\scriptsize 131}$,    
P.~Bagnaia$^\textrm{\scriptsize 70a,70b}$,    
M.~Bahmani$^\textrm{\scriptsize 82}$,    
H.~Bahrasemani$^\textrm{\scriptsize 149}$,    
J.T.~Baines$^\textrm{\scriptsize 141}$,    
M.~Bajic$^\textrm{\scriptsize 39}$,    
O.K.~Baker$^\textrm{\scriptsize 181}$,    
P.J.~Bakker$^\textrm{\scriptsize 118}$,    
D.~Bakshi~Gupta$^\textrm{\scriptsize 93}$,    
E.M.~Baldin$^\textrm{\scriptsize 120b,120a}$,    
P.~Balek$^\textrm{\scriptsize 178}$,    
F.~Balli$^\textrm{\scriptsize 142}$,    
W.K.~Balunas$^\textrm{\scriptsize 133}$,    
E.~Banas$^\textrm{\scriptsize 82}$,    
A.~Bandyopadhyay$^\textrm{\scriptsize 24}$,    
S.~Banerjee$^\textrm{\scriptsize 179,l}$,    
A.A.E.~Bannoura$^\textrm{\scriptsize 180}$,    
L.~Barak$^\textrm{\scriptsize 159}$,    
W.M.~Barbe$^\textrm{\scriptsize 37}$,    
E.L.~Barberio$^\textrm{\scriptsize 102}$,    
D.~Barberis$^\textrm{\scriptsize 53b,53a}$,    
M.~Barbero$^\textrm{\scriptsize 99}$,    
T.~Barillari$^\textrm{\scriptsize 113}$,    
M-S.~Barisits$^\textrm{\scriptsize 74}$,    
J.~Barkeloo$^\textrm{\scriptsize 127}$,    
T.~Barklow$^\textrm{\scriptsize 150}$,    
N.~Barlow$^\textrm{\scriptsize 31}$,    
R.~Barnea$^\textrm{\scriptsize 158}$,    
S.L.~Barnes$^\textrm{\scriptsize 58c}$,    
B.M.~Barnett$^\textrm{\scriptsize 141}$,    
R.M.~Barnett$^\textrm{\scriptsize 18}$,    
Z.~Barnovska-Blenessy$^\textrm{\scriptsize 58a}$,    
A.~Baroncelli$^\textrm{\scriptsize 72a}$,    
G.~Barone$^\textrm{\scriptsize 26}$,    
A.J.~Barr$^\textrm{\scriptsize 131}$,    
L.~Barranco~Navarro$^\textrm{\scriptsize 172}$,    
F.~Barreiro$^\textrm{\scriptsize 96}$,    
J.~Barreiro~Guimar\~{a}es~da~Costa$^\textrm{\scriptsize 15a}$,    
R.~Bartoldus$^\textrm{\scriptsize 150}$,    
A.E.~Barton$^\textrm{\scriptsize 87}$,    
P.~Bartos$^\textrm{\scriptsize 28a}$,    
A.~Basalaev$^\textrm{\scriptsize 134}$,    
A.~Bassalat$^\textrm{\scriptsize 128}$,    
R.L.~Bates$^\textrm{\scriptsize 55}$,    
S.J.~Batista$^\textrm{\scriptsize 165}$,    
J.R.~Batley$^\textrm{\scriptsize 31}$,    
M.~Battaglia$^\textrm{\scriptsize 143}$,    
M.~Bauce$^\textrm{\scriptsize 70a,70b}$,    
F.~Bauer$^\textrm{\scriptsize 142}$,    
K.T.~Bauer$^\textrm{\scriptsize 169}$,    
H.S.~Bawa$^\textrm{\scriptsize 150,n}$,    
J.B.~Beacham$^\textrm{\scriptsize 122}$,    
M.D.~Beattie$^\textrm{\scriptsize 87}$,    
T.~Beau$^\textrm{\scriptsize 132}$,    
P.H.~Beauchemin$^\textrm{\scriptsize 168}$,    
P.~Bechtle$^\textrm{\scriptsize 24}$,    
H.C.~Beck$^\textrm{\scriptsize 51}$,    
H.P.~Beck$^\textrm{\scriptsize 20,t}$,    
K.~Becker$^\textrm{\scriptsize 131}$,    
M.~Becker$^\textrm{\scriptsize 97}$,    
C.~Becot$^\textrm{\scriptsize 121}$,    
A.~Beddall$^\textrm{\scriptsize 12d}$,    
A.J.~Beddall$^\textrm{\scriptsize 12a}$,    
V.A.~Bednyakov$^\textrm{\scriptsize 77}$,    
M.~Bedognetti$^\textrm{\scriptsize 118}$,    
C.P.~Bee$^\textrm{\scriptsize 152}$,    
T.A.~Beermann$^\textrm{\scriptsize 35}$,    
M.~Begalli$^\textrm{\scriptsize 78b}$,    
M.~Begel$^\textrm{\scriptsize 29}$,    
A.~Behera$^\textrm{\scriptsize 152}$,    
J.K.~Behr$^\textrm{\scriptsize 44}$,    
A.S.~Bell$^\textrm{\scriptsize 92}$,    
G.~Bella$^\textrm{\scriptsize 159}$,    
L.~Bellagamba$^\textrm{\scriptsize 23b}$,    
A.~Bellerive$^\textrm{\scriptsize 33}$,    
M.~Bellomo$^\textrm{\scriptsize 158}$,    
K.~Belotskiy$^\textrm{\scriptsize 110}$,    
N.L.~Belyaev$^\textrm{\scriptsize 110}$,    
O.~Benary$^\textrm{\scriptsize 159,*}$,    
D.~Benchekroun$^\textrm{\scriptsize 34a}$,    
M.~Bender$^\textrm{\scriptsize 112}$,    
N.~Benekos$^\textrm{\scriptsize 10}$,    
Y.~Benhammou$^\textrm{\scriptsize 159}$,    
E.~Benhar~Noccioli$^\textrm{\scriptsize 181}$,    
J.~Benitez$^\textrm{\scriptsize 75}$,    
D.P.~Benjamin$^\textrm{\scriptsize 47}$,    
M.~Benoit$^\textrm{\scriptsize 52}$,    
J.R.~Bensinger$^\textrm{\scriptsize 26}$,    
S.~Bentvelsen$^\textrm{\scriptsize 118}$,    
L.~Beresford$^\textrm{\scriptsize 131}$,    
M.~Beretta$^\textrm{\scriptsize 49}$,    
D.~Berge$^\textrm{\scriptsize 44}$,    
E.~Bergeaas~Kuutmann$^\textrm{\scriptsize 170}$,    
N.~Berger$^\textrm{\scriptsize 5}$,    
L.J.~Bergsten$^\textrm{\scriptsize 26}$,    
J.~Beringer$^\textrm{\scriptsize 18}$,    
S.~Berlendis$^\textrm{\scriptsize 56}$,    
N.R.~Bernard$^\textrm{\scriptsize 100}$,    
G.~Bernardi$^\textrm{\scriptsize 132}$,    
C.~Bernius$^\textrm{\scriptsize 150}$,    
F.U.~Bernlochner$^\textrm{\scriptsize 24}$,    
T.~Berry$^\textrm{\scriptsize 91}$,    
P.~Berta$^\textrm{\scriptsize 97}$,    
C.~Bertella$^\textrm{\scriptsize 15a}$,    
G.~Bertoli$^\textrm{\scriptsize 43a,43b}$,    
I.A.~Bertram$^\textrm{\scriptsize 87}$,    
C.~Bertsche$^\textrm{\scriptsize 44}$,    
G.J.~Besjes$^\textrm{\scriptsize 39}$,    
O.~Bessidskaia~Bylund$^\textrm{\scriptsize 43a,43b}$,    
M.~Bessner$^\textrm{\scriptsize 44}$,    
N.~Besson$^\textrm{\scriptsize 142}$,    
A.~Bethani$^\textrm{\scriptsize 98}$,    
S.~Bethke$^\textrm{\scriptsize 113}$,    
A.~Betti$^\textrm{\scriptsize 24}$,    
A.J.~Bevan$^\textrm{\scriptsize 90}$,    
J.~Beyer$^\textrm{\scriptsize 113}$,    
R.M.~Bianchi$^\textrm{\scriptsize 135}$,    
O.~Biebel$^\textrm{\scriptsize 112}$,    
D.~Biedermann$^\textrm{\scriptsize 19}$,    
R.~Bielski$^\textrm{\scriptsize 98}$,    
K.~Bierwagen$^\textrm{\scriptsize 97}$,    
N.V.~Biesuz$^\textrm{\scriptsize 69a,69b}$,    
M.~Biglietti$^\textrm{\scriptsize 72a}$,    
T.R.V.~Billoud$^\textrm{\scriptsize 107}$,    
M.~Bindi$^\textrm{\scriptsize 51}$,    
A.~Bingul$^\textrm{\scriptsize 12d}$,    
C.~Bini$^\textrm{\scriptsize 70a,70b}$,    
S.~Biondi$^\textrm{\scriptsize 23b,23a}$,    
T.~Bisanz$^\textrm{\scriptsize 51}$,    
C.~Bittrich$^\textrm{\scriptsize 46}$,    
D.M.~Bjergaard$^\textrm{\scriptsize 47}$,    
J.E.~Black$^\textrm{\scriptsize 150}$,    
K.M.~Black$^\textrm{\scriptsize 25}$,    
R.E.~Blair$^\textrm{\scriptsize 6}$,    
T.~Blazek$^\textrm{\scriptsize 28a}$,    
I.~Bloch$^\textrm{\scriptsize 44}$,    
C.~Blocker$^\textrm{\scriptsize 26}$,    
A.~Blue$^\textrm{\scriptsize 55}$,    
U.~Blumenschein$^\textrm{\scriptsize 90}$,    
Dr.~Blunier$^\textrm{\scriptsize 144a}$,    
G.J.~Bobbink$^\textrm{\scriptsize 118}$,    
V.S.~Bobrovnikov$^\textrm{\scriptsize 120b,120a}$,    
S.S.~Bocchetta$^\textrm{\scriptsize 94}$,    
A.~Bocci$^\textrm{\scriptsize 47}$,    
C.~Bock$^\textrm{\scriptsize 112}$,    
D.~Boerner$^\textrm{\scriptsize 180}$,    
D.~Bogavac$^\textrm{\scriptsize 112}$,    
A.G.~Bogdanchikov$^\textrm{\scriptsize 120b,120a}$,    
C.~Bohm$^\textrm{\scriptsize 43a}$,    
V.~Boisvert$^\textrm{\scriptsize 91}$,    
P.~Bokan$^\textrm{\scriptsize 170}$,    
T.~Bold$^\textrm{\scriptsize 81a}$,    
A.S.~Boldyrev$^\textrm{\scriptsize 111}$,    
A.E.~Bolz$^\textrm{\scriptsize 59b}$,    
M.~Bomben$^\textrm{\scriptsize 132}$,    
M.~Bona$^\textrm{\scriptsize 90}$,    
J.S.~Bonilla$^\textrm{\scriptsize 127}$,    
M.~Boonekamp$^\textrm{\scriptsize 142}$,    
A.~Borisov$^\textrm{\scriptsize 140}$,    
G.~Borissov$^\textrm{\scriptsize 87}$,    
J.~Bortfeldt$^\textrm{\scriptsize 35}$,    
D.~Bortoletto$^\textrm{\scriptsize 131}$,    
V.~Bortolotto$^\textrm{\scriptsize 61a,61b,61c}$,    
D.~Boscherini$^\textrm{\scriptsize 23b}$,    
M.~Bosman$^\textrm{\scriptsize 14}$,    
J.D.~Bossio~Sola$^\textrm{\scriptsize 30}$,    
J.~Boudreau$^\textrm{\scriptsize 135}$,    
E.V.~Bouhova-Thacker$^\textrm{\scriptsize 87}$,    
D.~Boumediene$^\textrm{\scriptsize 37}$,    
C.~Bourdarios$^\textrm{\scriptsize 128}$,    
S.K.~Boutle$^\textrm{\scriptsize 55}$,    
A.~Boveia$^\textrm{\scriptsize 122}$,    
J.~Boyd$^\textrm{\scriptsize 35}$,    
I.R.~Boyko$^\textrm{\scriptsize 77}$,    
A.J.~Bozson$^\textrm{\scriptsize 91}$,    
J.~Bracinik$^\textrm{\scriptsize 21}$,    
A.~Brandt$^\textrm{\scriptsize 8}$,    
G.~Brandt$^\textrm{\scriptsize 180}$,    
O.~Brandt$^\textrm{\scriptsize 59a}$,    
F.~Braren$^\textrm{\scriptsize 44}$,    
U.~Bratzler$^\textrm{\scriptsize 162}$,    
B.~Brau$^\textrm{\scriptsize 100}$,    
J.E.~Brau$^\textrm{\scriptsize 127}$,    
W.D.~Breaden~Madden$^\textrm{\scriptsize 55}$,    
K.~Brendlinger$^\textrm{\scriptsize 44}$,    
A.J.~Brennan$^\textrm{\scriptsize 102}$,    
L.~Brenner$^\textrm{\scriptsize 44}$,    
R.~Brenner$^\textrm{\scriptsize 170}$,    
S.~Bressler$^\textrm{\scriptsize 178}$,    
D.L.~Briglin$^\textrm{\scriptsize 21}$,    
T.M.~Bristow$^\textrm{\scriptsize 48}$,    
D.~Britton$^\textrm{\scriptsize 55}$,    
D.~Britzger$^\textrm{\scriptsize 59b}$,    
I.~Brock$^\textrm{\scriptsize 24}$,    
R.~Brock$^\textrm{\scriptsize 104}$,    
G.~Brooijmans$^\textrm{\scriptsize 38}$,    
T.~Brooks$^\textrm{\scriptsize 91}$,    
W.K.~Brooks$^\textrm{\scriptsize 144b}$,    
E.~Brost$^\textrm{\scriptsize 119}$,    
J.H~Broughton$^\textrm{\scriptsize 21}$,    
P.A.~Bruckman~de~Renstrom$^\textrm{\scriptsize 82}$,    
D.~Bruncko$^\textrm{\scriptsize 28b}$,    
A.~Bruni$^\textrm{\scriptsize 23b}$,    
G.~Bruni$^\textrm{\scriptsize 23b}$,    
L.S.~Bruni$^\textrm{\scriptsize 118}$,    
S.~Bruno$^\textrm{\scriptsize 71a,71b}$,    
B.H.~Brunt$^\textrm{\scriptsize 31}$,    
M.~Bruschi$^\textrm{\scriptsize 23b}$,    
N.~Bruscino$^\textrm{\scriptsize 135}$,    
P.~Bryant$^\textrm{\scriptsize 36}$,    
L.~Bryngemark$^\textrm{\scriptsize 44}$,    
T.~Buanes$^\textrm{\scriptsize 17}$,    
Q.~Buat$^\textrm{\scriptsize 35}$,    
P.~Buchholz$^\textrm{\scriptsize 148}$,    
A.G.~Buckley$^\textrm{\scriptsize 55}$,    
I.A.~Budagov$^\textrm{\scriptsize 77}$,    
M.K.~Bugge$^\textrm{\scriptsize 130}$,    
F.~B\"uhrer$^\textrm{\scriptsize 50}$,    
O.~Bulekov$^\textrm{\scriptsize 110}$,    
D.~Bullock$^\textrm{\scriptsize 8}$,    
T.J.~Burch$^\textrm{\scriptsize 119}$,    
S.~Burdin$^\textrm{\scriptsize 88}$,    
C.D.~Burgard$^\textrm{\scriptsize 118}$,    
A.M.~Burger$^\textrm{\scriptsize 5}$,    
B.~Burghgrave$^\textrm{\scriptsize 119}$,    
K.~Burka$^\textrm{\scriptsize 82}$,    
S.~Burke$^\textrm{\scriptsize 141}$,    
I.~Burmeister$^\textrm{\scriptsize 45}$,    
J.T.P.~Burr$^\textrm{\scriptsize 131}$,    
D.~B\"uscher$^\textrm{\scriptsize 50}$,    
V.~B\"uscher$^\textrm{\scriptsize 97}$,    
E.~Buschmann$^\textrm{\scriptsize 51}$,    
P.~Bussey$^\textrm{\scriptsize 55}$,    
J.M.~Butler$^\textrm{\scriptsize 25}$,    
C.M.~Buttar$^\textrm{\scriptsize 55}$,    
J.M.~Butterworth$^\textrm{\scriptsize 92}$,    
P.~Butti$^\textrm{\scriptsize 35}$,    
W.~Buttinger$^\textrm{\scriptsize 35}$,    
A.~Buzatu$^\textrm{\scriptsize 155}$,    
A.R.~Buzykaev$^\textrm{\scriptsize 120b,120a}$,    
G.~Cabras$^\textrm{\scriptsize 23b,23a}$,    
S.~Cabrera~Urb\'an$^\textrm{\scriptsize 172}$,    
D.~Caforio$^\textrm{\scriptsize 138}$,    
H.~Cai$^\textrm{\scriptsize 171}$,    
V.M.M.~Cairo$^\textrm{\scriptsize 2}$,    
O.~Cakir$^\textrm{\scriptsize 4a}$,    
N.~Calace$^\textrm{\scriptsize 52}$,    
P.~Calafiura$^\textrm{\scriptsize 18}$,    
A.~Calandri$^\textrm{\scriptsize 99}$,    
G.~Calderini$^\textrm{\scriptsize 132}$,    
P.~Calfayan$^\textrm{\scriptsize 63}$,    
G.~Callea$^\textrm{\scriptsize 40b,40a}$,    
L.P.~Caloba$^\textrm{\scriptsize 78b}$,    
S.~Calvente~Lopez$^\textrm{\scriptsize 96}$,    
D.~Calvet$^\textrm{\scriptsize 37}$,    
S.~Calvet$^\textrm{\scriptsize 37}$,    
T.P.~Calvet$^\textrm{\scriptsize 152}$,    
M.~Calvetti$^\textrm{\scriptsize 69a,69b}$,    
R.~Camacho~Toro$^\textrm{\scriptsize 36}$,    
S.~Camarda$^\textrm{\scriptsize 35}$,    
P.~Camarri$^\textrm{\scriptsize 71a,71b}$,    
D.~Cameron$^\textrm{\scriptsize 130}$,    
R.~Caminal~Armadans$^\textrm{\scriptsize 100}$,    
C.~Camincher$^\textrm{\scriptsize 56}$,    
S.~Campana$^\textrm{\scriptsize 35}$,    
M.~Campanelli$^\textrm{\scriptsize 92}$,    
A.~Camplani$^\textrm{\scriptsize 66a,66b}$,    
A.~Campoverde$^\textrm{\scriptsize 148}$,    
V.~Canale$^\textrm{\scriptsize 67a,67b}$,    
M.~Cano~Bret$^\textrm{\scriptsize 58c}$,    
J.~Cantero$^\textrm{\scriptsize 125}$,    
T.~Cao$^\textrm{\scriptsize 159}$,    
Y.~Cao$^\textrm{\scriptsize 171}$,    
M.D.M.~Capeans~Garrido$^\textrm{\scriptsize 35}$,    
I.~Caprini$^\textrm{\scriptsize 27b}$,    
M.~Caprini$^\textrm{\scriptsize 27b}$,    
M.~Capua$^\textrm{\scriptsize 40b,40a}$,    
R.M.~Carbone$^\textrm{\scriptsize 38}$,    
R.~Cardarelli$^\textrm{\scriptsize 71a}$,    
F.C.~Cardillo$^\textrm{\scriptsize 50}$,    
I.~Carli$^\textrm{\scriptsize 139}$,    
T.~Carli$^\textrm{\scriptsize 35}$,    
G.~Carlino$^\textrm{\scriptsize 67a}$,    
B.T.~Carlson$^\textrm{\scriptsize 135}$,    
L.~Carminati$^\textrm{\scriptsize 66a,66b}$,    
R.M.D.~Carney$^\textrm{\scriptsize 43a,43b}$,    
S.~Caron$^\textrm{\scriptsize 117}$,    
E.~Carquin$^\textrm{\scriptsize 144b}$,    
S.~Carr\'a$^\textrm{\scriptsize 66a,66b}$,    
G.D.~Carrillo-Montoya$^\textrm{\scriptsize 35}$,    
D.~Casadei$^\textrm{\scriptsize 21}$,    
M.P.~Casado$^\textrm{\scriptsize 14,h}$,    
A.F.~Casha$^\textrm{\scriptsize 165}$,    
M.~Casolino$^\textrm{\scriptsize 14}$,    
D.W.~Casper$^\textrm{\scriptsize 169}$,    
R.~Castelijn$^\textrm{\scriptsize 118}$,    
V.~Castillo~Gimenez$^\textrm{\scriptsize 172}$,    
N.F.~Castro$^\textrm{\scriptsize 136a,136e}$,    
A.~Catinaccio$^\textrm{\scriptsize 35}$,    
J.R.~Catmore$^\textrm{\scriptsize 130}$,    
A.~Cattai$^\textrm{\scriptsize 35}$,    
J.~Caudron$^\textrm{\scriptsize 24}$,    
V.~Cavaliere$^\textrm{\scriptsize 29}$,    
E.~Cavallaro$^\textrm{\scriptsize 14}$,    
D.~Cavalli$^\textrm{\scriptsize 66a}$,    
M.~Cavalli-Sforza$^\textrm{\scriptsize 14}$,    
V.~Cavasinni$^\textrm{\scriptsize 69a,69b}$,    
E.~Celebi$^\textrm{\scriptsize 12b}$,    
F.~Ceradini$^\textrm{\scriptsize 72a,72b}$,    
L.~Cerda~Alberich$^\textrm{\scriptsize 172}$,    
A.S.~Cerqueira$^\textrm{\scriptsize 78a}$,    
A.~Cerri$^\textrm{\scriptsize 153}$,    
L.~Cerrito$^\textrm{\scriptsize 71a,71b}$,    
F.~Cerutti$^\textrm{\scriptsize 18}$,    
A.~Cervelli$^\textrm{\scriptsize 23b,23a}$,    
S.A.~Cetin$^\textrm{\scriptsize 12b}$,    
A.~Chafaq$^\textrm{\scriptsize 34a}$,    
D~Chakraborty$^\textrm{\scriptsize 119}$,    
S.K.~Chan$^\textrm{\scriptsize 57}$,    
W.S.~Chan$^\textrm{\scriptsize 118}$,    
Y.L.~Chan$^\textrm{\scriptsize 61a}$,    
P.~Chang$^\textrm{\scriptsize 171}$,    
J.D.~Chapman$^\textrm{\scriptsize 31}$,    
D.G.~Charlton$^\textrm{\scriptsize 21}$,    
C.C.~Chau$^\textrm{\scriptsize 33}$,    
C.A.~Chavez~Barajas$^\textrm{\scriptsize 153}$,    
S.~Che$^\textrm{\scriptsize 122}$,    
A.~Chegwidden$^\textrm{\scriptsize 104}$,    
S.~Chekanov$^\textrm{\scriptsize 6}$,    
S.V.~Chekulaev$^\textrm{\scriptsize 166a}$,    
G.A.~Chelkov$^\textrm{\scriptsize 77,aw}$,    
M.A.~Chelstowska$^\textrm{\scriptsize 35}$,    
C.~Chen$^\textrm{\scriptsize 58a}$,    
C.H.~Chen$^\textrm{\scriptsize 76}$,    
H.~Chen$^\textrm{\scriptsize 29}$,    
J.~Chen$^\textrm{\scriptsize 58a}$,    
J.~Chen$^\textrm{\scriptsize 38}$,    
S.~Chen$^\textrm{\scriptsize 133}$,    
S.J.~Chen$^\textrm{\scriptsize 15c}$,    
X.~Chen$^\textrm{\scriptsize 15b,av}$,    
Y.~Chen$^\textrm{\scriptsize 80}$,    
Y-H.~Chen$^\textrm{\scriptsize 44}$,    
H.C.~Cheng$^\textrm{\scriptsize 103}$,    
H.J.~Cheng$^\textrm{\scriptsize 15d}$,    
A.~Cheplakov$^\textrm{\scriptsize 77}$,    
E.~Cheremushkina$^\textrm{\scriptsize 140}$,    
R.~Cherkaoui~El~Moursli$^\textrm{\scriptsize 34e}$,    
E.~Cheu$^\textrm{\scriptsize 7}$,    
K.~Cheung$^\textrm{\scriptsize 62}$,    
L.~Chevalier$^\textrm{\scriptsize 142}$,    
V.~Chiarella$^\textrm{\scriptsize 49}$,    
G.~Chiarelli$^\textrm{\scriptsize 69a}$,    
G.~Chiodini$^\textrm{\scriptsize 65a}$,    
A.S.~Chisholm$^\textrm{\scriptsize 35}$,    
A.~Chitan$^\textrm{\scriptsize 27b}$,    
I.~Chiu$^\textrm{\scriptsize 161}$,    
Y.H.~Chiu$^\textrm{\scriptsize 174}$,    
M.V.~Chizhov$^\textrm{\scriptsize 77}$,    
K.~Choi$^\textrm{\scriptsize 63}$,    
A.R.~Chomont$^\textrm{\scriptsize 37}$,    
S.~Chouridou$^\textrm{\scriptsize 160}$,    
Y.S.~Chow$^\textrm{\scriptsize 118}$,    
V.~Christodoulou$^\textrm{\scriptsize 92}$,    
M.C.~Chu$^\textrm{\scriptsize 61a}$,    
J.~Chudoba$^\textrm{\scriptsize 137}$,    
A.J.~Chuinard$^\textrm{\scriptsize 101}$,    
J.J.~Chwastowski$^\textrm{\scriptsize 82}$,    
L.~Chytka$^\textrm{\scriptsize 126}$,    
D.~Cinca$^\textrm{\scriptsize 45}$,    
V.~Cindro$^\textrm{\scriptsize 89}$,    
I.A.~Cioar\u{a}$^\textrm{\scriptsize 24}$,    
A.~Ciocio$^\textrm{\scriptsize 18}$,    
F.~Cirotto$^\textrm{\scriptsize 67a,67b}$,    
Z.H.~Citron$^\textrm{\scriptsize 178}$,    
M.~Citterio$^\textrm{\scriptsize 66a}$,    
A.~Clark$^\textrm{\scriptsize 52}$,    
M.R.~Clark$^\textrm{\scriptsize 38}$,    
P.J.~Clark$^\textrm{\scriptsize 48}$,    
R.N.~Clarke$^\textrm{\scriptsize 18}$,    
C.~Clement$^\textrm{\scriptsize 43a,43b}$,    
Y.~Coadou$^\textrm{\scriptsize 99}$,    
M.~Cobal$^\textrm{\scriptsize 64a,64c}$,    
A.~Coccaro$^\textrm{\scriptsize 53b,53a}$,    
J.~Cochran$^\textrm{\scriptsize 76}$,    
L.~Colasurdo$^\textrm{\scriptsize 117}$,    
B.~Cole$^\textrm{\scriptsize 38}$,    
A.P.~Colijn$^\textrm{\scriptsize 118}$,    
J.~Collot$^\textrm{\scriptsize 56}$,    
P.~Conde~Mui\~no$^\textrm{\scriptsize 136a,136b}$,    
E.~Coniavitis$^\textrm{\scriptsize 50}$,    
S.H.~Connell$^\textrm{\scriptsize 32b}$,    
I.A.~Connelly$^\textrm{\scriptsize 98}$,    
S.~Constantinescu$^\textrm{\scriptsize 27b}$,    
G.~Conti$^\textrm{\scriptsize 35}$,    
F.~Conventi$^\textrm{\scriptsize 67a,ay}$,    
A.M.~Cooper-Sarkar$^\textrm{\scriptsize 131}$,    
F.~Cormier$^\textrm{\scriptsize 173}$,    
K.J.R.~Cormier$^\textrm{\scriptsize 165}$,    
M.~Corradi$^\textrm{\scriptsize 70a,70b}$,    
E.E.~Corrigan$^\textrm{\scriptsize 94}$,    
F.~Corriveau$^\textrm{\scriptsize 101,ag}$,    
A.~Cortes-Gonzalez$^\textrm{\scriptsize 35}$,    
M.J.~Costa$^\textrm{\scriptsize 172}$,    
D.~Costanzo$^\textrm{\scriptsize 146}$,    
G.~Cottin$^\textrm{\scriptsize 31}$,    
G.~Cowan$^\textrm{\scriptsize 91}$,    
B.E.~Cox$^\textrm{\scriptsize 98}$,    
J.~Crane$^\textrm{\scriptsize 98}$,    
K.~Cranmer$^\textrm{\scriptsize 121}$,    
S.J.~Crawley$^\textrm{\scriptsize 55}$,    
R.A.~Creager$^\textrm{\scriptsize 133}$,    
G.~Cree$^\textrm{\scriptsize 33}$,    
S.~Cr\'ep\'e-Renaudin$^\textrm{\scriptsize 56}$,    
F.~Crescioli$^\textrm{\scriptsize 132}$,    
M.~Cristinziani$^\textrm{\scriptsize 24}$,    
V.~Croft$^\textrm{\scriptsize 121}$,    
G.~Crosetti$^\textrm{\scriptsize 40b,40a}$,    
A.~Cueto$^\textrm{\scriptsize 96}$,    
T.~Cuhadar~Donszelmann$^\textrm{\scriptsize 146}$,    
A.R.~Cukierman$^\textrm{\scriptsize 150}$,    
M.~Curatolo$^\textrm{\scriptsize 49}$,    
J.~C\'uth$^\textrm{\scriptsize 97}$,    
S.~Czekierda$^\textrm{\scriptsize 82}$,    
P.~Czodrowski$^\textrm{\scriptsize 35}$,    
M.J.~Da~Cunha~Sargedas~De~Sousa$^\textrm{\scriptsize 136a,136b}$,    
C.~Da~Via$^\textrm{\scriptsize 98}$,    
W.~Dabrowski$^\textrm{\scriptsize 81a}$,    
T.~Dado$^\textrm{\scriptsize 28a,aa}$,    
S.~Dahbi$^\textrm{\scriptsize 34e}$,    
T.~Dai$^\textrm{\scriptsize 103}$,    
O.~Dale$^\textrm{\scriptsize 17}$,    
F.~Dallaire$^\textrm{\scriptsize 107}$,    
C.~Dallapiccola$^\textrm{\scriptsize 100}$,    
M.~Dam$^\textrm{\scriptsize 39}$,    
G.~D'amen$^\textrm{\scriptsize 23b,23a}$,    
J.R.~Dandoy$^\textrm{\scriptsize 133}$,    
M.F.~Daneri$^\textrm{\scriptsize 30}$,    
N.P.~Dang$^\textrm{\scriptsize 179,l}$,    
N.D~Dann$^\textrm{\scriptsize 98}$,    
M.~Danninger$^\textrm{\scriptsize 173}$,    
M.~Dano~Hoffmann$^\textrm{\scriptsize 142}$,    
V.~Dao$^\textrm{\scriptsize 35}$,    
G.~Darbo$^\textrm{\scriptsize 53b}$,    
S.~Darmora$^\textrm{\scriptsize 8}$,    
O.~Dartsi$^\textrm{\scriptsize 5}$,    
A.~Dattagupta$^\textrm{\scriptsize 127}$,    
T.~Daubney$^\textrm{\scriptsize 44}$,    
S.~D'Auria$^\textrm{\scriptsize 55}$,    
W.~Davey$^\textrm{\scriptsize 24}$,    
C.~David$^\textrm{\scriptsize 44}$,    
T.~Davidek$^\textrm{\scriptsize 139}$,    
D.R.~Davis$^\textrm{\scriptsize 47}$,    
E.~Dawe$^\textrm{\scriptsize 102}$,    
I.~Dawson$^\textrm{\scriptsize 146}$,    
K.~De$^\textrm{\scriptsize 8}$,    
R.~De~Asmundis$^\textrm{\scriptsize 67a}$,    
A.~De~Benedetti$^\textrm{\scriptsize 124}$,    
S.~De~Castro$^\textrm{\scriptsize 23b,23a}$,    
S.~De~Cecco$^\textrm{\scriptsize 132}$,    
N.~De~Groot$^\textrm{\scriptsize 117}$,    
P.~de~Jong$^\textrm{\scriptsize 118}$,    
H.~De~la~Torre$^\textrm{\scriptsize 104}$,    
F.~De~Lorenzi$^\textrm{\scriptsize 76}$,    
A.~De~Maria$^\textrm{\scriptsize 51,v}$,    
D.~De~Pedis$^\textrm{\scriptsize 70a}$,    
A.~De~Salvo$^\textrm{\scriptsize 70a}$,    
U.~De~Sanctis$^\textrm{\scriptsize 71a,71b}$,    
A.~De~Santo$^\textrm{\scriptsize 153}$,    
K.~De~Vasconcelos~Corga$^\textrm{\scriptsize 99}$,    
J.B.~De~Vivie~De~Regie$^\textrm{\scriptsize 128}$,    
C.~Debenedetti$^\textrm{\scriptsize 143}$,    
D.V.~Dedovich$^\textrm{\scriptsize 77}$,    
N.~Dehghanian$^\textrm{\scriptsize 3}$,    
I.~Deigaard$^\textrm{\scriptsize 118}$,    
M.~Del~Gaudio$^\textrm{\scriptsize 40b,40a}$,    
J.~Del~Peso$^\textrm{\scriptsize 96}$,    
D.~Delgove$^\textrm{\scriptsize 128}$,    
F.~Deliot$^\textrm{\scriptsize 142}$,    
C.M.~Delitzsch$^\textrm{\scriptsize 7}$,    
M.~Della~Pietra$^\textrm{\scriptsize 67a,67b}$,    
D.~Della~Volpe$^\textrm{\scriptsize 52}$,    
A.~Dell'Acqua$^\textrm{\scriptsize 35}$,    
L.~Dell'Asta$^\textrm{\scriptsize 25}$,    
M.~Delmastro$^\textrm{\scriptsize 5}$,    
C.~Delporte$^\textrm{\scriptsize 128}$,    
P.A.~Delsart$^\textrm{\scriptsize 56}$,    
D.A.~DeMarco$^\textrm{\scriptsize 165}$,    
S.~Demers$^\textrm{\scriptsize 181}$,    
M.~Demichev$^\textrm{\scriptsize 77}$,    
S.P.~Denisov$^\textrm{\scriptsize 140}$,    
D.~Denysiuk$^\textrm{\scriptsize 118}$,    
L.~D'Eramo$^\textrm{\scriptsize 132}$,    
D.~Derendarz$^\textrm{\scriptsize 82}$,    
J.E.~Derkaoui$^\textrm{\scriptsize 34d}$,    
F.~Derue$^\textrm{\scriptsize 132}$,    
P.~Dervan$^\textrm{\scriptsize 88}$,    
K.~Desch$^\textrm{\scriptsize 24}$,    
C.~Deterre$^\textrm{\scriptsize 44}$,    
K.~Dette$^\textrm{\scriptsize 165}$,    
M.R.~Devesa$^\textrm{\scriptsize 30}$,    
P.O.~Deviveiros$^\textrm{\scriptsize 35}$,    
A.~Dewhurst$^\textrm{\scriptsize 141}$,    
S.~Dhaliwal$^\textrm{\scriptsize 26}$,    
F.A.~Di~Bello$^\textrm{\scriptsize 52}$,    
A.~Di~Ciaccio$^\textrm{\scriptsize 71a,71b}$,    
L.~Di~Ciaccio$^\textrm{\scriptsize 5}$,    
W.K.~Di~Clemente$^\textrm{\scriptsize 133}$,    
C.~Di~Donato$^\textrm{\scriptsize 67a,67b}$,    
A.~Di~Girolamo$^\textrm{\scriptsize 35}$,    
B.~Di~Micco$^\textrm{\scriptsize 72a,72b}$,    
R.~Di~Nardo$^\textrm{\scriptsize 35}$,    
K.F.~Di~Petrillo$^\textrm{\scriptsize 57}$,    
A.~Di~Simone$^\textrm{\scriptsize 50}$,    
R.~Di~Sipio$^\textrm{\scriptsize 165}$,    
D.~Di~Valentino$^\textrm{\scriptsize 33}$,    
C.~Diaconu$^\textrm{\scriptsize 99}$,    
M.~Diamond$^\textrm{\scriptsize 165}$,    
F.A.~Dias$^\textrm{\scriptsize 39}$,    
T.~Dias~Do~Vale$^\textrm{\scriptsize 136a}$,    
M.A.~Diaz$^\textrm{\scriptsize 144a}$,    
J.~Dickinson$^\textrm{\scriptsize 18}$,    
E.B.~Diehl$^\textrm{\scriptsize 103}$,    
J.~Dietrich$^\textrm{\scriptsize 19}$,    
S.~D\'iez~Cornell$^\textrm{\scriptsize 44}$,    
A.~Dimitrievska$^\textrm{\scriptsize 18}$,    
J.~Dingfelder$^\textrm{\scriptsize 24}$,    
P.~Dita$^\textrm{\scriptsize 27b}$,    
S.~Dita$^\textrm{\scriptsize 27b}$,    
F.~Dittus$^\textrm{\scriptsize 35}$,    
F.~Djama$^\textrm{\scriptsize 99}$,    
T.~Djobava$^\textrm{\scriptsize 157b}$,    
J.I.~Djuvsland$^\textrm{\scriptsize 59a}$,    
M.A.B.~Do~Vale$^\textrm{\scriptsize 78c}$,    
M.~Dobre$^\textrm{\scriptsize 27b}$,    
D.~Dodsworth$^\textrm{\scriptsize 26}$,    
C.~Doglioni$^\textrm{\scriptsize 94}$,    
J.~Dolejsi$^\textrm{\scriptsize 139}$,    
Z.~Dolezal$^\textrm{\scriptsize 139}$,    
M.~Donadelli$^\textrm{\scriptsize 78d}$,    
J.~Donini$^\textrm{\scriptsize 37}$,    
M.~D'Onofrio$^\textrm{\scriptsize 88}$,    
J.~Dopke$^\textrm{\scriptsize 141}$,    
A.~Doria$^\textrm{\scriptsize 67a}$,    
M.T.~Dova$^\textrm{\scriptsize 86}$,    
A.T.~Doyle$^\textrm{\scriptsize 55}$,    
E.~Drechsler$^\textrm{\scriptsize 51}$,    
E.~Dreyer$^\textrm{\scriptsize 149}$,    
M.~Dris$^\textrm{\scriptsize 10}$,    
Y.~Du$^\textrm{\scriptsize 58b}$,    
J.~Duarte-Campderros$^\textrm{\scriptsize 159}$,    
F.~Dubinin$^\textrm{\scriptsize 108}$,    
A.~Dubreuil$^\textrm{\scriptsize 52}$,    
E.~Duchovni$^\textrm{\scriptsize 178}$,    
G.~Duckeck$^\textrm{\scriptsize 112}$,    
A.~Ducourthial$^\textrm{\scriptsize 132}$,    
O.A.~Ducu$^\textrm{\scriptsize 107,z}$,    
D.~Duda$^\textrm{\scriptsize 118}$,    
A.~Dudarev$^\textrm{\scriptsize 35}$,    
A.C.~Dudder$^\textrm{\scriptsize 97}$,    
E.M.~Duffield$^\textrm{\scriptsize 18}$,    
L.~Duflot$^\textrm{\scriptsize 128}$,    
M.~D\"uhrssen$^\textrm{\scriptsize 35}$,    
C.~D{\"u}lsen$^\textrm{\scriptsize 180}$,    
M.~Dumancic$^\textrm{\scriptsize 178}$,    
A.E.~Dumitriu$^\textrm{\scriptsize 27b,f}$,    
A.K.~Duncan$^\textrm{\scriptsize 55}$,    
M.~Dunford$^\textrm{\scriptsize 59a}$,    
A.~Duperrin$^\textrm{\scriptsize 99}$,    
H.~Duran~Yildiz$^\textrm{\scriptsize 4a}$,    
M.~D\"uren$^\textrm{\scriptsize 54}$,    
A.~Durglishvili$^\textrm{\scriptsize 157b}$,    
D.~Duschinger$^\textrm{\scriptsize 46}$,    
B.~Dutta$^\textrm{\scriptsize 44}$,    
D.~Duvnjak$^\textrm{\scriptsize 1}$,    
M.~Dyndal$^\textrm{\scriptsize 44}$,    
B.S.~Dziedzic$^\textrm{\scriptsize 82}$,    
C.~Eckardt$^\textrm{\scriptsize 44}$,    
K.M.~Ecker$^\textrm{\scriptsize 113}$,    
R.C.~Edgar$^\textrm{\scriptsize 103}$,    
T.~Eifert$^\textrm{\scriptsize 35}$,    
G.~Eigen$^\textrm{\scriptsize 17}$,    
K.~Einsweiler$^\textrm{\scriptsize 18}$,    
T.~Ekelof$^\textrm{\scriptsize 170}$,    
M.~El~Kacimi$^\textrm{\scriptsize 34c}$,    
R.~El~Kosseifi$^\textrm{\scriptsize 99}$,    
V.~Ellajosyula$^\textrm{\scriptsize 99}$,    
M.~Ellert$^\textrm{\scriptsize 170}$,    
F.~Ellinghaus$^\textrm{\scriptsize 180}$,    
A.A.~Elliot$^\textrm{\scriptsize 174}$,    
N.~Ellis$^\textrm{\scriptsize 35}$,    
J.~Elmsheuser$^\textrm{\scriptsize 29}$,    
M.~Elsing$^\textrm{\scriptsize 35}$,    
D.~Emeliyanov$^\textrm{\scriptsize 141}$,    
Y.~Enari$^\textrm{\scriptsize 161}$,    
J.S.~Ennis$^\textrm{\scriptsize 176}$,    
M.B.~Epland$^\textrm{\scriptsize 47}$,    
J.~Erdmann$^\textrm{\scriptsize 45}$,    
A.~Ereditato$^\textrm{\scriptsize 20}$,    
S.~Errede$^\textrm{\scriptsize 171}$,    
M.~Escalier$^\textrm{\scriptsize 128}$,    
C.~Escobar$^\textrm{\scriptsize 172}$,    
B.~Esposito$^\textrm{\scriptsize 49}$,    
O.~Estrada~Pastor$^\textrm{\scriptsize 172}$,    
A.I.~Etienvre$^\textrm{\scriptsize 142}$,    
E.~Etzion$^\textrm{\scriptsize 159}$,    
H.~Evans$^\textrm{\scriptsize 63}$,    
A.~Ezhilov$^\textrm{\scriptsize 134}$,    
M.~Ezzi$^\textrm{\scriptsize 34e}$,    
F.~Fabbri$^\textrm{\scriptsize 23b,23a}$,    
L.~Fabbri$^\textrm{\scriptsize 23b,23a}$,    
V.~Fabiani$^\textrm{\scriptsize 117}$,    
G.~Facini$^\textrm{\scriptsize 92}$,    
R.M.~Fakhrutdinov$^\textrm{\scriptsize 140}$,    
S.~Falciano$^\textrm{\scriptsize 70a}$,    
J.~Faltova$^\textrm{\scriptsize 139}$,    
Y.~Fang$^\textrm{\scriptsize 15a}$,    
M.~Fanti$^\textrm{\scriptsize 66a,66b}$,    
A.~Farbin$^\textrm{\scriptsize 8}$,    
A.~Farilla$^\textrm{\scriptsize 72a}$,    
E.M.~Farina$^\textrm{\scriptsize 68a,68b}$,    
T.~Farooque$^\textrm{\scriptsize 104}$,    
S.~Farrell$^\textrm{\scriptsize 18}$,    
S.M.~Farrington$^\textrm{\scriptsize 176}$,    
P.~Farthouat$^\textrm{\scriptsize 35}$,    
F.~Fassi$^\textrm{\scriptsize 34e}$,    
P.~Fassnacht$^\textrm{\scriptsize 35}$,    
D.~Fassouliotis$^\textrm{\scriptsize 9}$,    
M.~Faucci~Giannelli$^\textrm{\scriptsize 48}$,    
A.~Favareto$^\textrm{\scriptsize 53b,53a}$,    
W.J.~Fawcett$^\textrm{\scriptsize 52}$,    
L.~Fayard$^\textrm{\scriptsize 128}$,    
O.L.~Fedin$^\textrm{\scriptsize 134,r}$,    
W.~Fedorko$^\textrm{\scriptsize 173}$,    
M.~Feickert$^\textrm{\scriptsize 41}$,    
S.~Feigl$^\textrm{\scriptsize 130}$,    
L.~Feligioni$^\textrm{\scriptsize 99}$,    
C.~Feng$^\textrm{\scriptsize 58b}$,    
E.J.~Feng$^\textrm{\scriptsize 35}$,    
M.~Feng$^\textrm{\scriptsize 47}$,    
M.J.~Fenton$^\textrm{\scriptsize 55}$,    
A.B.~Fenyuk$^\textrm{\scriptsize 140}$,    
L.~Feremenga$^\textrm{\scriptsize 8}$,    
J.~Ferrando$^\textrm{\scriptsize 44}$,    
A.~Ferrari$^\textrm{\scriptsize 170}$,    
P.~Ferrari$^\textrm{\scriptsize 118}$,    
R.~Ferrari$^\textrm{\scriptsize 68a}$,    
D.E.~Ferreira~de~Lima$^\textrm{\scriptsize 59b}$,    
A.~Ferrer$^\textrm{\scriptsize 172}$,    
D.~Ferrere$^\textrm{\scriptsize 52}$,    
C.~Ferretti$^\textrm{\scriptsize 103}$,    
F.~Fiedler$^\textrm{\scriptsize 97}$,    
A.~Filip\v{c}i\v{c}$^\textrm{\scriptsize 89}$,    
F.~Filthaut$^\textrm{\scriptsize 117}$,    
M.~Fincke-Keeler$^\textrm{\scriptsize 174}$,    
K.D.~Finelli$^\textrm{\scriptsize 25}$,    
M.C.N.~Fiolhais$^\textrm{\scriptsize 136a,136c,b}$,    
L.~Fiorini$^\textrm{\scriptsize 172}$,    
C.~Fischer$^\textrm{\scriptsize 14}$,    
J.~Fischer$^\textrm{\scriptsize 180}$,    
W.C.~Fisher$^\textrm{\scriptsize 104}$,    
N.~Flaschel$^\textrm{\scriptsize 44}$,    
I.~Fleck$^\textrm{\scriptsize 148}$,    
P.~Fleischmann$^\textrm{\scriptsize 103}$,    
R.R.M.~Fletcher$^\textrm{\scriptsize 133}$,    
T.~Flick$^\textrm{\scriptsize 180}$,    
B.M.~Flierl$^\textrm{\scriptsize 112}$,    
L.M.~Flores$^\textrm{\scriptsize 133}$,    
L.R.~Flores~Castillo$^\textrm{\scriptsize 61a}$,    
N.~Fomin$^\textrm{\scriptsize 17}$,    
G.T.~Forcolin$^\textrm{\scriptsize 98}$,    
A.~Formica$^\textrm{\scriptsize 142}$,    
F.A.~F\"orster$^\textrm{\scriptsize 14}$,    
A.C.~Forti$^\textrm{\scriptsize 98}$,    
A.G.~Foster$^\textrm{\scriptsize 21}$,    
D.~Fournier$^\textrm{\scriptsize 128}$,    
H.~Fox$^\textrm{\scriptsize 87}$,    
S.~Fracchia$^\textrm{\scriptsize 146}$,    
P.~Francavilla$^\textrm{\scriptsize 69a,69b}$,    
M.~Franchini$^\textrm{\scriptsize 23b,23a}$,    
S.~Franchino$^\textrm{\scriptsize 59a}$,    
D.~Francis$^\textrm{\scriptsize 35}$,    
L.~Franconi$^\textrm{\scriptsize 130}$,    
M.~Franklin$^\textrm{\scriptsize 57}$,    
M.~Frate$^\textrm{\scriptsize 169}$,    
M.~Fraternali$^\textrm{\scriptsize 68a,68b}$,    
D.~Freeborn$^\textrm{\scriptsize 92}$,    
S.M.~Fressard-Batraneanu$^\textrm{\scriptsize 35}$,    
B.~Freund$^\textrm{\scriptsize 107}$,    
W.S.~Freund$^\textrm{\scriptsize 78b}$,    
D.~Froidevaux$^\textrm{\scriptsize 35}$,    
J.A.~Frost$^\textrm{\scriptsize 131}$,    
C.~Fukunaga$^\textrm{\scriptsize 162}$,    
T.~Fusayasu$^\textrm{\scriptsize 114}$,    
J.~Fuster$^\textrm{\scriptsize 172}$,    
O.~Gabizon$^\textrm{\scriptsize 158}$,    
A.~Gabrielli$^\textrm{\scriptsize 23b,23a}$,    
A.~Gabrielli$^\textrm{\scriptsize 18}$,    
G.P.~Gach$^\textrm{\scriptsize 81a}$,    
S.~Gadatsch$^\textrm{\scriptsize 52}$,    
S.~Gadomski$^\textrm{\scriptsize 52}$,    
P.~Gadow$^\textrm{\scriptsize 113}$,    
G.~Gagliardi$^\textrm{\scriptsize 53b,53a}$,    
L.G.~Gagnon$^\textrm{\scriptsize 107}$,    
C.~Galea$^\textrm{\scriptsize 117}$,    
B.~Galhardo$^\textrm{\scriptsize 136a,136c}$,    
E.J.~Gallas$^\textrm{\scriptsize 131}$,    
B.J.~Gallop$^\textrm{\scriptsize 141}$,    
P.~Gallus$^\textrm{\scriptsize 138}$,    
G.~Galster$^\textrm{\scriptsize 39}$,    
R.~Gamboa~Goni$^\textrm{\scriptsize 90}$,    
K.K.~Gan$^\textrm{\scriptsize 122}$,    
S.~Ganguly$^\textrm{\scriptsize 178}$,    
Y.~Gao$^\textrm{\scriptsize 88}$,    
Y.S.~Gao$^\textrm{\scriptsize 150,n}$,    
C.~Garc\'ia$^\textrm{\scriptsize 172}$,    
J.E.~Garc\'ia~Navarro$^\textrm{\scriptsize 172}$,    
J.A.~Garc\'ia~Pascual$^\textrm{\scriptsize 15a}$,    
M.~Garcia-Sciveres$^\textrm{\scriptsize 18}$,    
R.W.~Gardner$^\textrm{\scriptsize 36}$,    
N.~Garelli$^\textrm{\scriptsize 150}$,    
V.~Garonne$^\textrm{\scriptsize 130}$,    
K.~Gasnikova$^\textrm{\scriptsize 44}$,    
A.~Gaudiello$^\textrm{\scriptsize 53b,53a}$,    
G.~Gaudio$^\textrm{\scriptsize 68a}$,    
I.L.~Gavrilenko$^\textrm{\scriptsize 108}$,    
A.~Gavrilyuk$^\textrm{\scriptsize 109}$,    
C.~Gay$^\textrm{\scriptsize 173}$,    
G.~Gaycken$^\textrm{\scriptsize 24}$,    
E.N.~Gazis$^\textrm{\scriptsize 10}$,    
C.N.P.~Gee$^\textrm{\scriptsize 141}$,    
J.~Geisen$^\textrm{\scriptsize 51}$,    
M.~Geisen$^\textrm{\scriptsize 97}$,    
M.P.~Geisler$^\textrm{\scriptsize 59a}$,    
K.~Gellerstedt$^\textrm{\scriptsize 43a,43b}$,    
C.~Gemme$^\textrm{\scriptsize 53b}$,    
M.H.~Genest$^\textrm{\scriptsize 56}$,    
C.~Geng$^\textrm{\scriptsize 103}$,    
S.~Gentile$^\textrm{\scriptsize 70a,70b}$,    
C.~Gentsos$^\textrm{\scriptsize 160}$,    
S.~George$^\textrm{\scriptsize 91}$,    
D.~Gerbaudo$^\textrm{\scriptsize 14}$,    
G.~Gessner$^\textrm{\scriptsize 45}$,    
S.~Ghasemi$^\textrm{\scriptsize 148}$,    
M.~Ghneimat$^\textrm{\scriptsize 24}$,    
B.~Giacobbe$^\textrm{\scriptsize 23b}$,    
S.~Giagu$^\textrm{\scriptsize 70a,70b}$,    
N.~Giangiacomi$^\textrm{\scriptsize 23b,23a}$,    
P.~Giannetti$^\textrm{\scriptsize 69a}$,    
S.M.~Gibson$^\textrm{\scriptsize 91}$,    
M.~Gignac$^\textrm{\scriptsize 143}$,    
M.~Gilchriese$^\textrm{\scriptsize 18}$,    
D.~Gillberg$^\textrm{\scriptsize 33}$,    
G.~Gilles$^\textrm{\scriptsize 180}$,    
D.M.~Gingrich$^\textrm{\scriptsize 3,ax}$,    
M.P.~Giordani$^\textrm{\scriptsize 64a,64c}$,    
F.M.~Giorgi$^\textrm{\scriptsize 23b}$,    
P.F.~Giraud$^\textrm{\scriptsize 142}$,    
P.~Giromini$^\textrm{\scriptsize 57}$,    
G.~Giugliarelli$^\textrm{\scriptsize 64a,64c}$,    
D.~Giugni$^\textrm{\scriptsize 66a}$,    
F.~Giuli$^\textrm{\scriptsize 131}$,    
M.~Giulini$^\textrm{\scriptsize 59b}$,    
S.~Gkaitatzis$^\textrm{\scriptsize 160}$,    
I.~Gkialas$^\textrm{\scriptsize 9,k}$,    
E.L.~Gkougkousis$^\textrm{\scriptsize 14}$,    
P.~Gkountoumis$^\textrm{\scriptsize 10}$,    
L.K.~Gladilin$^\textrm{\scriptsize 111}$,    
C.~Glasman$^\textrm{\scriptsize 96}$,    
J.~Glatzer$^\textrm{\scriptsize 14}$,    
P.C.F.~Glaysher$^\textrm{\scriptsize 44}$,    
A.~Glazov$^\textrm{\scriptsize 44}$,    
M.~Goblirsch-Kolb$^\textrm{\scriptsize 26}$,    
J.~Godlewski$^\textrm{\scriptsize 82}$,    
S.~Goldfarb$^\textrm{\scriptsize 102}$,    
T.~Golling$^\textrm{\scriptsize 52}$,    
D.~Golubkov$^\textrm{\scriptsize 140}$,    
A.~Gomes$^\textrm{\scriptsize 136a,136b,136d}$,    
R.~Goncalves~Gama$^\textrm{\scriptsize 78a}$,    
R.~Gon\c{c}alo$^\textrm{\scriptsize 136a}$,    
G.~Gonella$^\textrm{\scriptsize 50}$,    
L.~Gonella$^\textrm{\scriptsize 21}$,    
A.~Gongadze$^\textrm{\scriptsize 77}$,    
F.~Gonnella$^\textrm{\scriptsize 21}$,    
J.L.~Gonski$^\textrm{\scriptsize 57}$,    
S.~Gonz\'alez~de~la~Hoz$^\textrm{\scriptsize 172}$,    
S.~Gonzalez-Sevilla$^\textrm{\scriptsize 52}$,    
L.~Goossens$^\textrm{\scriptsize 35}$,    
P.A.~Gorbounov$^\textrm{\scriptsize 109}$,    
H.A.~Gordon$^\textrm{\scriptsize 29}$,    
B.~Gorini$^\textrm{\scriptsize 35}$,    
E.~Gorini$^\textrm{\scriptsize 65a,65b}$,    
A.~Gori\v{s}ek$^\textrm{\scriptsize 89}$,    
A.T.~Goshaw$^\textrm{\scriptsize 47}$,    
C.~G\"ossling$^\textrm{\scriptsize 45}$,    
M.I.~Gostkin$^\textrm{\scriptsize 77}$,    
C.A.~Gottardo$^\textrm{\scriptsize 24}$,    
C.R.~Goudet$^\textrm{\scriptsize 128}$,    
D.~Goujdami$^\textrm{\scriptsize 34c}$,    
A.G.~Goussiou$^\textrm{\scriptsize 145}$,    
N.~Govender$^\textrm{\scriptsize 32b,d}$,    
C.~Goy$^\textrm{\scriptsize 5}$,    
E.~Gozani$^\textrm{\scriptsize 158}$,    
I.~Grabowska-Bold$^\textrm{\scriptsize 81a}$,    
P.O.J.~Gradin$^\textrm{\scriptsize 170}$,    
E.C.~Graham$^\textrm{\scriptsize 88}$,    
J.~Gramling$^\textrm{\scriptsize 169}$,    
E.~Gramstad$^\textrm{\scriptsize 130}$,    
S.~Grancagnolo$^\textrm{\scriptsize 19}$,    
V.~Gratchev$^\textrm{\scriptsize 134}$,    
P.M.~Gravila$^\textrm{\scriptsize 27f}$,    
C.~Gray$^\textrm{\scriptsize 55}$,    
H.M.~Gray$^\textrm{\scriptsize 18}$,    
Z.D.~Greenwood$^\textrm{\scriptsize 93,al}$,    
C.~Grefe$^\textrm{\scriptsize 24}$,    
K.~Gregersen$^\textrm{\scriptsize 92}$,    
I.M.~Gregor$^\textrm{\scriptsize 44}$,    
P.~Grenier$^\textrm{\scriptsize 150}$,    
K.~Grevtsov$^\textrm{\scriptsize 44}$,    
J.~Griffiths$^\textrm{\scriptsize 8}$,    
A.A.~Grillo$^\textrm{\scriptsize 143}$,    
K.~Grimm$^\textrm{\scriptsize 150,c}$,    
S.~Grinstein$^\textrm{\scriptsize 14,ab}$,    
Ph.~Gris$^\textrm{\scriptsize 37}$,    
J.-F.~Grivaz$^\textrm{\scriptsize 128}$,    
S.~Groh$^\textrm{\scriptsize 97}$,    
E.~Gross$^\textrm{\scriptsize 178}$,    
J.~Grosse-Knetter$^\textrm{\scriptsize 51}$,    
G.C.~Grossi$^\textrm{\scriptsize 93}$,    
Z.J.~Grout$^\textrm{\scriptsize 92}$,    
A.~Grummer$^\textrm{\scriptsize 116}$,    
L.~Guan$^\textrm{\scriptsize 103}$,    
W.~Guan$^\textrm{\scriptsize 179}$,    
J.~Guenther$^\textrm{\scriptsize 35}$,    
A.~Guerguichon$^\textrm{\scriptsize 128}$,    
F.~Guescini$^\textrm{\scriptsize 166a}$,    
D.~Guest$^\textrm{\scriptsize 169}$,    
O.~Gueta$^\textrm{\scriptsize 159}$,    
R.~Gugel$^\textrm{\scriptsize 50}$,    
B.~Gui$^\textrm{\scriptsize 122}$,    
T.~Guillemin$^\textrm{\scriptsize 5}$,    
S.~Guindon$^\textrm{\scriptsize 35}$,    
U.~Gul$^\textrm{\scriptsize 55}$,    
C.~Gumpert$^\textrm{\scriptsize 35}$,    
J.~Guo$^\textrm{\scriptsize 58c}$,    
W.~Guo$^\textrm{\scriptsize 103}$,    
Y.~Guo$^\textrm{\scriptsize 58a,u}$,    
R.~Gupta$^\textrm{\scriptsize 41}$,    
S.~Gurbuz$^\textrm{\scriptsize 12c}$,    
G.~Gustavino$^\textrm{\scriptsize 124}$,    
B.J.~Gutelman$^\textrm{\scriptsize 158}$,    
P.~Gutierrez$^\textrm{\scriptsize 124}$,    
N.G.~Gutierrez~Ortiz$^\textrm{\scriptsize 92}$,    
C.~Gutschow$^\textrm{\scriptsize 92}$,    
C.~Guyot$^\textrm{\scriptsize 142}$,    
M.P.~Guzik$^\textrm{\scriptsize 81a}$,    
C.~Gwenlan$^\textrm{\scriptsize 131}$,    
C.B.~Gwilliam$^\textrm{\scriptsize 88}$,    
A.~Haas$^\textrm{\scriptsize 121}$,    
C.~Haber$^\textrm{\scriptsize 18}$,    
H.K.~Hadavand$^\textrm{\scriptsize 8}$,    
N.~Haddad$^\textrm{\scriptsize 34e}$,    
A.~Hadef$^\textrm{\scriptsize 99}$,    
S.~Hageb\"ock$^\textrm{\scriptsize 24}$,    
M.~Hagihara$^\textrm{\scriptsize 167}$,    
H.~Hakobyan$^\textrm{\scriptsize 182,*}$,    
M.~Haleem$^\textrm{\scriptsize 175}$,    
J.~Haley$^\textrm{\scriptsize 125}$,    
G.~Halladjian$^\textrm{\scriptsize 104}$,    
G.D.~Hallewell$^\textrm{\scriptsize 99}$,    
K.~Hamacher$^\textrm{\scriptsize 180}$,    
P.~Hamal$^\textrm{\scriptsize 126}$,    
K.~Hamano$^\textrm{\scriptsize 174}$,    
A.~Hamilton$^\textrm{\scriptsize 32a}$,    
G.N.~Hamity$^\textrm{\scriptsize 146}$,    
K.~Han$^\textrm{\scriptsize 58a,ak}$,    
L.~Han$^\textrm{\scriptsize 58a}$,    
S.~Han$^\textrm{\scriptsize 15d}$,    
K.~Hanagaki$^\textrm{\scriptsize 79,x}$,    
M.~Hance$^\textrm{\scriptsize 143}$,    
D.M.~Handl$^\textrm{\scriptsize 112}$,    
B.~Haney$^\textrm{\scriptsize 133}$,    
R.~Hankache$^\textrm{\scriptsize 132}$,    
P.~Hanke$^\textrm{\scriptsize 59a}$,    
E.~Hansen$^\textrm{\scriptsize 94}$,    
J.B.~Hansen$^\textrm{\scriptsize 39}$,    
J.D.~Hansen$^\textrm{\scriptsize 39}$,    
M.C.~Hansen$^\textrm{\scriptsize 24}$,    
P.H.~Hansen$^\textrm{\scriptsize 39}$,    
K.~Hara$^\textrm{\scriptsize 167}$,    
A.S.~Hard$^\textrm{\scriptsize 179}$,    
T.~Harenberg$^\textrm{\scriptsize 180}$,    
S.~Harkusha$^\textrm{\scriptsize 105}$,    
P.F.~Harrison$^\textrm{\scriptsize 176}$,    
N.M.~Hartmann$^\textrm{\scriptsize 112}$,    
Y.~Hasegawa$^\textrm{\scriptsize 147}$,    
A.~Hasib$^\textrm{\scriptsize 48}$,    
S.~Hassani$^\textrm{\scriptsize 142}$,    
S.~Haug$^\textrm{\scriptsize 20}$,    
R.~Hauser$^\textrm{\scriptsize 104}$,    
L.~Hauswald$^\textrm{\scriptsize 46}$,    
L.B.~Havener$^\textrm{\scriptsize 38}$,    
M.~Havranek$^\textrm{\scriptsize 138}$,    
C.M.~Hawkes$^\textrm{\scriptsize 21}$,    
R.J.~Hawkings$^\textrm{\scriptsize 35}$,    
D.~Hayden$^\textrm{\scriptsize 104}$,    
C.P.~Hays$^\textrm{\scriptsize 131}$,    
J.M.~Hays$^\textrm{\scriptsize 90}$,    
H.S.~Hayward$^\textrm{\scriptsize 88}$,    
S.J.~Haywood$^\textrm{\scriptsize 141}$,    
M.P.~Heath$^\textrm{\scriptsize 48}$,    
T.~Heck$^\textrm{\scriptsize 97}$,    
V.~Hedberg$^\textrm{\scriptsize 94}$,    
L.~Heelan$^\textrm{\scriptsize 8}$,    
S.~Heer$^\textrm{\scriptsize 24}$,    
K.K.~Heidegger$^\textrm{\scriptsize 50}$,    
S.~Heim$^\textrm{\scriptsize 44}$,    
T.~Heim$^\textrm{\scriptsize 18}$,    
B.~Heinemann$^\textrm{\scriptsize 44,as}$,    
J.J.~Heinrich$^\textrm{\scriptsize 112}$,    
L.~Heinrich$^\textrm{\scriptsize 121}$,    
C.~Heinz$^\textrm{\scriptsize 54}$,    
J.~Hejbal$^\textrm{\scriptsize 137}$,    
L.~Helary$^\textrm{\scriptsize 35}$,    
A.~Held$^\textrm{\scriptsize 173}$,    
S.~Hellesund$^\textrm{\scriptsize 130}$,    
S.~Hellman$^\textrm{\scriptsize 43a,43b}$,    
C.~Helsens$^\textrm{\scriptsize 35}$,    
R.C.W.~Henderson$^\textrm{\scriptsize 87}$,    
Y.~Heng$^\textrm{\scriptsize 179}$,    
S.~Henkelmann$^\textrm{\scriptsize 173}$,    
A.M.~Henriques~Correia$^\textrm{\scriptsize 35}$,    
G.H.~Herbert$^\textrm{\scriptsize 19}$,    
H.~Herde$^\textrm{\scriptsize 26}$,    
V.~Herget$^\textrm{\scriptsize 175}$,    
Y.~Hern\'andez~Jim\'enez$^\textrm{\scriptsize 32c}$,    
H.~Herr$^\textrm{\scriptsize 97}$,    
G.~Herten$^\textrm{\scriptsize 50}$,    
R.~Hertenberger$^\textrm{\scriptsize 112}$,    
L.~Hervas$^\textrm{\scriptsize 35}$,    
T.C.~Herwig$^\textrm{\scriptsize 133}$,    
G.G.~Hesketh$^\textrm{\scriptsize 92}$,    
N.P.~Hessey$^\textrm{\scriptsize 166a}$,    
J.W.~Hetherly$^\textrm{\scriptsize 41}$,    
S.~Higashino$^\textrm{\scriptsize 79}$,    
E.~Hig\'on-Rodriguez$^\textrm{\scriptsize 172}$,    
K.~Hildebrand$^\textrm{\scriptsize 36}$,    
E.~Hill$^\textrm{\scriptsize 174}$,    
J.C.~Hill$^\textrm{\scriptsize 31}$,    
K.H.~Hiller$^\textrm{\scriptsize 44}$,    
S.J.~Hillier$^\textrm{\scriptsize 21}$,    
M.~Hils$^\textrm{\scriptsize 46}$,    
I.~Hinchliffe$^\textrm{\scriptsize 18}$,    
M.~Hirose$^\textrm{\scriptsize 129}$,    
D.~Hirschbuehl$^\textrm{\scriptsize 180}$,    
B.~Hiti$^\textrm{\scriptsize 89}$,    
O.~Hladik$^\textrm{\scriptsize 137}$,    
D.R.~Hlaluku$^\textrm{\scriptsize 32c}$,    
X.~Hoad$^\textrm{\scriptsize 48}$,    
J.~Hobbs$^\textrm{\scriptsize 152}$,    
N.~Hod$^\textrm{\scriptsize 166a}$,    
M.C.~Hodgkinson$^\textrm{\scriptsize 146}$,    
A.~Hoecker$^\textrm{\scriptsize 35}$,    
M.R.~Hoeferkamp$^\textrm{\scriptsize 116}$,    
F.~Hoenig$^\textrm{\scriptsize 112}$,    
D.~Hohn$^\textrm{\scriptsize 24}$,    
D.~Hohov$^\textrm{\scriptsize 128}$,    
T.R.~Holmes$^\textrm{\scriptsize 36}$,    
M.~Holzbock$^\textrm{\scriptsize 112}$,    
M.~Homann$^\textrm{\scriptsize 45}$,    
S.~Honda$^\textrm{\scriptsize 167}$,    
T.~Honda$^\textrm{\scriptsize 79}$,    
T.M.~Hong$^\textrm{\scriptsize 135}$,    
B.H.~Hooberman$^\textrm{\scriptsize 171}$,    
W.H.~Hopkins$^\textrm{\scriptsize 127}$,    
Y.~Horii$^\textrm{\scriptsize 115}$,    
A.J.~Horton$^\textrm{\scriptsize 149}$,    
L.A.~Horyn$^\textrm{\scriptsize 36}$,    
J-Y.~Hostachy$^\textrm{\scriptsize 56}$,    
A.~Hostiuc$^\textrm{\scriptsize 145}$,    
S.~Hou$^\textrm{\scriptsize 155}$,    
A.~Hoummada$^\textrm{\scriptsize 34a}$,    
J.~Howarth$^\textrm{\scriptsize 98}$,    
J.~Hoya$^\textrm{\scriptsize 86}$,    
M.~Hrabovsky$^\textrm{\scriptsize 126}$,    
J.~Hrdinka$^\textrm{\scriptsize 35}$,    
I.~Hristova$^\textrm{\scriptsize 19}$,    
J.~Hrivnac$^\textrm{\scriptsize 128}$,    
A.~Hrynevich$^\textrm{\scriptsize 106}$,    
T.~Hryn'ova$^\textrm{\scriptsize 5}$,    
P.J.~Hsu$^\textrm{\scriptsize 62}$,    
S.-C.~Hsu$^\textrm{\scriptsize 145}$,    
Q.~Hu$^\textrm{\scriptsize 29}$,    
S.~Hu$^\textrm{\scriptsize 58c}$,    
Y.~Huang$^\textrm{\scriptsize 15a}$,    
Z.~Hubacek$^\textrm{\scriptsize 138}$,    
F.~Hubaut$^\textrm{\scriptsize 99}$,    
F.~Huegging$^\textrm{\scriptsize 24}$,    
T.B.~Huffman$^\textrm{\scriptsize 131}$,    
E.W.~Hughes$^\textrm{\scriptsize 38}$,    
M.~Huhtinen$^\textrm{\scriptsize 35}$,    
R.F.H.~Hunter$^\textrm{\scriptsize 33}$,    
P.~Huo$^\textrm{\scriptsize 152}$,    
A.M.~Hupe$^\textrm{\scriptsize 33}$,    
N.~Huseynov$^\textrm{\scriptsize 77,ai}$,    
J.~Huston$^\textrm{\scriptsize 104}$,    
J.~Huth$^\textrm{\scriptsize 57}$,    
R.~Hyneman$^\textrm{\scriptsize 103}$,    
G.~Iacobucci$^\textrm{\scriptsize 52}$,    
G.~Iakovidis$^\textrm{\scriptsize 29}$,    
I.~Ibragimov$^\textrm{\scriptsize 148}$,    
L.~Iconomidou-Fayard$^\textrm{\scriptsize 128}$,    
Z.~Idrissi$^\textrm{\scriptsize 34e}$,    
P.~Iengo$^\textrm{\scriptsize 35}$,    
R.~Ignazzi$^\textrm{\scriptsize 39}$,    
O.~Igonkina$^\textrm{\scriptsize 118,ae}$,    
R.~Iguchi$^\textrm{\scriptsize 161}$,    
T.~Iizawa$^\textrm{\scriptsize 177}$,    
Y.~Ikegami$^\textrm{\scriptsize 79}$,    
M.~Ikeno$^\textrm{\scriptsize 79}$,    
D.~Iliadis$^\textrm{\scriptsize 160}$,    
N.~Ilic$^\textrm{\scriptsize 150}$,    
F.~Iltzsche$^\textrm{\scriptsize 46}$,    
G.~Introzzi$^\textrm{\scriptsize 68a,68b}$,    
M.~Iodice$^\textrm{\scriptsize 72a}$,    
K.~Iordanidou$^\textrm{\scriptsize 38}$,    
V.~Ippolito$^\textrm{\scriptsize 70a,70b}$,    
M.F.~Isacson$^\textrm{\scriptsize 170}$,    
N.~Ishijima$^\textrm{\scriptsize 129}$,    
M.~Ishino$^\textrm{\scriptsize 161}$,    
M.~Ishitsuka$^\textrm{\scriptsize 163}$,    
C.~Issever$^\textrm{\scriptsize 131}$,    
S.~Istin$^\textrm{\scriptsize 12c,aq}$,    
F.~Ito$^\textrm{\scriptsize 167}$,    
J.M.~Iturbe~Ponce$^\textrm{\scriptsize 61a}$,    
R.~Iuppa$^\textrm{\scriptsize 73a,73b}$,    
H.~Iwasaki$^\textrm{\scriptsize 79}$,    
J.M.~Izen$^\textrm{\scriptsize 42}$,    
V.~Izzo$^\textrm{\scriptsize 67a}$,    
S.~Jabbar$^\textrm{\scriptsize 3}$,    
P.~Jacka$^\textrm{\scriptsize 137}$,    
P.~Jackson$^\textrm{\scriptsize 1}$,    
R.M.~Jacobs$^\textrm{\scriptsize 24}$,    
V.~Jain$^\textrm{\scriptsize 2}$,    
G.~J\"akel$^\textrm{\scriptsize 180}$,    
K.B.~Jakobi$^\textrm{\scriptsize 97}$,    
K.~Jakobs$^\textrm{\scriptsize 50}$,    
S.~Jakobsen$^\textrm{\scriptsize 74}$,    
T.~Jakoubek$^\textrm{\scriptsize 137}$,    
D.O.~Jamin$^\textrm{\scriptsize 125}$,    
D.K.~Jana$^\textrm{\scriptsize 93}$,    
R.~Jansky$^\textrm{\scriptsize 52}$,    
J.~Janssen$^\textrm{\scriptsize 24}$,    
M.~Janus$^\textrm{\scriptsize 51}$,    
P.A.~Janus$^\textrm{\scriptsize 81a}$,    
G.~Jarlskog$^\textrm{\scriptsize 94}$,    
N.~Javadov$^\textrm{\scriptsize 77,ai}$,    
T.~Jav\r{u}rek$^\textrm{\scriptsize 50}$,    
M.~Javurkova$^\textrm{\scriptsize 50}$,    
F.~Jeanneau$^\textrm{\scriptsize 142}$,    
L.~Jeanty$^\textrm{\scriptsize 18}$,    
J.~Jejelava$^\textrm{\scriptsize 157a,aj}$,    
A.~Jelinskas$^\textrm{\scriptsize 176}$,    
P.~Jenni$^\textrm{\scriptsize 50,e}$,    
C.~Jeske$^\textrm{\scriptsize 176}$,    
S.~J\'ez\'equel$^\textrm{\scriptsize 5}$,    
H.~Ji$^\textrm{\scriptsize 179}$,    
J.~Jia$^\textrm{\scriptsize 152}$,    
H.~Jiang$^\textrm{\scriptsize 76}$,    
Y.~Jiang$^\textrm{\scriptsize 58a}$,    
Z.~Jiang$^\textrm{\scriptsize 150,s}$,    
S.~Jiggins$^\textrm{\scriptsize 92}$,    
J.~Jimenez~Pena$^\textrm{\scriptsize 172}$,    
S.~Jin$^\textrm{\scriptsize 15c}$,    
A.~Jinaru$^\textrm{\scriptsize 27b}$,    
O.~Jinnouchi$^\textrm{\scriptsize 163}$,    
H.~Jivan$^\textrm{\scriptsize 32c}$,    
P.~Johansson$^\textrm{\scriptsize 146}$,    
K.A.~Johns$^\textrm{\scriptsize 7}$,    
C.A.~Johnson$^\textrm{\scriptsize 63}$,    
W.J.~Johnson$^\textrm{\scriptsize 145}$,    
K.~Jon-And$^\textrm{\scriptsize 43a,43b}$,    
R.W.L.~Jones$^\textrm{\scriptsize 87}$,    
S.D.~Jones$^\textrm{\scriptsize 153}$,    
S.~Jones$^\textrm{\scriptsize 7}$,    
T.J.~Jones$^\textrm{\scriptsize 88}$,    
J.~Jongmanns$^\textrm{\scriptsize 59a}$,    
P.M.~Jorge$^\textrm{\scriptsize 136a,136b}$,    
J.~Jovicevic$^\textrm{\scriptsize 166a}$,    
X.~Ju$^\textrm{\scriptsize 179}$,    
J.J.~Junggeburth$^\textrm{\scriptsize 113}$,    
A.~Juste~Rozas$^\textrm{\scriptsize 14,ab}$,    
A.~Kaczmarska$^\textrm{\scriptsize 82}$,    
M.~Kado$^\textrm{\scriptsize 128}$,    
H.~Kagan$^\textrm{\scriptsize 122}$,    
M.~Kagan$^\textrm{\scriptsize 150}$,    
T.~Kaji$^\textrm{\scriptsize 177}$,    
E.~Kajomovitz$^\textrm{\scriptsize 158}$,    
C.W.~Kalderon$^\textrm{\scriptsize 94}$,    
A.~Kaluza$^\textrm{\scriptsize 97}$,    
S.~Kama$^\textrm{\scriptsize 41}$,    
A.~Kamenshchikov$^\textrm{\scriptsize 140}$,    
L.~Kanjir$^\textrm{\scriptsize 89}$,    
Y.~Kano$^\textrm{\scriptsize 161}$,    
V.A.~Kantserov$^\textrm{\scriptsize 110}$,    
J.~Kanzaki$^\textrm{\scriptsize 79}$,    
B.~Kaplan$^\textrm{\scriptsize 121}$,    
L.S.~Kaplan$^\textrm{\scriptsize 179}$,    
D.~Kar$^\textrm{\scriptsize 32c}$,    
K.~Karakostas$^\textrm{\scriptsize 10}$,    
N.~Karastathis$^\textrm{\scriptsize 10}$,    
M.J.~Kareem$^\textrm{\scriptsize 166b}$,    
E.~Karentzos$^\textrm{\scriptsize 10}$,    
S.N.~Karpov$^\textrm{\scriptsize 77}$,    
Z.M.~Karpova$^\textrm{\scriptsize 77}$,    
V.~Kartvelishvili$^\textrm{\scriptsize 87}$,    
A.N.~Karyukhin$^\textrm{\scriptsize 140}$,    
K.~Kasahara$^\textrm{\scriptsize 167}$,    
L.~Kashif$^\textrm{\scriptsize 179}$,    
R.D.~Kass$^\textrm{\scriptsize 122}$,    
A.~Kastanas$^\textrm{\scriptsize 151}$,    
Y.~Kataoka$^\textrm{\scriptsize 161}$,    
C.~Kato$^\textrm{\scriptsize 161}$,    
A.~Katre$^\textrm{\scriptsize 52}$,    
J.~Katzy$^\textrm{\scriptsize 44}$,    
K.~Kawade$^\textrm{\scriptsize 80}$,    
K.~Kawagoe$^\textrm{\scriptsize 85}$,    
T.~Kawamoto$^\textrm{\scriptsize 161}$,    
G.~Kawamura$^\textrm{\scriptsize 51}$,    
E.F.~Kay$^\textrm{\scriptsize 88}$,    
V.F.~Kazanin$^\textrm{\scriptsize 120b,120a}$,    
R.~Keeler$^\textrm{\scriptsize 174}$,    
R.~Kehoe$^\textrm{\scriptsize 41}$,    
J.S.~Keller$^\textrm{\scriptsize 33}$,    
E.~Kellermann$^\textrm{\scriptsize 94}$,    
J.J.~Kempster$^\textrm{\scriptsize 21}$,    
J.~Kendrick$^\textrm{\scriptsize 21}$,    
O.~Kepka$^\textrm{\scriptsize 137}$,    
S.~Kersten$^\textrm{\scriptsize 180}$,    
B.P.~Ker\v{s}evan$^\textrm{\scriptsize 89}$,    
R.A.~Keyes$^\textrm{\scriptsize 101}$,    
M.~Khader$^\textrm{\scriptsize 171}$,    
F.~Khalil-Zada$^\textrm{\scriptsize 13}$,    
A.~Khanov$^\textrm{\scriptsize 125}$,    
A.G.~Kharlamov$^\textrm{\scriptsize 120b,120a}$,    
T.~Kharlamova$^\textrm{\scriptsize 120b,120a}$,    
A.~Khodinov$^\textrm{\scriptsize 164}$,    
T.J.~Khoo$^\textrm{\scriptsize 52}$,    
V.~Khovanskiy$^\textrm{\scriptsize 109,*}$,    
E.~Khramov$^\textrm{\scriptsize 77}$,    
J.~Khubua$^\textrm{\scriptsize 157b}$,    
S.~Kido$^\textrm{\scriptsize 80}$,    
M.~Kiehn$^\textrm{\scriptsize 52}$,    
C.R.~Kilby$^\textrm{\scriptsize 91}$,    
H.Y.~Kim$^\textrm{\scriptsize 8}$,    
S.H.~Kim$^\textrm{\scriptsize 167}$,    
Y.K.~Kim$^\textrm{\scriptsize 36}$,    
N.~Kimura$^\textrm{\scriptsize 64a,64c}$,    
O.M.~Kind$^\textrm{\scriptsize 19}$,    
B.T.~King$^\textrm{\scriptsize 88}$,    
D.~Kirchmeier$^\textrm{\scriptsize 46}$,    
J.~Kirk$^\textrm{\scriptsize 141}$,    
A.E.~Kiryunin$^\textrm{\scriptsize 113}$,    
T.~Kishimoto$^\textrm{\scriptsize 161}$,    
D.~Kisielewska$^\textrm{\scriptsize 81a}$,    
V.~Kitali$^\textrm{\scriptsize 44}$,    
O.~Kivernyk$^\textrm{\scriptsize 5}$,    
E.~Kladiva$^\textrm{\scriptsize 28b,*}$,    
T.~Klapdor-Kleingrothaus$^\textrm{\scriptsize 50}$,    
M.H.~Klein$^\textrm{\scriptsize 103}$,    
M.~Klein$^\textrm{\scriptsize 88}$,    
U.~Klein$^\textrm{\scriptsize 88}$,    
K.~Kleinknecht$^\textrm{\scriptsize 97}$,    
P.~Klimek$^\textrm{\scriptsize 119}$,    
A.~Klimentov$^\textrm{\scriptsize 29}$,    
R.~Klingenberg$^\textrm{\scriptsize 45,*}$,    
T.~Klingl$^\textrm{\scriptsize 24}$,    
T.~Klioutchnikova$^\textrm{\scriptsize 35}$,    
F.F.~Klitzner$^\textrm{\scriptsize 112}$,    
P.~Kluit$^\textrm{\scriptsize 118}$,    
S.~Kluth$^\textrm{\scriptsize 113}$,    
E.~Kneringer$^\textrm{\scriptsize 74}$,    
E.B.F.G.~Knoops$^\textrm{\scriptsize 99}$,    
A.~Knue$^\textrm{\scriptsize 50}$,    
A.~Kobayashi$^\textrm{\scriptsize 161}$,    
D.~Kobayashi$^\textrm{\scriptsize 85}$,    
T.~Kobayashi$^\textrm{\scriptsize 161}$,    
M.~Kobel$^\textrm{\scriptsize 46}$,    
M.~Kocian$^\textrm{\scriptsize 150}$,    
P.~Kodys$^\textrm{\scriptsize 139}$,    
T.~Koffas$^\textrm{\scriptsize 33}$,    
E.~Koffeman$^\textrm{\scriptsize 118}$,    
N.M.~K\"ohler$^\textrm{\scriptsize 113}$,    
T.~Koi$^\textrm{\scriptsize 150}$,    
M.~Kolb$^\textrm{\scriptsize 59b}$,    
I.~Koletsou$^\textrm{\scriptsize 5}$,    
T.~Kondo$^\textrm{\scriptsize 79}$,    
N.~Kondrashova$^\textrm{\scriptsize 58c}$,    
K.~K\"oneke$^\textrm{\scriptsize 50}$,    
A.C.~K\"onig$^\textrm{\scriptsize 117}$,    
T.~Kono$^\textrm{\scriptsize 79,ar}$,    
R.~Konoplich$^\textrm{\scriptsize 121,an}$,    
N.~Konstantinidis$^\textrm{\scriptsize 92}$,    
B.~Konya$^\textrm{\scriptsize 94}$,    
R.~Kopeliansky$^\textrm{\scriptsize 63}$,    
S.~Koperny$^\textrm{\scriptsize 81a}$,    
K.~Korcyl$^\textrm{\scriptsize 82}$,    
K.~Kordas$^\textrm{\scriptsize 160}$,    
A.~Korn$^\textrm{\scriptsize 92}$,    
I.~Korolkov$^\textrm{\scriptsize 14}$,    
E.V.~Korolkova$^\textrm{\scriptsize 146}$,    
O.~Kortner$^\textrm{\scriptsize 113}$,    
S.~Kortner$^\textrm{\scriptsize 113}$,    
T.~Kosek$^\textrm{\scriptsize 139}$,    
V.V.~Kostyukhin$^\textrm{\scriptsize 24}$,    
A.~Kotwal$^\textrm{\scriptsize 47}$,    
A.~Koulouris$^\textrm{\scriptsize 10}$,    
A.~Kourkoumeli-Charalampidi$^\textrm{\scriptsize 68a,68b}$,    
C.~Kourkoumelis$^\textrm{\scriptsize 9}$,    
E.~Kourlitis$^\textrm{\scriptsize 146}$,    
V.~Kouskoura$^\textrm{\scriptsize 29}$,    
A.B.~Kowalewska$^\textrm{\scriptsize 82}$,    
R.~Kowalewski$^\textrm{\scriptsize 174}$,    
T.Z.~Kowalski$^\textrm{\scriptsize 81a}$,    
C.~Kozakai$^\textrm{\scriptsize 161}$,    
W.~Kozanecki$^\textrm{\scriptsize 142}$,    
A.S.~Kozhin$^\textrm{\scriptsize 140}$,    
V.A.~Kramarenko$^\textrm{\scriptsize 111}$,    
G.~Kramberger$^\textrm{\scriptsize 89}$,    
D.~Krasnopevtsev$^\textrm{\scriptsize 110}$,    
M.W.~Krasny$^\textrm{\scriptsize 132}$,    
A.~Krasznahorkay$^\textrm{\scriptsize 35}$,    
D.~Krauss$^\textrm{\scriptsize 113}$,    
J.A.~Kremer$^\textrm{\scriptsize 81a}$,    
J.~Kretzschmar$^\textrm{\scriptsize 88}$,    
K.~Kreutzfeldt$^\textrm{\scriptsize 54}$,    
P.~Krieger$^\textrm{\scriptsize 165}$,    
F.~Krieter$^\textrm{\scriptsize 112}$,    
K.~Krizka$^\textrm{\scriptsize 18}$,    
K.~Kroeninger$^\textrm{\scriptsize 45}$,    
H.~Kroha$^\textrm{\scriptsize 113}$,    
J.~Kroll$^\textrm{\scriptsize 137}$,    
J.~Kroll$^\textrm{\scriptsize 133}$,    
J.~Kroseberg$^\textrm{\scriptsize 24}$,    
J.~Krstic$^\textrm{\scriptsize 16}$,    
U.~Kruchonak$^\textrm{\scriptsize 77}$,    
H.~Kr\"uger$^\textrm{\scriptsize 24}$,    
N.~Krumnack$^\textrm{\scriptsize 76}$,    
M.C.~Kruse$^\textrm{\scriptsize 47}$,    
T.~Kubota$^\textrm{\scriptsize 102}$,    
S.~Kuday$^\textrm{\scriptsize 4b}$,    
J.T.~Kuechler$^\textrm{\scriptsize 180}$,    
S.~Kuehn$^\textrm{\scriptsize 35}$,    
A.~Kugel$^\textrm{\scriptsize 59a}$,    
F.~Kuger$^\textrm{\scriptsize 175}$,    
T.~Kuhl$^\textrm{\scriptsize 44}$,    
V.~Kukhtin$^\textrm{\scriptsize 77}$,    
R.~Kukla$^\textrm{\scriptsize 99}$,    
Y.~Kulchitsky$^\textrm{\scriptsize 105}$,    
S.~Kuleshov$^\textrm{\scriptsize 144b}$,    
Y.P.~Kulinich$^\textrm{\scriptsize 171}$,    
M.~Kuna$^\textrm{\scriptsize 56}$,    
T.~Kunigo$^\textrm{\scriptsize 83}$,    
A.~Kupco$^\textrm{\scriptsize 137}$,    
T.~Kupfer$^\textrm{\scriptsize 45}$,    
O.~Kuprash$^\textrm{\scriptsize 159}$,    
H.~Kurashige$^\textrm{\scriptsize 80}$,    
L.L.~Kurchaninov$^\textrm{\scriptsize 166a}$,    
Y.A.~Kurochkin$^\textrm{\scriptsize 105}$,    
M.G.~Kurth$^\textrm{\scriptsize 15d}$,    
E.S.~Kuwertz$^\textrm{\scriptsize 174}$,    
M.~Kuze$^\textrm{\scriptsize 163}$,    
J.~Kvita$^\textrm{\scriptsize 126}$,    
T.~Kwan$^\textrm{\scriptsize 174}$,    
A.~La~Rosa$^\textrm{\scriptsize 113}$,    
J.L.~La~Rosa~Navarro$^\textrm{\scriptsize 78d}$,    
L.~La~Rotonda$^\textrm{\scriptsize 40b,40a}$,    
F.~La~Ruffa$^\textrm{\scriptsize 40b,40a}$,    
C.~Lacasta$^\textrm{\scriptsize 172}$,    
F.~Lacava$^\textrm{\scriptsize 70a,70b}$,    
J.~Lacey$^\textrm{\scriptsize 44}$,    
D.P.J.~Lack$^\textrm{\scriptsize 98}$,    
H.~Lacker$^\textrm{\scriptsize 19}$,    
D.~Lacour$^\textrm{\scriptsize 132}$,    
E.~Ladygin$^\textrm{\scriptsize 77}$,    
R.~Lafaye$^\textrm{\scriptsize 5}$,    
B.~Laforge$^\textrm{\scriptsize 132}$,    
S.~Lai$^\textrm{\scriptsize 51}$,    
S.~Lammers$^\textrm{\scriptsize 63}$,    
W.~Lampl$^\textrm{\scriptsize 7}$,    
E.~Lan\c{c}on$^\textrm{\scriptsize 29}$,    
U.~Landgraf$^\textrm{\scriptsize 50}$,    
M.P.J.~Landon$^\textrm{\scriptsize 90}$,    
M.C.~Lanfermann$^\textrm{\scriptsize 52}$,    
V.S.~Lang$^\textrm{\scriptsize 44}$,    
J.C.~Lange$^\textrm{\scriptsize 14}$,    
R.J.~Langenberg$^\textrm{\scriptsize 35}$,    
A.J.~Lankford$^\textrm{\scriptsize 169}$,    
F.~Lanni$^\textrm{\scriptsize 29}$,    
K.~Lantzsch$^\textrm{\scriptsize 24}$,    
A.~Lanza$^\textrm{\scriptsize 68a}$,    
A.~Lapertosa$^\textrm{\scriptsize 53b,53a}$,    
S.~Laplace$^\textrm{\scriptsize 132}$,    
J.F.~Laporte$^\textrm{\scriptsize 142}$,    
T.~Lari$^\textrm{\scriptsize 66a}$,    
F.~Lasagni~Manghi$^\textrm{\scriptsize 23b,23a}$,    
M.~Lassnig$^\textrm{\scriptsize 35}$,    
T.S.~Lau$^\textrm{\scriptsize 61a}$,    
A.~Laudrain$^\textrm{\scriptsize 128}$,    
A.T.~Law$^\textrm{\scriptsize 143}$,    
P.~Laycock$^\textrm{\scriptsize 88}$,    
M.~Lazzaroni$^\textrm{\scriptsize 66a,66b}$,    
B.~Le$^\textrm{\scriptsize 102}$,    
O.~Le~Dortz$^\textrm{\scriptsize 132}$,    
E.~Le~Guirriec$^\textrm{\scriptsize 99}$,    
E.P.~Le~Quilleuc$^\textrm{\scriptsize 142}$,    
M.~LeBlanc$^\textrm{\scriptsize 7}$,    
T.~LeCompte$^\textrm{\scriptsize 6}$,    
F.~Ledroit-Guillon$^\textrm{\scriptsize 56}$,    
C.A.~Lee$^\textrm{\scriptsize 29}$,    
G.R.~Lee$^\textrm{\scriptsize 144a}$,    
L.~Lee$^\textrm{\scriptsize 57}$,    
S.C.~Lee$^\textrm{\scriptsize 155}$,    
B.~Lefebvre$^\textrm{\scriptsize 101}$,    
M.~Lefebvre$^\textrm{\scriptsize 174}$,    
F.~Legger$^\textrm{\scriptsize 112}$,    
C.~Leggett$^\textrm{\scriptsize 18}$,    
G.~Lehmann~Miotto$^\textrm{\scriptsize 35}$,    
W.A.~Leight$^\textrm{\scriptsize 44}$,    
A.~Leisos$^\textrm{\scriptsize 160,y}$,    
M.A.L.~Leite$^\textrm{\scriptsize 78d}$,    
R.~Leitner$^\textrm{\scriptsize 139}$,    
D.~Lellouch$^\textrm{\scriptsize 178}$,    
B.~Lemmer$^\textrm{\scriptsize 51}$,    
K.J.C.~Leney$^\textrm{\scriptsize 92}$,    
T.~Lenz$^\textrm{\scriptsize 24}$,    
B.~Lenzi$^\textrm{\scriptsize 35}$,    
R.~Leone$^\textrm{\scriptsize 7}$,    
S.~Leone$^\textrm{\scriptsize 69a}$,    
C.~Leonidopoulos$^\textrm{\scriptsize 48}$,    
G.~Lerner$^\textrm{\scriptsize 153}$,    
C.~Leroy$^\textrm{\scriptsize 107}$,    
R.~Les$^\textrm{\scriptsize 165}$,    
A.A.J.~Lesage$^\textrm{\scriptsize 142}$,    
C.G.~Lester$^\textrm{\scriptsize 31}$,    
M.~Levchenko$^\textrm{\scriptsize 134}$,    
J.~Lev\^eque$^\textrm{\scriptsize 5}$,    
D.~Levin$^\textrm{\scriptsize 103}$,    
L.J.~Levinson$^\textrm{\scriptsize 178}$,    
M.~Levy$^\textrm{\scriptsize 21}$,    
D.~Lewis$^\textrm{\scriptsize 90}$,    
B.~Li$^\textrm{\scriptsize 58a,u}$,    
C-Q.~Li$^\textrm{\scriptsize 58a,am}$,    
H.~Li$^\textrm{\scriptsize 58b}$,    
L.~Li$^\textrm{\scriptsize 58c}$,    
Q.~Li$^\textrm{\scriptsize 15d}$,    
Q.Y.~Li$^\textrm{\scriptsize 58a}$,    
S.~Li$^\textrm{\scriptsize 58d,58c}$,    
X.~Li$^\textrm{\scriptsize 58c}$,    
Y.~Li$^\textrm{\scriptsize 148}$,    
Z.~Liang$^\textrm{\scriptsize 15a}$,    
B.~Liberti$^\textrm{\scriptsize 71a}$,    
A.~Liblong$^\textrm{\scriptsize 165}$,    
K.~Lie$^\textrm{\scriptsize 61c}$,    
A.~Limosani$^\textrm{\scriptsize 154}$,    
C.Y.~Lin$^\textrm{\scriptsize 31}$,    
K.~Lin$^\textrm{\scriptsize 104}$,    
S.C.~Lin$^\textrm{\scriptsize 156}$,    
T.H.~Lin$^\textrm{\scriptsize 97}$,    
R.A.~Linck$^\textrm{\scriptsize 63}$,    
B.E.~Lindquist$^\textrm{\scriptsize 152}$,    
A.L.~Lionti$^\textrm{\scriptsize 52}$,    
E.~Lipeles$^\textrm{\scriptsize 133}$,    
A.~Lipniacka$^\textrm{\scriptsize 17}$,    
M.~Lisovyi$^\textrm{\scriptsize 59b}$,    
T.M.~Liss$^\textrm{\scriptsize 171,au}$,    
A.~Lister$^\textrm{\scriptsize 173}$,    
A.M.~Litke$^\textrm{\scriptsize 143}$,    
J.D.~Little$^\textrm{\scriptsize 8}$,    
B.~Liu$^\textrm{\scriptsize 76}$,    
B.L~Liu$^\textrm{\scriptsize 6}$,    
H.B.~Liu$^\textrm{\scriptsize 29}$,    
H.~Liu$^\textrm{\scriptsize 103}$,    
J.B.~Liu$^\textrm{\scriptsize 58a}$,    
J.K.K.~Liu$^\textrm{\scriptsize 131}$,    
K.~Liu$^\textrm{\scriptsize 132}$,    
M.~Liu$^\textrm{\scriptsize 58a}$,    
P.~Liu$^\textrm{\scriptsize 18}$,    
Y.L.~Liu$^\textrm{\scriptsize 58a}$,    
Y.W.~Liu$^\textrm{\scriptsize 58a}$,    
M.~Livan$^\textrm{\scriptsize 68a,68b}$,    
A.~Lleres$^\textrm{\scriptsize 56}$,    
J.~Llorente~Merino$^\textrm{\scriptsize 15a}$,    
S.L.~Lloyd$^\textrm{\scriptsize 90}$,    
C.Y.~Lo$^\textrm{\scriptsize 61b}$,    
F.~Lo~Sterzo$^\textrm{\scriptsize 41}$,    
E.M.~Lobodzinska$^\textrm{\scriptsize 44}$,    
P.~Loch$^\textrm{\scriptsize 7}$,    
F.K.~Loebinger$^\textrm{\scriptsize 98}$,    
K.M.~Loew$^\textrm{\scriptsize 26}$,    
T.~Lohse$^\textrm{\scriptsize 19}$,    
K.~Lohwasser$^\textrm{\scriptsize 146}$,    
M.~Lokajicek$^\textrm{\scriptsize 137}$,    
B.A.~Long$^\textrm{\scriptsize 25}$,    
J.D.~Long$^\textrm{\scriptsize 171}$,    
R.E.~Long$^\textrm{\scriptsize 87}$,    
L.~Longo$^\textrm{\scriptsize 65a,65b}$,    
K.A.~Looper$^\textrm{\scriptsize 122}$,    
J.A.~Lopez$^\textrm{\scriptsize 144b}$,    
I.~Lopez~Paz$^\textrm{\scriptsize 14}$,    
A.~Lopez~Solis$^\textrm{\scriptsize 132}$,    
J.~Lorenz$^\textrm{\scriptsize 112}$,    
N.~Lorenzo~Martinez$^\textrm{\scriptsize 5}$,    
M.~Losada$^\textrm{\scriptsize 22}$,    
P.J.~L{\"o}sel$^\textrm{\scriptsize 112}$,    
A.~L\"osle$^\textrm{\scriptsize 50}$,    
X.~Lou$^\textrm{\scriptsize 44}$,    
X.~Lou$^\textrm{\scriptsize 15a}$,    
A.~Lounis$^\textrm{\scriptsize 128}$,    
J.~Love$^\textrm{\scriptsize 6}$,    
P.A.~Love$^\textrm{\scriptsize 87}$,    
H.~Lu$^\textrm{\scriptsize 61a}$,    
N.~Lu$^\textrm{\scriptsize 103}$,    
Y.J.~Lu$^\textrm{\scriptsize 62}$,    
H.J.~Lubatti$^\textrm{\scriptsize 145}$,    
C.~Luci$^\textrm{\scriptsize 70a,70b}$,    
A.~Lucotte$^\textrm{\scriptsize 56}$,    
C.~Luedtke$^\textrm{\scriptsize 50}$,    
F.~Luehring$^\textrm{\scriptsize 63}$,    
I.~Luise$^\textrm{\scriptsize 132}$,    
W.~Lukas$^\textrm{\scriptsize 74}$,    
L.~Luminari$^\textrm{\scriptsize 70a}$,    
B.~Lund-Jensen$^\textrm{\scriptsize 151}$,    
M.S.~Lutz$^\textrm{\scriptsize 100}$,    
P.M.~Luzi$^\textrm{\scriptsize 132}$,    
D.~Lynn$^\textrm{\scriptsize 29}$,    
R.~Lysak$^\textrm{\scriptsize 137}$,    
E.~Lytken$^\textrm{\scriptsize 94}$,    
F.~Lyu$^\textrm{\scriptsize 15a}$,    
V.~Lyubushkin$^\textrm{\scriptsize 77}$,    
H.~Ma$^\textrm{\scriptsize 29}$,    
L.L.~Ma$^\textrm{\scriptsize 58b}$,    
Y.~Ma$^\textrm{\scriptsize 58b}$,    
G.~Maccarrone$^\textrm{\scriptsize 49}$,    
A.~Macchiolo$^\textrm{\scriptsize 113}$,    
C.M.~Macdonald$^\textrm{\scriptsize 146}$,    
J.~Machado~Miguens$^\textrm{\scriptsize 133,136b}$,    
D.~Madaffari$^\textrm{\scriptsize 172}$,    
R.~Madar$^\textrm{\scriptsize 37}$,    
W.F.~Mader$^\textrm{\scriptsize 46}$,    
A.~Madsen$^\textrm{\scriptsize 44}$,    
N.~Madysa$^\textrm{\scriptsize 46}$,    
J.~Maeda$^\textrm{\scriptsize 80}$,    
S.~Maeland$^\textrm{\scriptsize 17}$,    
T.~Maeno$^\textrm{\scriptsize 29}$,    
A.S.~Maevskiy$^\textrm{\scriptsize 111}$,    
V.~Magerl$^\textrm{\scriptsize 50}$,    
C.~Maidantchik$^\textrm{\scriptsize 78b}$,    
T.~Maier$^\textrm{\scriptsize 112}$,    
A.~Maio$^\textrm{\scriptsize 136a,136b,136d}$,    
O.~Majersky$^\textrm{\scriptsize 28a}$,    
S.~Majewski$^\textrm{\scriptsize 127}$,    
Y.~Makida$^\textrm{\scriptsize 79}$,    
N.~Makovec$^\textrm{\scriptsize 128}$,    
B.~Malaescu$^\textrm{\scriptsize 132}$,    
Pa.~Malecki$^\textrm{\scriptsize 82}$,    
V.P.~Maleev$^\textrm{\scriptsize 134}$,    
F.~Malek$^\textrm{\scriptsize 56}$,    
U.~Mallik$^\textrm{\scriptsize 75}$,    
D.~Malon$^\textrm{\scriptsize 6}$,    
C.~Malone$^\textrm{\scriptsize 31}$,    
S.~Maltezos$^\textrm{\scriptsize 10}$,    
S.~Malyukov$^\textrm{\scriptsize 35}$,    
J.~Mamuzic$^\textrm{\scriptsize 172}$,    
G.~Mancini$^\textrm{\scriptsize 49}$,    
I.~Mandi\'{c}$^\textrm{\scriptsize 89}$,    
J.~Maneira$^\textrm{\scriptsize 136a}$,    
L.~Manhaes~de~Andrade~Filho$^\textrm{\scriptsize 78a}$,    
J.~Manjarres~Ramos$^\textrm{\scriptsize 46}$,    
K.H.~Mankinen$^\textrm{\scriptsize 94}$,    
A.~Mann$^\textrm{\scriptsize 112}$,    
A.~Manousos$^\textrm{\scriptsize 74}$,    
B.~Mansoulie$^\textrm{\scriptsize 142}$,    
J.D.~Mansour$^\textrm{\scriptsize 15a}$,    
R.~Mantifel$^\textrm{\scriptsize 101}$,    
M.~Mantoani$^\textrm{\scriptsize 51}$,    
S.~Manzoni$^\textrm{\scriptsize 66a,66b}$,    
G.~Marceca$^\textrm{\scriptsize 30}$,    
L.~March$^\textrm{\scriptsize 52}$,    
L.~Marchese$^\textrm{\scriptsize 131}$,    
G.~Marchiori$^\textrm{\scriptsize 132}$,    
M.~Marcisovsky$^\textrm{\scriptsize 137}$,    
C.A.~Marin~Tobon$^\textrm{\scriptsize 35}$,    
M.~Marjanovic$^\textrm{\scriptsize 37}$,    
D.E.~Marley$^\textrm{\scriptsize 103}$,    
F.~Marroquim$^\textrm{\scriptsize 78b}$,    
Z.~Marshall$^\textrm{\scriptsize 18}$,    
M.U.F~Martensson$^\textrm{\scriptsize 170}$,    
S.~Marti-Garcia$^\textrm{\scriptsize 172}$,    
C.B.~Martin$^\textrm{\scriptsize 122}$,    
T.A.~Martin$^\textrm{\scriptsize 176}$,    
V.J.~Martin$^\textrm{\scriptsize 48}$,    
B.~Martin~dit~Latour$^\textrm{\scriptsize 17}$,    
M.~Martinez$^\textrm{\scriptsize 14,ab}$,    
V.I.~Martinez~Outschoorn$^\textrm{\scriptsize 100}$,    
S.~Martin-Haugh$^\textrm{\scriptsize 141}$,    
V.S.~Martoiu$^\textrm{\scriptsize 27b}$,    
A.C.~Martyniuk$^\textrm{\scriptsize 92}$,    
A.~Marzin$^\textrm{\scriptsize 35}$,    
L.~Masetti$^\textrm{\scriptsize 97}$,    
T.~Mashimo$^\textrm{\scriptsize 161}$,    
R.~Mashinistov$^\textrm{\scriptsize 108}$,    
J.~Masik$^\textrm{\scriptsize 98}$,    
A.L.~Maslennikov$^\textrm{\scriptsize 120b,120a}$,    
L.H.~Mason$^\textrm{\scriptsize 102}$,    
L.~Massa$^\textrm{\scriptsize 71a,71b}$,    
P.~Mastrandrea$^\textrm{\scriptsize 5}$,    
A.~Mastroberardino$^\textrm{\scriptsize 40b,40a}$,    
T.~Masubuchi$^\textrm{\scriptsize 161}$,    
P.~M\"attig$^\textrm{\scriptsize 180}$,    
J.~Maurer$^\textrm{\scriptsize 27b}$,    
B.~Ma\v{c}ek$^\textrm{\scriptsize 89}$,    
S.J.~Maxfield$^\textrm{\scriptsize 88}$,    
D.A.~Maximov$^\textrm{\scriptsize 120b,120a}$,    
R.~Mazini$^\textrm{\scriptsize 155}$,    
I.~Maznas$^\textrm{\scriptsize 160}$,    
S.M.~Mazza$^\textrm{\scriptsize 143}$,    
N.C.~Mc~Fadden$^\textrm{\scriptsize 116}$,    
G.~Mc~Goldrick$^\textrm{\scriptsize 165}$,    
S.P.~Mc~Kee$^\textrm{\scriptsize 103}$,    
A.~McCarn$^\textrm{\scriptsize 103}$,    
T.G.~McCarthy$^\textrm{\scriptsize 113}$,    
L.I.~McClymont$^\textrm{\scriptsize 92}$,    
E.F.~McDonald$^\textrm{\scriptsize 102}$,    
J.A.~Mcfayden$^\textrm{\scriptsize 35}$,    
G.~Mchedlidze$^\textrm{\scriptsize 51}$,    
M.A.~McKay$^\textrm{\scriptsize 41}$,    
S.J.~McMahon$^\textrm{\scriptsize 141}$,    
P.C.~McNamara$^\textrm{\scriptsize 102}$,    
C.J.~McNicol$^\textrm{\scriptsize 176}$,    
R.A.~McPherson$^\textrm{\scriptsize 174,ag}$,    
Z.A.~Meadows$^\textrm{\scriptsize 100}$,    
S.~Meehan$^\textrm{\scriptsize 145}$,    
T.M.~Megy$^\textrm{\scriptsize 50}$,    
S.~Mehlhase$^\textrm{\scriptsize 112}$,    
A.~Mehta$^\textrm{\scriptsize 88}$,    
T.~Meideck$^\textrm{\scriptsize 56}$,    
B.~Meirose$^\textrm{\scriptsize 42}$,    
D.~Melini$^\textrm{\scriptsize 172,i}$,    
B.R.~Mellado~Garcia$^\textrm{\scriptsize 32c}$,    
J.D.~Mellenthin$^\textrm{\scriptsize 51}$,    
M.~Melo$^\textrm{\scriptsize 28a}$,    
F.~Meloni$^\textrm{\scriptsize 20}$,    
A.~Melzer$^\textrm{\scriptsize 24}$,    
S.B.~Menary$^\textrm{\scriptsize 98}$,    
L.~Meng$^\textrm{\scriptsize 88}$,    
X.T.~Meng$^\textrm{\scriptsize 103}$,    
A.~Mengarelli$^\textrm{\scriptsize 23b,23a}$,    
S.~Menke$^\textrm{\scriptsize 113}$,    
E.~Meoni$^\textrm{\scriptsize 40b,40a}$,    
S.~Mergelmeyer$^\textrm{\scriptsize 19}$,    
C.~Merlassino$^\textrm{\scriptsize 20}$,    
P.~Mermod$^\textrm{\scriptsize 52}$,    
L.~Merola$^\textrm{\scriptsize 67a,67b}$,    
C.~Meroni$^\textrm{\scriptsize 66a}$,    
F.S.~Merritt$^\textrm{\scriptsize 36}$,    
A.~Messina$^\textrm{\scriptsize 70a,70b}$,    
J.~Metcalfe$^\textrm{\scriptsize 6}$,    
A.S.~Mete$^\textrm{\scriptsize 169}$,    
C.~Meyer$^\textrm{\scriptsize 133}$,    
J.~Meyer$^\textrm{\scriptsize 158}$,    
J-P.~Meyer$^\textrm{\scriptsize 142}$,    
H.~Meyer~Zu~Theenhausen$^\textrm{\scriptsize 59a}$,    
F.~Miano$^\textrm{\scriptsize 153}$,    
R.P.~Middleton$^\textrm{\scriptsize 141}$,    
S.~Miglioranzi$^\textrm{\scriptsize 53b,53a}$,    
L.~Mijovi\'{c}$^\textrm{\scriptsize 48}$,    
G.~Mikenberg$^\textrm{\scriptsize 178}$,    
M.~Mikestikova$^\textrm{\scriptsize 137}$,    
M.~Miku\v{z}$^\textrm{\scriptsize 89}$,    
M.~Milesi$^\textrm{\scriptsize 102}$,    
A.~Milic$^\textrm{\scriptsize 165}$,    
D.A.~Millar$^\textrm{\scriptsize 90}$,    
D.W.~Miller$^\textrm{\scriptsize 36}$,    
A.~Milov$^\textrm{\scriptsize 178}$,    
D.A.~Milstead$^\textrm{\scriptsize 43a,43b}$,    
A.A.~Minaenko$^\textrm{\scriptsize 140}$,    
I.A.~Minashvili$^\textrm{\scriptsize 157b}$,    
A.I.~Mincer$^\textrm{\scriptsize 121}$,    
B.~Mindur$^\textrm{\scriptsize 81a}$,    
M.~Mineev$^\textrm{\scriptsize 77}$,    
Y.~Minegishi$^\textrm{\scriptsize 161}$,    
Y.~Ming$^\textrm{\scriptsize 179}$,    
L.M.~Mir$^\textrm{\scriptsize 14}$,    
A.~Mirto$^\textrm{\scriptsize 65a,65b}$,    
K.P.~Mistry$^\textrm{\scriptsize 133}$,    
T.~Mitani$^\textrm{\scriptsize 177}$,    
J.~Mitrevski$^\textrm{\scriptsize 112}$,    
V.A.~Mitsou$^\textrm{\scriptsize 172}$,    
A.~Miucci$^\textrm{\scriptsize 20}$,    
P.S.~Miyagawa$^\textrm{\scriptsize 146}$,    
A.~Mizukami$^\textrm{\scriptsize 79}$,    
J.U.~Mj\"ornmark$^\textrm{\scriptsize 94}$,    
T.~Mkrtchyan$^\textrm{\scriptsize 182}$,    
M.~Mlynarikova$^\textrm{\scriptsize 139}$,    
T.~Moa$^\textrm{\scriptsize 43a,43b}$,    
K.~Mochizuki$^\textrm{\scriptsize 107}$,    
P.~Mogg$^\textrm{\scriptsize 50}$,    
S.~Mohapatra$^\textrm{\scriptsize 38}$,    
S.~Molander$^\textrm{\scriptsize 43a,43b}$,    
R.~Moles-Valls$^\textrm{\scriptsize 24}$,    
M.C.~Mondragon$^\textrm{\scriptsize 104}$,    
K.~M\"onig$^\textrm{\scriptsize 44}$,    
J.~Monk$^\textrm{\scriptsize 39}$,    
E.~Monnier$^\textrm{\scriptsize 99}$,    
A.~Montalbano$^\textrm{\scriptsize 149}$,    
J.~Montejo~Berlingen$^\textrm{\scriptsize 35}$,    
F.~Monticelli$^\textrm{\scriptsize 86}$,    
S.~Monzani$^\textrm{\scriptsize 66a}$,    
R.W.~Moore$^\textrm{\scriptsize 3}$,    
N.~Morange$^\textrm{\scriptsize 128}$,    
D.~Moreno$^\textrm{\scriptsize 22}$,    
M.~Moreno~Ll\'acer$^\textrm{\scriptsize 35}$,    
P.~Morettini$^\textrm{\scriptsize 53b}$,    
M.~Morgenstern$^\textrm{\scriptsize 118}$,    
S.~Morgenstern$^\textrm{\scriptsize 35}$,    
D.~Mori$^\textrm{\scriptsize 149}$,    
T.~Mori$^\textrm{\scriptsize 161}$,    
M.~Morii$^\textrm{\scriptsize 57}$,    
M.~Morinaga$^\textrm{\scriptsize 177}$,    
V.~Morisbak$^\textrm{\scriptsize 130}$,    
A.K.~Morley$^\textrm{\scriptsize 35}$,    
G.~Mornacchi$^\textrm{\scriptsize 35}$,    
J.D.~Morris$^\textrm{\scriptsize 90}$,    
L.~Morvaj$^\textrm{\scriptsize 152}$,    
P.~Moschovakos$^\textrm{\scriptsize 10}$,    
M.~Mosidze$^\textrm{\scriptsize 157b}$,    
H.J.~Moss$^\textrm{\scriptsize 146}$,    
J.~Moss$^\textrm{\scriptsize 150,o}$,    
K.~Motohashi$^\textrm{\scriptsize 163}$,    
R.~Mount$^\textrm{\scriptsize 150}$,    
E.~Mountricha$^\textrm{\scriptsize 29}$,    
E.J.W.~Moyse$^\textrm{\scriptsize 100}$,    
S.~Muanza$^\textrm{\scriptsize 99}$,    
F.~Mueller$^\textrm{\scriptsize 113}$,    
J.~Mueller$^\textrm{\scriptsize 135}$,    
R.S.P.~Mueller$^\textrm{\scriptsize 112}$,    
D.~Muenstermann$^\textrm{\scriptsize 87}$,    
P.~Mullen$^\textrm{\scriptsize 55}$,    
G.A.~Mullier$^\textrm{\scriptsize 20}$,    
F.J.~Munoz~Sanchez$^\textrm{\scriptsize 98}$,    
P.~Murin$^\textrm{\scriptsize 28b}$,    
W.J.~Murray$^\textrm{\scriptsize 176,141}$,    
A.~Murrone$^\textrm{\scriptsize 66a,66b}$,    
M.~Mu\v{s}kinja$^\textrm{\scriptsize 89}$,    
C.~Mwewa$^\textrm{\scriptsize 32a}$,    
A.G.~Myagkov$^\textrm{\scriptsize 140,ao}$,    
J.~Myers$^\textrm{\scriptsize 127}$,    
M.~Myska$^\textrm{\scriptsize 138}$,    
B.P.~Nachman$^\textrm{\scriptsize 18}$,    
O.~Nackenhorst$^\textrm{\scriptsize 45}$,    
K.~Nagai$^\textrm{\scriptsize 131}$,    
R.~Nagai$^\textrm{\scriptsize 79,ar}$,    
K.~Nagano$^\textrm{\scriptsize 79}$,    
Y.~Nagasaka$^\textrm{\scriptsize 60}$,    
K.~Nagata$^\textrm{\scriptsize 167}$,    
M.~Nagel$^\textrm{\scriptsize 50}$,    
E.~Nagy$^\textrm{\scriptsize 99}$,    
A.M.~Nairz$^\textrm{\scriptsize 35}$,    
Y.~Nakahama$^\textrm{\scriptsize 115}$,    
K.~Nakamura$^\textrm{\scriptsize 79}$,    
T.~Nakamura$^\textrm{\scriptsize 161}$,    
I.~Nakano$^\textrm{\scriptsize 123}$,    
R.F.~Naranjo~Garcia$^\textrm{\scriptsize 44}$,    
R.~Narayan$^\textrm{\scriptsize 11}$,    
D.I.~Narrias~Villar$^\textrm{\scriptsize 59a}$,    
I.~Naryshkin$^\textrm{\scriptsize 134}$,    
T.~Naumann$^\textrm{\scriptsize 44}$,    
G.~Navarro$^\textrm{\scriptsize 22}$,    
R.~Nayyar$^\textrm{\scriptsize 7}$,    
H.A.~Neal$^\textrm{\scriptsize 103,*}$,    
P.Y.~Nechaeva$^\textrm{\scriptsize 108}$,    
T.J.~Neep$^\textrm{\scriptsize 142}$,    
A.~Negri$^\textrm{\scriptsize 68a,68b}$,    
M.~Negrini$^\textrm{\scriptsize 23b}$,    
S.~Nektarijevic$^\textrm{\scriptsize 117}$,    
C.~Nellist$^\textrm{\scriptsize 51}$,    
M.E.~Nelson$^\textrm{\scriptsize 131}$,    
S.~Nemecek$^\textrm{\scriptsize 137}$,    
P.~Nemethy$^\textrm{\scriptsize 121}$,    
M.~Nessi$^\textrm{\scriptsize 35,g}$,    
M.S.~Neubauer$^\textrm{\scriptsize 171}$,    
M.~Neumann$^\textrm{\scriptsize 180}$,    
P.R.~Newman$^\textrm{\scriptsize 21}$,    
T.Y.~Ng$^\textrm{\scriptsize 61c}$,    
Y.S.~Ng$^\textrm{\scriptsize 19}$,    
H.D.N.~Nguyen$^\textrm{\scriptsize 99}$,    
T.~Nguyen~Manh$^\textrm{\scriptsize 107}$,    
E.~Nibigira$^\textrm{\scriptsize 37}$,    
R.B.~Nickerson$^\textrm{\scriptsize 131}$,    
R.~Nicolaidou$^\textrm{\scriptsize 142}$,    
J.~Nielsen$^\textrm{\scriptsize 143}$,    
N.~Nikiforou$^\textrm{\scriptsize 11}$,    
V.~Nikolaenko$^\textrm{\scriptsize 140,ao}$,    
I.~Nikolic-Audit$^\textrm{\scriptsize 132}$,    
K.~Nikolopoulos$^\textrm{\scriptsize 21}$,    
P.~Nilsson$^\textrm{\scriptsize 29}$,    
Y.~Ninomiya$^\textrm{\scriptsize 79}$,    
A.~Nisati$^\textrm{\scriptsize 70a}$,    
N.~Nishu$^\textrm{\scriptsize 58c}$,    
R.~Nisius$^\textrm{\scriptsize 113}$,    
I.~Nitsche$^\textrm{\scriptsize 45}$,    
T.~Nitta$^\textrm{\scriptsize 177}$,    
T.~Nobe$^\textrm{\scriptsize 161}$,    
Y.~Noguchi$^\textrm{\scriptsize 83}$,    
M.~Nomachi$^\textrm{\scriptsize 129}$,    
I.~Nomidis$^\textrm{\scriptsize 33}$,    
M.A.~Nomura$^\textrm{\scriptsize 29}$,    
T.~Nooney$^\textrm{\scriptsize 90}$,    
M.~Nordberg$^\textrm{\scriptsize 35}$,    
N.~Norjoharuddeen$^\textrm{\scriptsize 131}$,    
T.~Novak$^\textrm{\scriptsize 89}$,    
O.~Novgorodova$^\textrm{\scriptsize 46}$,    
R.~Novotny$^\textrm{\scriptsize 138}$,    
M.~Nozaki$^\textrm{\scriptsize 79}$,    
L.~Nozka$^\textrm{\scriptsize 126}$,    
K.~Ntekas$^\textrm{\scriptsize 169}$,    
E.~Nurse$^\textrm{\scriptsize 92}$,    
F.~Nuti$^\textrm{\scriptsize 102}$,    
F.G.~Oakham$^\textrm{\scriptsize 33,ax}$,    
H.~Oberlack$^\textrm{\scriptsize 113}$,    
T.~Obermann$^\textrm{\scriptsize 24}$,    
J.~Ocariz$^\textrm{\scriptsize 132}$,    
A.~Ochi$^\textrm{\scriptsize 80}$,    
I.~Ochoa$^\textrm{\scriptsize 38}$,    
J.P.~Ochoa-Ricoux$^\textrm{\scriptsize 144a}$,    
K.~O'Connor$^\textrm{\scriptsize 26}$,    
S.~Oda$^\textrm{\scriptsize 85}$,    
S.~Odaka$^\textrm{\scriptsize 79}$,    
A.~Oh$^\textrm{\scriptsize 98}$,    
S.H.~Oh$^\textrm{\scriptsize 47}$,    
C.C.~Ohm$^\textrm{\scriptsize 151}$,    
H.~Ohman$^\textrm{\scriptsize 170}$,    
H.~Oide$^\textrm{\scriptsize 53b,53a}$,    
H.~Okawa$^\textrm{\scriptsize 167}$,    
Y.~Okumura$^\textrm{\scriptsize 161}$,    
T.~Okuyama$^\textrm{\scriptsize 79}$,    
A.~Olariu$^\textrm{\scriptsize 27b}$,    
L.F.~Oleiro~Seabra$^\textrm{\scriptsize 136a}$,    
S.A.~Olivares~Pino$^\textrm{\scriptsize 144a}$,    
D.~Oliveira~Damazio$^\textrm{\scriptsize 29}$,    
J.L.~Oliver$^\textrm{\scriptsize 1}$,    
M.J.R.~Olsson$^\textrm{\scriptsize 36}$,    
A.~Olszewski$^\textrm{\scriptsize 82}$,    
J.~Olszowska$^\textrm{\scriptsize 82}$,    
D.C.~O'Neil$^\textrm{\scriptsize 149}$,    
A.~Onofre$^\textrm{\scriptsize 136a,136e}$,    
K.~Onogi$^\textrm{\scriptsize 115}$,    
P.U.E.~Onyisi$^\textrm{\scriptsize 11}$,    
H.~Oppen$^\textrm{\scriptsize 130}$,    
M.J.~Oreglia$^\textrm{\scriptsize 36}$,    
Y.~Oren$^\textrm{\scriptsize 159}$,    
D.~Orestano$^\textrm{\scriptsize 72a,72b}$,    
E.C.~Orgill$^\textrm{\scriptsize 98}$,    
N.~Orlando$^\textrm{\scriptsize 61b}$,    
A.A.~O'Rourke$^\textrm{\scriptsize 44}$,    
R.S.~Orr$^\textrm{\scriptsize 165}$,    
B.~Osculati$^\textrm{\scriptsize 53b,53a,*}$,    
V.~O'Shea$^\textrm{\scriptsize 55}$,    
R.~Ospanov$^\textrm{\scriptsize 58a}$,    
G.~Otero~y~Garzon$^\textrm{\scriptsize 30}$,    
H.~Otono$^\textrm{\scriptsize 85}$,    
M.~Ouchrif$^\textrm{\scriptsize 34d}$,    
F.~Ould-Saada$^\textrm{\scriptsize 130}$,    
A.~Ouraou$^\textrm{\scriptsize 142}$,    
K.P.~Oussoren$^\textrm{\scriptsize 118}$,    
Q.~Ouyang$^\textrm{\scriptsize 15a}$,    
M.~Owen$^\textrm{\scriptsize 55}$,    
R.E.~Owen$^\textrm{\scriptsize 21}$,    
V.E.~Ozcan$^\textrm{\scriptsize 12c}$,    
N.~Ozturk$^\textrm{\scriptsize 8}$,    
K.~Pachal$^\textrm{\scriptsize 149}$,    
A.~Pacheco~Pages$^\textrm{\scriptsize 14}$,    
L.~Pacheco~Rodriguez$^\textrm{\scriptsize 142}$,    
C.~Padilla~Aranda$^\textrm{\scriptsize 14}$,    
S.~Pagan~Griso$^\textrm{\scriptsize 18}$,    
M.~Paganini$^\textrm{\scriptsize 181}$,    
G.~Palacino$^\textrm{\scriptsize 63}$,    
S.~Palazzo$^\textrm{\scriptsize 40b,40a}$,    
S.~Palestini$^\textrm{\scriptsize 35}$,    
M.~Palka$^\textrm{\scriptsize 81b}$,    
D.~Pallin$^\textrm{\scriptsize 37}$,    
E.St.~Panagiotopoulou$^\textrm{\scriptsize 10}$,    
I.~Panagoulias$^\textrm{\scriptsize 10}$,    
C.E.~Pandini$^\textrm{\scriptsize 52}$,    
J.G.~Panduro~Vazquez$^\textrm{\scriptsize 91}$,    
P.~Pani$^\textrm{\scriptsize 35}$,    
D.~Pantea$^\textrm{\scriptsize 27b}$,    
L.~Paolozzi$^\textrm{\scriptsize 52}$,    
T.D.~Papadopoulou$^\textrm{\scriptsize 10}$,    
K.~Papageorgiou$^\textrm{\scriptsize 9,k}$,    
A.~Paramonov$^\textrm{\scriptsize 6}$,    
D.~Paredes~Hernandez$^\textrm{\scriptsize 61b}$,    
B.~Parida$^\textrm{\scriptsize 58c}$,    
A.J.~Parker$^\textrm{\scriptsize 87}$,    
K.A.~Parker$^\textrm{\scriptsize 44}$,    
M.A.~Parker$^\textrm{\scriptsize 31}$,    
F.~Parodi$^\textrm{\scriptsize 53b,53a}$,    
J.A.~Parsons$^\textrm{\scriptsize 38}$,    
U.~Parzefall$^\textrm{\scriptsize 50}$,    
V.R.~Pascuzzi$^\textrm{\scriptsize 165}$,    
J.M.P.~Pasner$^\textrm{\scriptsize 143}$,    
E.~Pasqualucci$^\textrm{\scriptsize 70a}$,    
S.~Passaggio$^\textrm{\scriptsize 53b}$,    
F.~Pastore$^\textrm{\scriptsize 91}$,    
P.~Pasuwan$^\textrm{\scriptsize 43a,43b}$,    
S.~Pataraia$^\textrm{\scriptsize 97}$,    
J.R.~Pater$^\textrm{\scriptsize 98}$,    
A.~Pathak$^\textrm{\scriptsize 179,l}$,    
T.~Pauly$^\textrm{\scriptsize 35}$,    
B.~Pearson$^\textrm{\scriptsize 113}$,    
S.~Pedraza~Lopez$^\textrm{\scriptsize 172}$,    
R.~Pedro$^\textrm{\scriptsize 136a,136b}$,    
S.V.~Peleganchuk$^\textrm{\scriptsize 120b,120a}$,    
O.~Penc$^\textrm{\scriptsize 137}$,    
C.~Peng$^\textrm{\scriptsize 15d}$,    
H.~Peng$^\textrm{\scriptsize 58a}$,    
J.~Penwell$^\textrm{\scriptsize 63}$,    
B.S.~Peralva$^\textrm{\scriptsize 78a}$,    
M.M.~Perego$^\textrm{\scriptsize 142}$,    
A.P.~Pereira~Peixoto$^\textrm{\scriptsize 136a}$,    
D.V.~Perepelitsa$^\textrm{\scriptsize 29}$,    
F.~Peri$^\textrm{\scriptsize 19}$,    
L.~Perini$^\textrm{\scriptsize 66a,66b}$,    
H.~Pernegger$^\textrm{\scriptsize 35}$,    
S.~Perrella$^\textrm{\scriptsize 67a,67b}$,    
V.D.~Peshekhonov$^\textrm{\scriptsize 77,*}$,    
K.~Peters$^\textrm{\scriptsize 44}$,    
R.F.Y.~Peters$^\textrm{\scriptsize 98}$,    
B.A.~Petersen$^\textrm{\scriptsize 35}$,    
T.C.~Petersen$^\textrm{\scriptsize 39}$,    
E.~Petit$^\textrm{\scriptsize 56}$,    
A.~Petridis$^\textrm{\scriptsize 1}$,    
C.~Petridou$^\textrm{\scriptsize 160}$,    
P.~Petroff$^\textrm{\scriptsize 128}$,    
E.~Petrolo$^\textrm{\scriptsize 70a}$,    
M.~Petrov$^\textrm{\scriptsize 131}$,    
F.~Petrucci$^\textrm{\scriptsize 72a,72b}$,    
N.E.~Pettersson$^\textrm{\scriptsize 100}$,    
A.~Peyaud$^\textrm{\scriptsize 142}$,    
R.~Pezoa$^\textrm{\scriptsize 144b}$,    
T.~Pham$^\textrm{\scriptsize 102}$,    
F.H.~Phillips$^\textrm{\scriptsize 104}$,    
P.W.~Phillips$^\textrm{\scriptsize 141}$,    
G.~Piacquadio$^\textrm{\scriptsize 152}$,    
E.~Pianori$^\textrm{\scriptsize 176}$,    
A.~Picazio$^\textrm{\scriptsize 100}$,    
M.A.~Pickering$^\textrm{\scriptsize 131}$,    
R.~Piegaia$^\textrm{\scriptsize 30}$,    
J.E.~Pilcher$^\textrm{\scriptsize 36}$,    
A.D.~Pilkington$^\textrm{\scriptsize 98}$,    
M.~Pinamonti$^\textrm{\scriptsize 71a,71b}$,    
J.L.~Pinfold$^\textrm{\scriptsize 3}$,    
M.~Pitt$^\textrm{\scriptsize 178}$,    
M.-A.~Pleier$^\textrm{\scriptsize 29}$,    
V.~Pleskot$^\textrm{\scriptsize 139}$,    
E.~Plotnikova$^\textrm{\scriptsize 77}$,    
D.~Pluth$^\textrm{\scriptsize 76}$,    
P.~Podberezko$^\textrm{\scriptsize 120b,120a}$,    
R.~Poettgen$^\textrm{\scriptsize 94}$,    
R.~Poggi$^\textrm{\scriptsize 68a,68b}$,    
L.~Poggioli$^\textrm{\scriptsize 128}$,    
I.~Pogrebnyak$^\textrm{\scriptsize 104}$,    
D.~Pohl$^\textrm{\scriptsize 24}$,    
I.~Pokharel$^\textrm{\scriptsize 51}$,    
G.~Polesello$^\textrm{\scriptsize 68a}$,    
A.~Poley$^\textrm{\scriptsize 44}$,    
A.~Policicchio$^\textrm{\scriptsize 40b,40a}$,    
R.~Polifka$^\textrm{\scriptsize 35}$,    
A.~Polini$^\textrm{\scriptsize 23b}$,    
C.S.~Pollard$^\textrm{\scriptsize 44}$,    
V.~Polychronakos$^\textrm{\scriptsize 29}$,    
D.~Ponomarenko$^\textrm{\scriptsize 110}$,    
L.~Pontecorvo$^\textrm{\scriptsize 70a}$,    
G.A.~Popeneciu$^\textrm{\scriptsize 27d}$,    
D.M.~Portillo~Quintero$^\textrm{\scriptsize 132}$,    
S.~Pospisil$^\textrm{\scriptsize 138}$,    
K.~Potamianos$^\textrm{\scriptsize 44}$,    
I.N.~Potrap$^\textrm{\scriptsize 77}$,    
C.J.~Potter$^\textrm{\scriptsize 31}$,    
H.~Potti$^\textrm{\scriptsize 11}$,    
T.~Poulsen$^\textrm{\scriptsize 94}$,    
J.~Poveda$^\textrm{\scriptsize 35}$,    
M.E.~Pozo~Astigarraga$^\textrm{\scriptsize 35}$,    
P.~Pralavorio$^\textrm{\scriptsize 99}$,    
S.~Prell$^\textrm{\scriptsize 76}$,    
D.~Price$^\textrm{\scriptsize 98}$,    
M.~Primavera$^\textrm{\scriptsize 65a}$,    
S.~Prince$^\textrm{\scriptsize 101}$,    
N.~Proklova$^\textrm{\scriptsize 110}$,    
K.~Prokofiev$^\textrm{\scriptsize 61c}$,    
F.~Prokoshin$^\textrm{\scriptsize 144b}$,    
S.~Protopopescu$^\textrm{\scriptsize 29}$,    
J.~Proudfoot$^\textrm{\scriptsize 6}$,    
M.~Przybycien$^\textrm{\scriptsize 81a}$,    
A.~Puri$^\textrm{\scriptsize 171}$,    
P.~Puzo$^\textrm{\scriptsize 128}$,    
J.~Qian$^\textrm{\scriptsize 103}$,    
Y.~Qin$^\textrm{\scriptsize 98}$,    
A.~Quadt$^\textrm{\scriptsize 51}$,    
M.~Queitsch-Maitland$^\textrm{\scriptsize 44}$,    
A.~Qureshi$^\textrm{\scriptsize 1}$,    
S.K.~Radhakrishnan$^\textrm{\scriptsize 152}$,    
P.~Rados$^\textrm{\scriptsize 102}$,    
F.~Ragusa$^\textrm{\scriptsize 66a,66b}$,    
G.~Rahal$^\textrm{\scriptsize 95}$,    
J.A.~Raine$^\textrm{\scriptsize 98}$,    
S.~Rajagopalan$^\textrm{\scriptsize 29}$,    
T.~Rashid$^\textrm{\scriptsize 128}$,    
S.~Raspopov$^\textrm{\scriptsize 5}$,    
M.G.~Ratti$^\textrm{\scriptsize 66a,66b}$,    
D.M.~Rauch$^\textrm{\scriptsize 44}$,    
F.~Rauscher$^\textrm{\scriptsize 112}$,    
S.~Rave$^\textrm{\scriptsize 97}$,    
B.~Ravina$^\textrm{\scriptsize 146}$,    
I.~Ravinovich$^\textrm{\scriptsize 178}$,    
J.H.~Rawling$^\textrm{\scriptsize 98}$,    
M.~Raymond$^\textrm{\scriptsize 35}$,    
A.L.~Read$^\textrm{\scriptsize 130}$,    
N.P.~Readioff$^\textrm{\scriptsize 56}$,    
M.~Reale$^\textrm{\scriptsize 65a,65b}$,    
D.M.~Rebuzzi$^\textrm{\scriptsize 68a,68b}$,    
A.~Redelbach$^\textrm{\scriptsize 175}$,    
G.~Redlinger$^\textrm{\scriptsize 29}$,    
R.~Reece$^\textrm{\scriptsize 143}$,    
R.G.~Reed$^\textrm{\scriptsize 32c}$,    
K.~Reeves$^\textrm{\scriptsize 42}$,    
L.~Rehnisch$^\textrm{\scriptsize 19}$,    
J.~Reichert$^\textrm{\scriptsize 133}$,    
A.~Reiss$^\textrm{\scriptsize 97}$,    
C.~Rembser$^\textrm{\scriptsize 35}$,    
H.~Ren$^\textrm{\scriptsize 15d}$,    
M.~Rescigno$^\textrm{\scriptsize 70a}$,    
S.~Resconi$^\textrm{\scriptsize 66a}$,    
E.D.~Resseguie$^\textrm{\scriptsize 133}$,    
S.~Rettie$^\textrm{\scriptsize 173}$,    
E.~Reynolds$^\textrm{\scriptsize 21}$,    
O.L.~Rezanova$^\textrm{\scriptsize 120b,120a}$,    
P.~Reznicek$^\textrm{\scriptsize 139}$,    
R.~Richter$^\textrm{\scriptsize 113}$,    
S.~Richter$^\textrm{\scriptsize 92}$,    
E.~Richter-Was$^\textrm{\scriptsize 81b}$,    
O.~Ricken$^\textrm{\scriptsize 24}$,    
M.~Ridel$^\textrm{\scriptsize 132}$,    
P.~Rieck$^\textrm{\scriptsize 113}$,    
C.J.~Riegel$^\textrm{\scriptsize 180}$,    
O.~Rifki$^\textrm{\scriptsize 44}$,    
M.~Rijssenbeek$^\textrm{\scriptsize 152}$,    
A.~Rimoldi$^\textrm{\scriptsize 68a,68b}$,    
M.~Rimoldi$^\textrm{\scriptsize 20}$,    
L.~Rinaldi$^\textrm{\scriptsize 23b}$,    
G.~Ripellino$^\textrm{\scriptsize 151}$,    
B.~Risti\'{c}$^\textrm{\scriptsize 35}$,    
E.~Ritsch$^\textrm{\scriptsize 35}$,    
I.~Riu$^\textrm{\scriptsize 14}$,    
J.C.~Rivera~Vergara$^\textrm{\scriptsize 144a}$,    
F.~Rizatdinova$^\textrm{\scriptsize 125}$,    
E.~Rizvi$^\textrm{\scriptsize 90}$,    
C.~Rizzi$^\textrm{\scriptsize 14}$,    
R.T.~Roberts$^\textrm{\scriptsize 98}$,    
S.H.~Robertson$^\textrm{\scriptsize 101,ag}$,    
A.~Robichaud-Veronneau$^\textrm{\scriptsize 101}$,    
D.~Robinson$^\textrm{\scriptsize 31}$,    
J.E.M.~Robinson$^\textrm{\scriptsize 44}$,    
A.~Robson$^\textrm{\scriptsize 55}$,    
E.~Rocco$^\textrm{\scriptsize 97}$,    
C.~Roda$^\textrm{\scriptsize 69a,69b}$,    
Y.~Rodina$^\textrm{\scriptsize 99,ac}$,    
S.~Rodriguez~Bosca$^\textrm{\scriptsize 172}$,    
A.~Rodriguez~Perez$^\textrm{\scriptsize 14}$,    
D.~Rodriguez~Rodriguez$^\textrm{\scriptsize 172}$,    
A.M.~Rodr\'iguez~Vera$^\textrm{\scriptsize 166b}$,    
S.~Roe$^\textrm{\scriptsize 35}$,    
C.S.~Rogan$^\textrm{\scriptsize 57}$,    
O.~R{\o}hne$^\textrm{\scriptsize 130}$,    
R.~R\"ohrig$^\textrm{\scriptsize 113}$,    
J.~Roloff$^\textrm{\scriptsize 57}$,    
A.~Romaniouk$^\textrm{\scriptsize 110}$,    
M.~Romano$^\textrm{\scriptsize 23b,23a}$,    
E.~Romero~Adam$^\textrm{\scriptsize 172}$,    
N.~Rompotis$^\textrm{\scriptsize 88}$,    
M.~Ronzani$^\textrm{\scriptsize 121}$,    
L.~Roos$^\textrm{\scriptsize 132}$,    
S.~Rosati$^\textrm{\scriptsize 70a}$,    
K.~Rosbach$^\textrm{\scriptsize 50}$,    
P.~Rose$^\textrm{\scriptsize 143}$,    
N-A.~Rosien$^\textrm{\scriptsize 51}$,    
E.~Rossi$^\textrm{\scriptsize 67a,67b}$,    
L.P.~Rossi$^\textrm{\scriptsize 53b}$,    
L.~Rossini$^\textrm{\scriptsize 66a,66b}$,    
J.H.N.~Rosten$^\textrm{\scriptsize 31}$,    
R.~Rosten$^\textrm{\scriptsize 145}$,    
M.~Rotaru$^\textrm{\scriptsize 27b}$,    
J.~Rothberg$^\textrm{\scriptsize 145}$,    
D.~Rousseau$^\textrm{\scriptsize 128}$,    
D.~Roy$^\textrm{\scriptsize 32c}$,    
A.~Rozanov$^\textrm{\scriptsize 99}$,    
Y.~Rozen$^\textrm{\scriptsize 158}$,    
X.~Ruan$^\textrm{\scriptsize 32c}$,    
F.~Rubbo$^\textrm{\scriptsize 150}$,    
F.~R\"uhr$^\textrm{\scriptsize 50}$,    
A.~Ruiz-Martinez$^\textrm{\scriptsize 33}$,    
Z.~Rurikova$^\textrm{\scriptsize 50}$,    
N.A.~Rusakovich$^\textrm{\scriptsize 77}$,    
H.L.~Russell$^\textrm{\scriptsize 101}$,    
J.P.~Rutherfoord$^\textrm{\scriptsize 7}$,    
N.~Ruthmann$^\textrm{\scriptsize 35}$,    
E.M.~R{\"u}ttinger$^\textrm{\scriptsize 44,m}$,    
Y.F.~Ryabov$^\textrm{\scriptsize 134}$,    
M.~Rybar$^\textrm{\scriptsize 171}$,    
G.~Rybkin$^\textrm{\scriptsize 128}$,    
S.~Ryu$^\textrm{\scriptsize 6}$,    
A.~Ryzhov$^\textrm{\scriptsize 140}$,    
G.F.~Rzehorz$^\textrm{\scriptsize 51}$,    
P.~Sabatini$^\textrm{\scriptsize 51}$,    
G.~Sabato$^\textrm{\scriptsize 118}$,    
S.~Sacerdoti$^\textrm{\scriptsize 128}$,    
H.F-W.~Sadrozinski$^\textrm{\scriptsize 143}$,    
R.~Sadykov$^\textrm{\scriptsize 77}$,    
F.~Safai~Tehrani$^\textrm{\scriptsize 70a}$,    
P.~Saha$^\textrm{\scriptsize 119}$,    
M.~Sahinsoy$^\textrm{\scriptsize 59a}$,    
M.~Saimpert$^\textrm{\scriptsize 44}$,    
M.~Saito$^\textrm{\scriptsize 161}$,    
T.~Saito$^\textrm{\scriptsize 161}$,    
H.~Sakamoto$^\textrm{\scriptsize 161}$,    
A.~Sakharov$^\textrm{\scriptsize 121,an}$,    
D.~Salamani$^\textrm{\scriptsize 52}$,    
G.~Salamanna$^\textrm{\scriptsize 72a,72b}$,    
J.E.~Salazar~Loyola$^\textrm{\scriptsize 144b}$,    
D.~Salek$^\textrm{\scriptsize 118}$,    
P.H.~Sales~De~Bruin$^\textrm{\scriptsize 170}$,    
D.~Salihagic$^\textrm{\scriptsize 113}$,    
A.~Salnikov$^\textrm{\scriptsize 150}$,    
J.~Salt$^\textrm{\scriptsize 172}$,    
D.~Salvatore$^\textrm{\scriptsize 40b,40a}$,    
F.~Salvatore$^\textrm{\scriptsize 153}$,    
A.~Salvucci$^\textrm{\scriptsize 61a,61b,61c}$,    
A.~Salzburger$^\textrm{\scriptsize 35}$,    
D.~Sammel$^\textrm{\scriptsize 50}$,    
D.~Sampsonidis$^\textrm{\scriptsize 160}$,    
D.~Sampsonidou$^\textrm{\scriptsize 160}$,    
J.~S\'anchez$^\textrm{\scriptsize 172}$,    
A.~Sanchez~Pineda$^\textrm{\scriptsize 64a,64c}$,    
H.~Sandaker$^\textrm{\scriptsize 130}$,    
C.O.~Sander$^\textrm{\scriptsize 44}$,    
M.~Sandhoff$^\textrm{\scriptsize 180}$,    
C.~Sandoval$^\textrm{\scriptsize 22}$,    
D.P.C.~Sankey$^\textrm{\scriptsize 141}$,    
M.~Sannino$^\textrm{\scriptsize 53b,53a}$,    
Y.~Sano$^\textrm{\scriptsize 115}$,    
A.~Sansoni$^\textrm{\scriptsize 49}$,    
C.~Santoni$^\textrm{\scriptsize 37}$,    
H.~Santos$^\textrm{\scriptsize 136a}$,    
I.~Santoyo~Castillo$^\textrm{\scriptsize 153}$,    
A.~Sapronov$^\textrm{\scriptsize 77}$,    
J.G.~Saraiva$^\textrm{\scriptsize 136a,136d}$,    
O.~Sasaki$^\textrm{\scriptsize 79}$,    
K.~Sato$^\textrm{\scriptsize 167}$,    
E.~Sauvan$^\textrm{\scriptsize 5}$,    
P.~Savard$^\textrm{\scriptsize 165,ax}$,    
N.~Savic$^\textrm{\scriptsize 113}$,    
R.~Sawada$^\textrm{\scriptsize 161}$,    
C.~Sawyer$^\textrm{\scriptsize 141}$,    
L.~Sawyer$^\textrm{\scriptsize 93,al}$,    
C.~Sbarra$^\textrm{\scriptsize 23b}$,    
A.~Sbrizzi$^\textrm{\scriptsize 23b,23a}$,    
T.~Scanlon$^\textrm{\scriptsize 92}$,    
D.A.~Scannicchio$^\textrm{\scriptsize 169}$,    
J.~Schaarschmidt$^\textrm{\scriptsize 145}$,    
P.~Schacht$^\textrm{\scriptsize 113}$,    
B.M.~Schachtner$^\textrm{\scriptsize 112}$,    
D.~Schaefer$^\textrm{\scriptsize 36}$,    
L.~Schaefer$^\textrm{\scriptsize 133}$,    
J.~Schaeffer$^\textrm{\scriptsize 97}$,    
S.~Schaepe$^\textrm{\scriptsize 35}$,    
U.~Sch\"afer$^\textrm{\scriptsize 97}$,    
A.C.~Schaffer$^\textrm{\scriptsize 128}$,    
D.~Schaile$^\textrm{\scriptsize 112}$,    
R.D.~Schamberger$^\textrm{\scriptsize 152}$,    
V.A.~Schegelsky$^\textrm{\scriptsize 134}$,    
D.~Scheirich$^\textrm{\scriptsize 139}$,    
F.~Schenck$^\textrm{\scriptsize 19}$,    
M.~Schernau$^\textrm{\scriptsize 169}$,    
C.~Schiavi$^\textrm{\scriptsize 53b,53a}$,    
S.~Schier$^\textrm{\scriptsize 143}$,    
L.K.~Schildgen$^\textrm{\scriptsize 24}$,    
Z.M.~Schillaci$^\textrm{\scriptsize 26}$,    
E.J.~Schioppa$^\textrm{\scriptsize 35}$,    
M.~Schioppa$^\textrm{\scriptsize 40b,40a}$,    
K.E.~Schleicher$^\textrm{\scriptsize 50}$,    
S.~Schlenker$^\textrm{\scriptsize 35}$,    
K.R.~Schmidt-Sommerfeld$^\textrm{\scriptsize 113}$,    
K.~Schmieden$^\textrm{\scriptsize 35}$,    
C.~Schmitt$^\textrm{\scriptsize 97}$,    
S.~Schmitt$^\textrm{\scriptsize 44}$,    
S.~Schmitz$^\textrm{\scriptsize 97}$,    
U.~Schnoor$^\textrm{\scriptsize 50}$,    
L.~Schoeffel$^\textrm{\scriptsize 142}$,    
A.~Schoening$^\textrm{\scriptsize 59b}$,    
E.~Schopf$^\textrm{\scriptsize 24}$,    
M.~Schott$^\textrm{\scriptsize 97}$,    
J.F.P.~Schouwenberg$^\textrm{\scriptsize 117}$,    
J.~Schovancova$^\textrm{\scriptsize 35}$,    
S.~Schramm$^\textrm{\scriptsize 52}$,    
N.~Schuh$^\textrm{\scriptsize 97}$,    
A.~Schulte$^\textrm{\scriptsize 97}$,    
H-C.~Schultz-Coulon$^\textrm{\scriptsize 59a}$,    
M.~Schumacher$^\textrm{\scriptsize 50}$,    
B.A.~Schumm$^\textrm{\scriptsize 143}$,    
Ph.~Schune$^\textrm{\scriptsize 142}$,    
A.~Schwartzman$^\textrm{\scriptsize 150}$,    
T.A.~Schwarz$^\textrm{\scriptsize 103}$,    
H.~Schweiger$^\textrm{\scriptsize 98}$,    
Ph.~Schwemling$^\textrm{\scriptsize 142}$,    
R.~Schwienhorst$^\textrm{\scriptsize 104}$,    
A.~Sciandra$^\textrm{\scriptsize 24}$,    
G.~Sciolla$^\textrm{\scriptsize 26}$,    
M.~Scornajenghi$^\textrm{\scriptsize 40b,40a}$,    
F.~Scuri$^\textrm{\scriptsize 69a}$,    
F.~Scutti$^\textrm{\scriptsize 102}$,    
L.M.~Scyboz$^\textrm{\scriptsize 113}$,    
J.~Searcy$^\textrm{\scriptsize 103}$,    
P.~Seema$^\textrm{\scriptsize 24}$,    
S.C.~Seidel$^\textrm{\scriptsize 116}$,    
A.~Seiden$^\textrm{\scriptsize 143}$,    
J.M.~Seixas$^\textrm{\scriptsize 78b}$,    
G.~Sekhniaidze$^\textrm{\scriptsize 67a}$,    
K.~Sekhon$^\textrm{\scriptsize 103}$,    
S.J.~Sekula$^\textrm{\scriptsize 41}$,    
N.~Semprini-Cesari$^\textrm{\scriptsize 23b,23a}$,    
S.~Senkin$^\textrm{\scriptsize 37}$,    
C.~Serfon$^\textrm{\scriptsize 130}$,    
L.~Serin$^\textrm{\scriptsize 128}$,    
L.~Serkin$^\textrm{\scriptsize 64a,64b}$,    
M.~Sessa$^\textrm{\scriptsize 72a,72b}$,    
H.~Severini$^\textrm{\scriptsize 124}$,    
F.~Sforza$^\textrm{\scriptsize 168}$,    
A.~Sfyrla$^\textrm{\scriptsize 52}$,    
E.~Shabalina$^\textrm{\scriptsize 51}$,    
J.D.~Shahinian$^\textrm{\scriptsize 143}$,    
N.W.~Shaikh$^\textrm{\scriptsize 43a,43b}$,    
L.Y.~Shan$^\textrm{\scriptsize 15a}$,    
R.~Shang$^\textrm{\scriptsize 171}$,    
J.T.~Shank$^\textrm{\scriptsize 25}$,    
M.~Shapiro$^\textrm{\scriptsize 18}$,    
A.S.~Sharma$^\textrm{\scriptsize 1}$,    
A.~Sharma$^\textrm{\scriptsize 131}$,    
P.B.~Shatalov$^\textrm{\scriptsize 109}$,    
K.~Shaw$^\textrm{\scriptsize 64a,64b}$,    
S.M.~Shaw$^\textrm{\scriptsize 98}$,    
A.~Shcherbakova$^\textrm{\scriptsize 43a,43b}$,    
C.Y.~Shehu$^\textrm{\scriptsize 153}$,    
Y.~Shen$^\textrm{\scriptsize 124}$,    
N.~Sherafati$^\textrm{\scriptsize 33}$,    
A.D.~Sherman$^\textrm{\scriptsize 25}$,    
P.~Sherwood$^\textrm{\scriptsize 92}$,    
L.~Shi$^\textrm{\scriptsize 155,at}$,    
S.~Shimizu$^\textrm{\scriptsize 80}$,    
C.O.~Shimmin$^\textrm{\scriptsize 181}$,    
M.~Shimojima$^\textrm{\scriptsize 114}$,    
I.P.J.~Shipsey$^\textrm{\scriptsize 131}$,    
S.~Shirabe$^\textrm{\scriptsize 85}$,    
M.~Shiyakova$^\textrm{\scriptsize 77}$,    
J.~Shlomi$^\textrm{\scriptsize 178}$,    
A.~Shmeleva$^\textrm{\scriptsize 108}$,    
D.~Shoaleh~Saadi$^\textrm{\scriptsize 107}$,    
M.J.~Shochet$^\textrm{\scriptsize 36}$,    
S.~Shojaii$^\textrm{\scriptsize 102}$,    
D.R.~Shope$^\textrm{\scriptsize 124}$,    
S.~Shrestha$^\textrm{\scriptsize 122}$,    
E.~Shulga$^\textrm{\scriptsize 110}$,    
P.~Sicho$^\textrm{\scriptsize 137}$,    
A.M.~Sickles$^\textrm{\scriptsize 171}$,    
P.E.~Sidebo$^\textrm{\scriptsize 151}$,    
E.~Sideras~Haddad$^\textrm{\scriptsize 32c}$,    
O.~Sidiropoulou$^\textrm{\scriptsize 175}$,    
A.~Sidoti$^\textrm{\scriptsize 23b,23a}$,    
F.~Siegert$^\textrm{\scriptsize 46}$,    
Dj.~Sijacki$^\textrm{\scriptsize 16}$,    
J.~Silva$^\textrm{\scriptsize 136a}$,    
M.~Silva~Jr.$^\textrm{\scriptsize 179}$,    
S.B.~Silverstein$^\textrm{\scriptsize 43a}$,    
L.~Simic$^\textrm{\scriptsize 77}$,    
S.~Simion$^\textrm{\scriptsize 128}$,    
E.~Simioni$^\textrm{\scriptsize 97}$,    
B.~Simmons$^\textrm{\scriptsize 92}$,    
M.~Simon$^\textrm{\scriptsize 97}$,    
P.~Sinervo$^\textrm{\scriptsize 165}$,    
N.B.~Sinev$^\textrm{\scriptsize 127}$,    
M.~Sioli$^\textrm{\scriptsize 23b,23a}$,    
G.~Siragusa$^\textrm{\scriptsize 175}$,    
I.~Siral$^\textrm{\scriptsize 103}$,    
S.Yu.~Sivoklokov$^\textrm{\scriptsize 111}$,    
J.~Sj\"{o}lin$^\textrm{\scriptsize 43a,43b}$,    
M.B.~Skinner$^\textrm{\scriptsize 87}$,    
P.~Skubic$^\textrm{\scriptsize 124}$,    
M.~Slater$^\textrm{\scriptsize 21}$,    
T.~Slavicek$^\textrm{\scriptsize 138}$,    
M.~Slawinska$^\textrm{\scriptsize 82}$,    
K.~Sliwa$^\textrm{\scriptsize 168}$,    
R.~Slovak$^\textrm{\scriptsize 139}$,    
V.~Smakhtin$^\textrm{\scriptsize 178}$,    
B.H.~Smart$^\textrm{\scriptsize 5}$,    
J.~Smiesko$^\textrm{\scriptsize 28a}$,    
N.~Smirnov$^\textrm{\scriptsize 110}$,    
S.Yu.~Smirnov$^\textrm{\scriptsize 110}$,    
Y.~Smirnov$^\textrm{\scriptsize 110}$,    
L.N.~Smirnova$^\textrm{\scriptsize 111}$,    
O.~Smirnova$^\textrm{\scriptsize 94}$,    
J.W.~Smith$^\textrm{\scriptsize 51}$,    
M.N.K.~Smith$^\textrm{\scriptsize 38}$,    
R.W.~Smith$^\textrm{\scriptsize 38}$,    
M.~Smizanska$^\textrm{\scriptsize 87}$,    
K.~Smolek$^\textrm{\scriptsize 138}$,    
A.A.~Snesarev$^\textrm{\scriptsize 108}$,    
I.M.~Snyder$^\textrm{\scriptsize 127}$,    
S.~Snyder$^\textrm{\scriptsize 29}$,    
R.~Sobie$^\textrm{\scriptsize 174,ag}$,    
F.~Socher$^\textrm{\scriptsize 46}$,    
A.M.~Soffa$^\textrm{\scriptsize 169}$,    
A.~Soffer$^\textrm{\scriptsize 159}$,    
A.~S{\o}gaard$^\textrm{\scriptsize 48}$,    
D.A.~Soh$^\textrm{\scriptsize 155}$,    
G.~Sokhrannyi$^\textrm{\scriptsize 89}$,    
C.A.~Solans~Sanchez$^\textrm{\scriptsize 35}$,    
M.~Solar$^\textrm{\scriptsize 138}$,    
E.Yu.~Soldatov$^\textrm{\scriptsize 110}$,    
U.~Soldevila$^\textrm{\scriptsize 172}$,    
A.A.~Solodkov$^\textrm{\scriptsize 140}$,    
A.~Soloshenko$^\textrm{\scriptsize 77}$,    
O.V.~Solovyanov$^\textrm{\scriptsize 140}$,    
V.~Solovyev$^\textrm{\scriptsize 134}$,    
P.~Sommer$^\textrm{\scriptsize 146}$,    
H.~Son$^\textrm{\scriptsize 168}$,    
W.~Song$^\textrm{\scriptsize 141}$,    
A.~Sopczak$^\textrm{\scriptsize 138}$,    
F.~Sopkova$^\textrm{\scriptsize 28b}$,    
D.~Sosa$^\textrm{\scriptsize 59b}$,    
C.L.~Sotiropoulou$^\textrm{\scriptsize 69a,69b}$,    
S.~Sottocornola$^\textrm{\scriptsize 68a,68b}$,    
R.~Soualah$^\textrm{\scriptsize 64a,64c,j}$,    
A.M.~Soukharev$^\textrm{\scriptsize 120b,120a}$,    
D.~South$^\textrm{\scriptsize 44}$,    
B.C.~Sowden$^\textrm{\scriptsize 91}$,    
S.~Spagnolo$^\textrm{\scriptsize 65a,65b}$,    
M.~Spalla$^\textrm{\scriptsize 113}$,    
M.~Spangenberg$^\textrm{\scriptsize 176}$,    
F.~Span\`o$^\textrm{\scriptsize 91}$,    
D.~Sperlich$^\textrm{\scriptsize 19}$,    
F.~Spettel$^\textrm{\scriptsize 113}$,    
T.M.~Spieker$^\textrm{\scriptsize 59a}$,    
R.~Spighi$^\textrm{\scriptsize 23b}$,    
G.~Spigo$^\textrm{\scriptsize 35}$,    
L.A.~Spiller$^\textrm{\scriptsize 102}$,    
M.~Spousta$^\textrm{\scriptsize 139}$,    
R.D.~St.~Denis$^\textrm{\scriptsize 55,*}$,    
A.~Stabile$^\textrm{\scriptsize 66a,66b}$,    
R.~Stamen$^\textrm{\scriptsize 59a}$,    
S.~Stamm$^\textrm{\scriptsize 19}$,    
E.~Stanecka$^\textrm{\scriptsize 82}$,    
R.W.~Stanek$^\textrm{\scriptsize 6}$,    
C.~Stanescu$^\textrm{\scriptsize 72a}$,    
M.M.~Stanitzki$^\textrm{\scriptsize 44}$,    
B.~Stapf$^\textrm{\scriptsize 118}$,    
S.~Stapnes$^\textrm{\scriptsize 130}$,    
E.A.~Starchenko$^\textrm{\scriptsize 140}$,    
G.H.~Stark$^\textrm{\scriptsize 36}$,    
J.~Stark$^\textrm{\scriptsize 56}$,    
S.H~Stark$^\textrm{\scriptsize 39}$,    
P.~Staroba$^\textrm{\scriptsize 137}$,    
P.~Starovoitov$^\textrm{\scriptsize 59a}$,    
S.~St\"arz$^\textrm{\scriptsize 35}$,    
R.~Staszewski$^\textrm{\scriptsize 82}$,    
M.~Stegler$^\textrm{\scriptsize 44}$,    
P.~Steinberg$^\textrm{\scriptsize 29}$,    
B.~Stelzer$^\textrm{\scriptsize 149}$,    
H.J.~Stelzer$^\textrm{\scriptsize 35}$,    
O.~Stelzer-Chilton$^\textrm{\scriptsize 166a}$,    
H.~Stenzel$^\textrm{\scriptsize 54}$,    
T.J.~Stevenson$^\textrm{\scriptsize 90}$,    
G.A.~Stewart$^\textrm{\scriptsize 55}$,    
M.C.~Stockton$^\textrm{\scriptsize 127}$,    
G.~Stoicea$^\textrm{\scriptsize 27b}$,    
P.~Stolte$^\textrm{\scriptsize 51}$,    
S.~Stonjek$^\textrm{\scriptsize 113}$,    
A.~Straessner$^\textrm{\scriptsize 46}$,    
M.E.~Stramaglia$^\textrm{\scriptsize 20}$,    
J.~Strandberg$^\textrm{\scriptsize 151}$,    
S.~Strandberg$^\textrm{\scriptsize 43a,43b}$,    
M.~Strauss$^\textrm{\scriptsize 124}$,    
P.~Strizenec$^\textrm{\scriptsize 28b}$,    
R.~Str\"ohmer$^\textrm{\scriptsize 175}$,    
D.M.~Strom$^\textrm{\scriptsize 127}$,    
R.~Stroynowski$^\textrm{\scriptsize 41}$,    
A.~Strubig$^\textrm{\scriptsize 48}$,    
S.A.~Stucci$^\textrm{\scriptsize 29}$,    
B.~Stugu$^\textrm{\scriptsize 17}$,    
N.A.~Styles$^\textrm{\scriptsize 44}$,    
D.~Su$^\textrm{\scriptsize 150}$,    
J.~Su$^\textrm{\scriptsize 135}$,    
S.~Suchek$^\textrm{\scriptsize 59a}$,    
Y.~Sugaya$^\textrm{\scriptsize 129}$,    
M.~Suk$^\textrm{\scriptsize 138}$,    
V.V.~Sulin$^\textrm{\scriptsize 108}$,    
D.M.S.~Sultan$^\textrm{\scriptsize 52}$,    
S.~Sultansoy$^\textrm{\scriptsize 4c}$,    
T.~Sumida$^\textrm{\scriptsize 83}$,    
S.~Sun$^\textrm{\scriptsize 103}$,    
X.~Sun$^\textrm{\scriptsize 3}$,    
K.~Suruliz$^\textrm{\scriptsize 153}$,    
C.J.E.~Suster$^\textrm{\scriptsize 154}$,    
M.R.~Sutton$^\textrm{\scriptsize 153}$,    
S.~Suzuki$^\textrm{\scriptsize 79}$,    
M.~Svatos$^\textrm{\scriptsize 137}$,    
M.~Swiatlowski$^\textrm{\scriptsize 36}$,    
S.P.~Swift$^\textrm{\scriptsize 2}$,    
A.~Sydorenko$^\textrm{\scriptsize 97}$,    
I.~Sykora$^\textrm{\scriptsize 28a}$,    
T.~Sykora$^\textrm{\scriptsize 139}$,    
D.~Ta$^\textrm{\scriptsize 97}$,    
K.~Tackmann$^\textrm{\scriptsize 44,ad}$,    
J.~Taenzer$^\textrm{\scriptsize 159}$,    
A.~Taffard$^\textrm{\scriptsize 169}$,    
R.~Tafirout$^\textrm{\scriptsize 166a}$,    
E.~Tahirovic$^\textrm{\scriptsize 90}$,    
N.~Taiblum$^\textrm{\scriptsize 159}$,    
H.~Takai$^\textrm{\scriptsize 29}$,    
R.~Takashima$^\textrm{\scriptsize 84}$,    
E.H.~Takasugi$^\textrm{\scriptsize 113}$,    
K.~Takeda$^\textrm{\scriptsize 80}$,    
T.~Takeshita$^\textrm{\scriptsize 147}$,    
Y.~Takubo$^\textrm{\scriptsize 79}$,    
M.~Talby$^\textrm{\scriptsize 99}$,    
A.A.~Talyshev$^\textrm{\scriptsize 120b,120a}$,    
J.~Tanaka$^\textrm{\scriptsize 161}$,    
M.~Tanaka$^\textrm{\scriptsize 163}$,    
R.~Tanaka$^\textrm{\scriptsize 128}$,    
R.~Tanioka$^\textrm{\scriptsize 80}$,    
B.B.~Tannenwald$^\textrm{\scriptsize 122}$,    
S.~Tapia~Araya$^\textrm{\scriptsize 144b}$,    
S.~Tapprogge$^\textrm{\scriptsize 97}$,    
A.~Tarek~Abouelfadl~Mohamed$^\textrm{\scriptsize 132}$,    
S.~Tarem$^\textrm{\scriptsize 158}$,    
G.~Tarna$^\textrm{\scriptsize 27b,f}$,    
G.F.~Tartarelli$^\textrm{\scriptsize 66a}$,    
P.~Tas$^\textrm{\scriptsize 139}$,    
M.~Tasevsky$^\textrm{\scriptsize 137}$,    
T.~Tashiro$^\textrm{\scriptsize 83}$,    
E.~Tassi$^\textrm{\scriptsize 40b,40a}$,    
A.~Tavares~Delgado$^\textrm{\scriptsize 136a,136b}$,    
Y.~Tayalati$^\textrm{\scriptsize 34e}$,    
A.C.~Taylor$^\textrm{\scriptsize 116}$,    
A.J.~Taylor$^\textrm{\scriptsize 48}$,    
G.N.~Taylor$^\textrm{\scriptsize 102}$,    
P.T.E.~Taylor$^\textrm{\scriptsize 102}$,    
W.~Taylor$^\textrm{\scriptsize 166b}$,    
P.~Teixeira-Dias$^\textrm{\scriptsize 91}$,    
D.~Temple$^\textrm{\scriptsize 149}$,    
H.~Ten~Kate$^\textrm{\scriptsize 35}$,    
P.K.~Teng$^\textrm{\scriptsize 155}$,    
J.J.~Teoh$^\textrm{\scriptsize 129}$,    
F.~Tepel$^\textrm{\scriptsize 180}$,    
S.~Terada$^\textrm{\scriptsize 79}$,    
K.~Terashi$^\textrm{\scriptsize 161}$,    
J.~Terron$^\textrm{\scriptsize 96}$,    
S.~Terzo$^\textrm{\scriptsize 14}$,    
M.~Testa$^\textrm{\scriptsize 49}$,    
R.J.~Teuscher$^\textrm{\scriptsize 165,ag}$,    
S.J.~Thais$^\textrm{\scriptsize 181}$,    
T.~Theveneaux-Pelzer$^\textrm{\scriptsize 44}$,    
F.~Thiele$^\textrm{\scriptsize 39}$,    
J.P.~Thomas$^\textrm{\scriptsize 21}$,    
A.S.~Thompson$^\textrm{\scriptsize 55}$,    
P.D.~Thompson$^\textrm{\scriptsize 21}$,    
L.A.~Thomsen$^\textrm{\scriptsize 181}$,    
E.~Thomson$^\textrm{\scriptsize 133}$,    
Y.~Tian$^\textrm{\scriptsize 38}$,    
R.E.~Ticse~Torres$^\textrm{\scriptsize 51}$,    
V.O.~Tikhomirov$^\textrm{\scriptsize 108,ap}$,    
Yu.A.~Tikhonov$^\textrm{\scriptsize 120b,120a}$,    
S.~Timoshenko$^\textrm{\scriptsize 110}$,    
P.~Tipton$^\textrm{\scriptsize 181}$,    
S.~Tisserant$^\textrm{\scriptsize 99}$,    
K.~Todome$^\textrm{\scriptsize 163}$,    
S.~Todorova-Nova$^\textrm{\scriptsize 5}$,    
S.~Todt$^\textrm{\scriptsize 46}$,    
J.~Tojo$^\textrm{\scriptsize 85}$,    
S.~Tok\'ar$^\textrm{\scriptsize 28a}$,    
K.~Tokushuku$^\textrm{\scriptsize 79}$,    
E.~Tolley$^\textrm{\scriptsize 122}$,    
M.~Tomoto$^\textrm{\scriptsize 115}$,    
L.~Tompkins$^\textrm{\scriptsize 150,s}$,    
K.~Toms$^\textrm{\scriptsize 116}$,    
B.~Tong$^\textrm{\scriptsize 57}$,    
P.~Tornambe$^\textrm{\scriptsize 50}$,    
E.~Torrence$^\textrm{\scriptsize 127}$,    
H.~Torres$^\textrm{\scriptsize 46}$,    
E.~Torr\'o~Pastor$^\textrm{\scriptsize 145}$,    
C.~Tosciri$^\textrm{\scriptsize 131}$,    
J.~Toth$^\textrm{\scriptsize 99,af}$,    
F.~Touchard$^\textrm{\scriptsize 99}$,    
D.R.~Tovey$^\textrm{\scriptsize 146}$,    
C.J.~Treado$^\textrm{\scriptsize 121}$,    
T.~Trefzger$^\textrm{\scriptsize 175}$,    
F.~Tresoldi$^\textrm{\scriptsize 153}$,    
A.~Tricoli$^\textrm{\scriptsize 29}$,    
I.M.~Trigger$^\textrm{\scriptsize 166a}$,    
S.~Trincaz-Duvoid$^\textrm{\scriptsize 132}$,    
M.F.~Tripiana$^\textrm{\scriptsize 14}$,    
W.~Trischuk$^\textrm{\scriptsize 165}$,    
B.~Trocm\'e$^\textrm{\scriptsize 56}$,    
A.~Trofymov$^\textrm{\scriptsize 44}$,    
C.~Troncon$^\textrm{\scriptsize 66a}$,    
M.~Trovatelli$^\textrm{\scriptsize 174}$,    
L.~Truong$^\textrm{\scriptsize 32b}$,    
M.~Trzebinski$^\textrm{\scriptsize 82}$,    
A.~Trzupek$^\textrm{\scriptsize 82}$,    
F.~Tsai$^\textrm{\scriptsize 44}$,    
K.W.~Tsang$^\textrm{\scriptsize 61a}$,    
J.C-L.~Tseng$^\textrm{\scriptsize 131}$,    
P.V.~Tsiareshka$^\textrm{\scriptsize 105}$,    
N.~Tsirintanis$^\textrm{\scriptsize 9}$,    
S.~Tsiskaridze$^\textrm{\scriptsize 14}$,    
V.~Tsiskaridze$^\textrm{\scriptsize 152}$,    
E.G.~Tskhadadze$^\textrm{\scriptsize 157a}$,    
I.I.~Tsukerman$^\textrm{\scriptsize 109}$,    
V.~Tsulaia$^\textrm{\scriptsize 18}$,    
S.~Tsuno$^\textrm{\scriptsize 79}$,    
D.~Tsybychev$^\textrm{\scriptsize 152}$,    
Y.~Tu$^\textrm{\scriptsize 61b}$,    
A.~Tudorache$^\textrm{\scriptsize 27b}$,    
V.~Tudorache$^\textrm{\scriptsize 27b}$,    
T.T.~Tulbure$^\textrm{\scriptsize 27a}$,    
A.N.~Tuna$^\textrm{\scriptsize 57}$,    
S.~Turchikhin$^\textrm{\scriptsize 77}$,    
D.~Turgeman$^\textrm{\scriptsize 178}$,    
I.~Turk~Cakir$^\textrm{\scriptsize 4b,w}$,    
R.~Turra$^\textrm{\scriptsize 66a}$,    
P.M.~Tuts$^\textrm{\scriptsize 38}$,    
G.~Ucchielli$^\textrm{\scriptsize 23b,23a}$,    
I.~Ueda$^\textrm{\scriptsize 79}$,    
M.~Ughetto$^\textrm{\scriptsize 43a,43b}$,    
F.~Ukegawa$^\textrm{\scriptsize 167}$,    
G.~Unal$^\textrm{\scriptsize 35}$,    
A.~Undrus$^\textrm{\scriptsize 29}$,    
G.~Unel$^\textrm{\scriptsize 169}$,    
F.C.~Ungaro$^\textrm{\scriptsize 102}$,    
Y.~Unno$^\textrm{\scriptsize 79}$,    
K.~Uno$^\textrm{\scriptsize 161}$,    
J.~Urban$^\textrm{\scriptsize 28b}$,    
P.~Urquijo$^\textrm{\scriptsize 102}$,    
P.~Urrejola$^\textrm{\scriptsize 97}$,    
G.~Usai$^\textrm{\scriptsize 8}$,    
J.~Usui$^\textrm{\scriptsize 79}$,    
L.~Vacavant$^\textrm{\scriptsize 99}$,    
V.~Vacek$^\textrm{\scriptsize 138}$,    
B.~Vachon$^\textrm{\scriptsize 101}$,    
K.O.H.~Vadla$^\textrm{\scriptsize 130}$,    
A.~Vaidya$^\textrm{\scriptsize 92}$,    
C.~Valderanis$^\textrm{\scriptsize 112}$,    
E.~Valdes~Santurio$^\textrm{\scriptsize 43a,43b}$,    
M.~Valente$^\textrm{\scriptsize 52}$,    
S.~Valentinetti$^\textrm{\scriptsize 23b,23a}$,    
A.~Valero$^\textrm{\scriptsize 172}$,    
L.~Val\'ery$^\textrm{\scriptsize 44}$,    
R.A.~Vallance$^\textrm{\scriptsize 21}$,    
A.~Vallier$^\textrm{\scriptsize 5}$,    
J.A.~Valls~Ferrer$^\textrm{\scriptsize 172}$,    
T.R.~Van~Daalen$^\textrm{\scriptsize 14}$,    
W.~Van~Den~Wollenberg$^\textrm{\scriptsize 118}$,    
H.~Van~der~Graaf$^\textrm{\scriptsize 118}$,    
P.~Van~Gemmeren$^\textrm{\scriptsize 6}$,    
J.~Van~Nieuwkoop$^\textrm{\scriptsize 149}$,    
I.~Van~Vulpen$^\textrm{\scriptsize 118}$,    
M.C.~van~Woerden$^\textrm{\scriptsize 118}$,    
M.~Vanadia$^\textrm{\scriptsize 71a,71b}$,    
W.~Vandelli$^\textrm{\scriptsize 35}$,    
A.~Vaniachine$^\textrm{\scriptsize 164}$,    
P.~Vankov$^\textrm{\scriptsize 118}$,    
R.~Vari$^\textrm{\scriptsize 70a}$,    
E.W.~Varnes$^\textrm{\scriptsize 7}$,    
C.~Varni$^\textrm{\scriptsize 53b,53a}$,    
T.~Varol$^\textrm{\scriptsize 41}$,    
D.~Varouchas$^\textrm{\scriptsize 128}$,    
A.~Vartapetian$^\textrm{\scriptsize 8}$,    
K.E.~Varvell$^\textrm{\scriptsize 154}$,    
G.A.~Vasquez$^\textrm{\scriptsize 144b}$,    
J.G.~Vasquez$^\textrm{\scriptsize 181}$,    
F.~Vazeille$^\textrm{\scriptsize 37}$,    
D.~Vazquez~Furelos$^\textrm{\scriptsize 14}$,    
T.~Vazquez~Schroeder$^\textrm{\scriptsize 101}$,    
J.~Veatch$^\textrm{\scriptsize 51}$,    
L.M.~Veloce$^\textrm{\scriptsize 165}$,    
F.~Veloso$^\textrm{\scriptsize 136a,136c}$,    
S.~Veneziano$^\textrm{\scriptsize 70a}$,    
A.~Ventura$^\textrm{\scriptsize 65a,65b}$,    
M.~Venturi$^\textrm{\scriptsize 174}$,    
N.~Venturi$^\textrm{\scriptsize 35}$,    
V.~Vercesi$^\textrm{\scriptsize 68a}$,    
M.~Verducci$^\textrm{\scriptsize 72a,72b}$,    
W.~Verkerke$^\textrm{\scriptsize 118}$,    
A.T.~Vermeulen$^\textrm{\scriptsize 118}$,    
J.C.~Vermeulen$^\textrm{\scriptsize 118}$,    
M.C.~Vetterli$^\textrm{\scriptsize 149,ax}$,    
N.~Viaux~Maira$^\textrm{\scriptsize 144b}$,    
O.~Viazlo$^\textrm{\scriptsize 94}$,    
I.~Vichou$^\textrm{\scriptsize 171,*}$,    
T.~Vickey$^\textrm{\scriptsize 146}$,    
O.E.~Vickey~Boeriu$^\textrm{\scriptsize 146}$,    
G.H.A.~Viehhauser$^\textrm{\scriptsize 131}$,    
S.~Viel$^\textrm{\scriptsize 18}$,    
L.~Vigani$^\textrm{\scriptsize 131}$,    
M.~Villa$^\textrm{\scriptsize 23b,23a}$,    
M.~Villaplana~Perez$^\textrm{\scriptsize 66a,66b}$,    
E.~Vilucchi$^\textrm{\scriptsize 49}$,    
M.G.~Vincter$^\textrm{\scriptsize 33}$,    
V.B.~Vinogradov$^\textrm{\scriptsize 77}$,    
A.~Vishwakarma$^\textrm{\scriptsize 44}$,    
C.~Vittori$^\textrm{\scriptsize 23b,23a}$,    
I.~Vivarelli$^\textrm{\scriptsize 153}$,    
S.~Vlachos$^\textrm{\scriptsize 10}$,    
M.~Vogel$^\textrm{\scriptsize 180}$,    
P.~Vokac$^\textrm{\scriptsize 138}$,    
G.~Volpi$^\textrm{\scriptsize 14}$,    
S.E.~von~Buddenbrock$^\textrm{\scriptsize 32c}$,    
E.~Von~Toerne$^\textrm{\scriptsize 24}$,    
V.~Vorobel$^\textrm{\scriptsize 139}$,    
K.~Vorobev$^\textrm{\scriptsize 110}$,    
M.~Vos$^\textrm{\scriptsize 172}$,    
J.H.~Vossebeld$^\textrm{\scriptsize 88}$,    
N.~Vranjes$^\textrm{\scriptsize 16}$,    
M.~Vranjes~Milosavljevic$^\textrm{\scriptsize 16}$,    
V.~Vrba$^\textrm{\scriptsize 138}$,    
M.~Vreeswijk$^\textrm{\scriptsize 118}$,    
T.~\v{S}filigoj$^\textrm{\scriptsize 89}$,    
R.~Vuillermet$^\textrm{\scriptsize 35}$,    
I.~Vukotic$^\textrm{\scriptsize 36}$,    
T.~\v{Z}eni\v{s}$^\textrm{\scriptsize 28a}$,    
L.~\v{Z}ivkovi\'{c}$^\textrm{\scriptsize 16}$,    
P.~Wagner$^\textrm{\scriptsize 24}$,    
W.~Wagner$^\textrm{\scriptsize 180}$,    
J.~Wagner-Kuhr$^\textrm{\scriptsize 112}$,    
H.~Wahlberg$^\textrm{\scriptsize 86}$,    
S.~Wahrmund$^\textrm{\scriptsize 46}$,    
K.~Wakamiya$^\textrm{\scriptsize 80}$,    
J.~Walder$^\textrm{\scriptsize 87}$,    
R.~Walker$^\textrm{\scriptsize 112}$,    
W.~Walkowiak$^\textrm{\scriptsize 148}$,    
V.~Wallangen$^\textrm{\scriptsize 43a,43b}$,    
A.M.~Wang$^\textrm{\scriptsize 57}$,    
C.~Wang$^\textrm{\scriptsize 58b,f}$,    
F.~Wang$^\textrm{\scriptsize 179}$,    
H.~Wang$^\textrm{\scriptsize 18}$,    
H.~Wang$^\textrm{\scriptsize 3}$,    
J.~Wang$^\textrm{\scriptsize 154}$,    
J.~Wang$^\textrm{\scriptsize 59b}$,    
Q.~Wang$^\textrm{\scriptsize 124}$,    
R.-J.~Wang$^\textrm{\scriptsize 132}$,    
R.~Wang$^\textrm{\scriptsize 58a}$,    
R.~Wang$^\textrm{\scriptsize 6}$,    
S.M.~Wang$^\textrm{\scriptsize 155}$,    
T.~Wang$^\textrm{\scriptsize 38}$,    
W.~Wang$^\textrm{\scriptsize 155,q}$,    
W.X.~Wang$^\textrm{\scriptsize 58a,ah}$,    
Z.~Wang$^\textrm{\scriptsize 58c}$,    
C.~Wanotayaroj$^\textrm{\scriptsize 44}$,    
A.~Warburton$^\textrm{\scriptsize 101}$,    
C.P.~Ward$^\textrm{\scriptsize 31}$,    
D.R.~Wardrope$^\textrm{\scriptsize 92}$,    
A.~Washbrook$^\textrm{\scriptsize 48}$,    
P.M.~Watkins$^\textrm{\scriptsize 21}$,    
A.T.~Watson$^\textrm{\scriptsize 21}$,    
M.F.~Watson$^\textrm{\scriptsize 21}$,    
G.~Watts$^\textrm{\scriptsize 145}$,    
S.~Watts$^\textrm{\scriptsize 98}$,    
B.M.~Waugh$^\textrm{\scriptsize 92}$,    
A.F.~Webb$^\textrm{\scriptsize 11}$,    
S.~Webb$^\textrm{\scriptsize 97}$,    
M.S.~Weber$^\textrm{\scriptsize 20}$,    
S.A.~Weber$^\textrm{\scriptsize 33}$,    
S.M.~Weber$^\textrm{\scriptsize 59a}$,    
J.S.~Webster$^\textrm{\scriptsize 6}$,    
A.R.~Weidberg$^\textrm{\scriptsize 131}$,    
B.~Weinert$^\textrm{\scriptsize 63}$,    
J.~Weingarten$^\textrm{\scriptsize 51}$,    
M.~Weirich$^\textrm{\scriptsize 97}$,    
C.~Weiser$^\textrm{\scriptsize 50}$,    
P.S.~Wells$^\textrm{\scriptsize 35}$,    
T.~Wenaus$^\textrm{\scriptsize 29}$,    
T.~Wengler$^\textrm{\scriptsize 35}$,    
S.~Wenig$^\textrm{\scriptsize 35}$,    
N.~Wermes$^\textrm{\scriptsize 24}$,    
M.D.~Werner$^\textrm{\scriptsize 76}$,    
P.~Werner$^\textrm{\scriptsize 35}$,    
M.~Wessels$^\textrm{\scriptsize 59a}$,    
T.D.~Weston$^\textrm{\scriptsize 20}$,    
K.~Whalen$^\textrm{\scriptsize 127}$,    
N.L.~Whallon$^\textrm{\scriptsize 145}$,    
A.M.~Wharton$^\textrm{\scriptsize 87}$,    
A.S.~White$^\textrm{\scriptsize 103}$,    
A.~White$^\textrm{\scriptsize 8}$,    
M.J.~White$^\textrm{\scriptsize 1}$,    
R.~White$^\textrm{\scriptsize 144b}$,    
D.~Whiteson$^\textrm{\scriptsize 169}$,    
B.W.~Whitmore$^\textrm{\scriptsize 87}$,    
F.J.~Wickens$^\textrm{\scriptsize 141}$,    
W.~Wiedenmann$^\textrm{\scriptsize 179}$,    
M.~Wielers$^\textrm{\scriptsize 141}$,    
C.~Wiglesworth$^\textrm{\scriptsize 39}$,    
L.A.M.~Wiik-Fuchs$^\textrm{\scriptsize 50}$,    
A.~Wildauer$^\textrm{\scriptsize 113}$,    
F.~Wilk$^\textrm{\scriptsize 98}$,    
H.G.~Wilkens$^\textrm{\scriptsize 35}$,    
H.H.~Williams$^\textrm{\scriptsize 133}$,    
S.~Williams$^\textrm{\scriptsize 31}$,    
C.~Willis$^\textrm{\scriptsize 104}$,    
S.~Willocq$^\textrm{\scriptsize 100}$,    
J.A.~Wilson$^\textrm{\scriptsize 21}$,    
I.~Wingerter-Seez$^\textrm{\scriptsize 5}$,    
E.~Winkels$^\textrm{\scriptsize 153}$,    
F.~Winklmeier$^\textrm{\scriptsize 127}$,    
O.J.~Winston$^\textrm{\scriptsize 153}$,    
B.T.~Winter$^\textrm{\scriptsize 24}$,    
M.~Wittgen$^\textrm{\scriptsize 150}$,    
M.~Wobisch$^\textrm{\scriptsize 93}$,    
A.~Wolf$^\textrm{\scriptsize 97}$,    
T.M.H.~Wolf$^\textrm{\scriptsize 118}$,    
R.~Wolff$^\textrm{\scriptsize 99}$,    
M.W.~Wolter$^\textrm{\scriptsize 82}$,    
H.~Wolters$^\textrm{\scriptsize 136a,136c}$,    
V.W.S.~Wong$^\textrm{\scriptsize 173}$,    
N.L.~Woods$^\textrm{\scriptsize 143}$,    
S.D.~Worm$^\textrm{\scriptsize 21}$,    
B.K.~Wosiek$^\textrm{\scriptsize 82}$,    
K.W.~Wo\'{z}niak$^\textrm{\scriptsize 82}$,    
K.~Wraight$^\textrm{\scriptsize 55}$,    
M.~Wu$^\textrm{\scriptsize 36}$,    
S.L.~Wu$^\textrm{\scriptsize 179}$,    
X.~Wu$^\textrm{\scriptsize 52}$,    
Y.~Wu$^\textrm{\scriptsize 58a}$,    
T.R.~Wyatt$^\textrm{\scriptsize 98}$,    
B.M.~Wynne$^\textrm{\scriptsize 48}$,    
S.~Xella$^\textrm{\scriptsize 39}$,    
Z.~Xi$^\textrm{\scriptsize 103}$,    
L.~Xia$^\textrm{\scriptsize 15b}$,    
D.~Xu$^\textrm{\scriptsize 15a}$,    
H.~Xu$^\textrm{\scriptsize 58a,f}$,    
L.~Xu$^\textrm{\scriptsize 29}$,    
T.~Xu$^\textrm{\scriptsize 142}$,    
W.~Xu$^\textrm{\scriptsize 103}$,    
B.~Yabsley$^\textrm{\scriptsize 154}$,    
S.~Yacoob$^\textrm{\scriptsize 32a}$,    
K.~Yajima$^\textrm{\scriptsize 129}$,    
D.P.~Yallup$^\textrm{\scriptsize 92}$,    
D.~Yamaguchi$^\textrm{\scriptsize 163}$,    
Y.~Yamaguchi$^\textrm{\scriptsize 163}$,    
A.~Yamamoto$^\textrm{\scriptsize 79}$,    
T.~Yamanaka$^\textrm{\scriptsize 161}$,    
F.~Yamane$^\textrm{\scriptsize 80}$,    
M.~Yamatani$^\textrm{\scriptsize 161}$,    
T.~Yamazaki$^\textrm{\scriptsize 161}$,    
Y.~Yamazaki$^\textrm{\scriptsize 80}$,    
Z.~Yan$^\textrm{\scriptsize 25}$,    
H.J.~Yang$^\textrm{\scriptsize 58c,58d}$,    
H.T.~Yang$^\textrm{\scriptsize 18}$,    
S.~Yang$^\textrm{\scriptsize 75}$,    
Y.~Yang$^\textrm{\scriptsize 161}$,    
Y.~Yang$^\textrm{\scriptsize 155}$,    
Z.~Yang$^\textrm{\scriptsize 17}$,    
W-M.~Yao$^\textrm{\scriptsize 18}$,    
Y.C.~Yap$^\textrm{\scriptsize 44}$,    
Y.~Yasu$^\textrm{\scriptsize 79}$,    
E.~Yatsenko$^\textrm{\scriptsize 5}$,    
K.H.~Yau~Wong$^\textrm{\scriptsize 24}$,    
J.~Ye$^\textrm{\scriptsize 41}$,    
S.~Ye$^\textrm{\scriptsize 29}$,    
I.~Yeletskikh$^\textrm{\scriptsize 77}$,    
E.~Yigitbasi$^\textrm{\scriptsize 25}$,    
E.~Yildirim$^\textrm{\scriptsize 97}$,    
K.~Yorita$^\textrm{\scriptsize 177}$,    
K.~Yoshihara$^\textrm{\scriptsize 133}$,    
C.J.S.~Young$^\textrm{\scriptsize 35}$,    
C.~Young$^\textrm{\scriptsize 150}$,    
J.~Yu$^\textrm{\scriptsize 8}$,    
J.~Yu$^\textrm{\scriptsize 76}$,    
X.~Yue$^\textrm{\scriptsize 59a}$,    
S.P.Y.~Yuen$^\textrm{\scriptsize 24}$,    
I.~Yusuff$^\textrm{\scriptsize 31,a}$,    
B.~Zabinski$^\textrm{\scriptsize 82}$,    
G.~Zacharis$^\textrm{\scriptsize 10}$,    
R.~Zaidan$^\textrm{\scriptsize 14}$,    
A.M.~Zaitsev$^\textrm{\scriptsize 140,ao}$,    
N.~Zakharchuk$^\textrm{\scriptsize 44}$,    
J.~Zalieckas$^\textrm{\scriptsize 17}$,    
S.~Zambito$^\textrm{\scriptsize 57}$,    
D.~Zanzi$^\textrm{\scriptsize 35}$,    
C.~Zeitnitz$^\textrm{\scriptsize 180}$,    
G.~Zemaityte$^\textrm{\scriptsize 131}$,    
J.C.~Zeng$^\textrm{\scriptsize 171}$,    
Q.~Zeng$^\textrm{\scriptsize 150}$,    
O.~Zenin$^\textrm{\scriptsize 140}$,    
D.~Zerwas$^\textrm{\scriptsize 128}$,    
M.~Zgubi\v{c}$^\textrm{\scriptsize 131}$,    
D.F.~Zhang$^\textrm{\scriptsize 58b}$,    
D.~Zhang$^\textrm{\scriptsize 103}$,    
F.~Zhang$^\textrm{\scriptsize 179}$,    
G.~Zhang$^\textrm{\scriptsize 58a,ah}$,    
H.~Zhang$^\textrm{\scriptsize 15c}$,    
J.~Zhang$^\textrm{\scriptsize 6}$,    
L.~Zhang$^\textrm{\scriptsize 50}$,    
L.~Zhang$^\textrm{\scriptsize 58a}$,    
M.~Zhang$^\textrm{\scriptsize 171}$,    
P.~Zhang$^\textrm{\scriptsize 15c}$,    
R.~Zhang$^\textrm{\scriptsize 58a,f}$,    
R.~Zhang$^\textrm{\scriptsize 24}$,    
X.~Zhang$^\textrm{\scriptsize 58b}$,    
Y.~Zhang$^\textrm{\scriptsize 15d}$,    
Z.~Zhang$^\textrm{\scriptsize 128}$,    
X.~Zhao$^\textrm{\scriptsize 41}$,    
Y.~Zhao$^\textrm{\scriptsize 58b,128,ak}$,    
Z.~Zhao$^\textrm{\scriptsize 58a}$,    
A.~Zhemchugov$^\textrm{\scriptsize 77}$,    
B.~Zhou$^\textrm{\scriptsize 103}$,    
C.~Zhou$^\textrm{\scriptsize 179}$,    
L.~Zhou$^\textrm{\scriptsize 41}$,    
M.S.~Zhou$^\textrm{\scriptsize 15d}$,    
M.~Zhou$^\textrm{\scriptsize 152}$,    
N.~Zhou$^\textrm{\scriptsize 58c}$,    
Y.~Zhou$^\textrm{\scriptsize 7}$,    
C.G.~Zhu$^\textrm{\scriptsize 58b}$,    
H.~Zhu$^\textrm{\scriptsize 15a}$,    
J.~Zhu$^\textrm{\scriptsize 103}$,    
Y.~Zhu$^\textrm{\scriptsize 58a}$,    
X.~Zhuang$^\textrm{\scriptsize 15a}$,    
K.~Zhukov$^\textrm{\scriptsize 108}$,    
V.~Zhulanov$^\textrm{\scriptsize 120b,120a}$,    
A.~Zibell$^\textrm{\scriptsize 175}$,    
D.~Zieminska$^\textrm{\scriptsize 63}$,    
N.I.~Zimine$^\textrm{\scriptsize 77}$,    
S.~Zimmermann$^\textrm{\scriptsize 50}$,    
Z.~Zinonos$^\textrm{\scriptsize 113}$,    
M.~Zinser$^\textrm{\scriptsize 97}$,    
M.~Ziolkowski$^\textrm{\scriptsize 148}$,    
G.~Zobernig$^\textrm{\scriptsize 179}$,    
A.~Zoccoli$^\textrm{\scriptsize 23b,23a}$,    
T.G.~Zorbas$^\textrm{\scriptsize 146}$,    
R.~Zou$^\textrm{\scriptsize 36}$,    
M.~Zur~Nedden$^\textrm{\scriptsize 19}$,    
L.~Zwalinski$^\textrm{\scriptsize 35}$.    
\bigskip
\\

$^{1}$Department of Physics, University of Adelaide, Adelaide; Australia.\\
$^{2}$Physics Department, SUNY Albany, Albany NY; United States of America.\\
$^{3}$Department of Physics, University of Alberta, Edmonton AB; Canada.\\
$^{4}$$^{(a)}$Department of Physics, Ankara University, Ankara;$^{(b)}$Istanbul Aydin University, Istanbul;$^{(c)}$Division of Physics, TOBB University of Economics and Technology, Ankara; Turkey.\\
$^{5}$LAPP, Universit\'e Grenoble Alpes, Universit\'e Savoie Mont Blanc, CNRS/IN2P3, Annecy; France.\\
$^{6}$High Energy Physics Division, Argonne National Laboratory, Argonne IL; United States of America.\\
$^{7}$Department of Physics, University of Arizona, Tucson AZ; United States of America.\\
$^{8}$Department of Physics, University of Texas at Arlington, Arlington TX; United States of America.\\
$^{9}$Physics Department, National and Kapodistrian University of Athens, Athens; Greece.\\
$^{10}$Physics Department, National Technical University of Athens, Zografou; Greece.\\
$^{11}$Department of Physics, University of Texas at Austin, Austin TX; United States of America.\\
$^{12}$$^{(a)}$Bahcesehir University, Faculty of Engineering and Natural Sciences, Istanbul;$^{(b)}$Istanbul Bilgi University, Faculty of Engineering and Natural Sciences, Istanbul;$^{(c)}$Department of Physics, Bogazici University, Istanbul;$^{(d)}$Department of Physics Engineering, Gaziantep University, Gaziantep; Turkey.\\
$^{13}$Institute of Physics, Azerbaijan Academy of Sciences, Baku; Azerbaijan.\\
$^{14}$Institut de F\'isica d'Altes Energies (IFAE), Barcelona Institute of Science and Technology, Barcelona; Spain.\\
$^{15}$$^{(a)}$Institute of High Energy Physics, Chinese Academy of Sciences, Beijing;$^{(b)}$Physics Department, Tsinghua University, Beijing;$^{(c)}$Department of Physics, Nanjing University, Nanjing;$^{(d)}$University of Chinese Academy of Science (UCAS), Beijing; China.\\
$^{16}$Institute of Physics, University of Belgrade, Belgrade; Serbia.\\
$^{17}$Department for Physics and Technology, University of Bergen, Bergen; Norway.\\
$^{18}$Physics Division, Lawrence Berkeley National Laboratory and University of California, Berkeley CA; United States of America.\\
$^{19}$Institut f\"{u}r Physik, Humboldt Universit\"{a}t zu Berlin, Berlin; Germany.\\
$^{20}$Albert Einstein Center for Fundamental Physics and Laboratory for High Energy Physics, University of Bern, Bern; Switzerland.\\
$^{21}$School of Physics and Astronomy, University of Birmingham, Birmingham; United Kingdom.\\
$^{22}$Centro de Investigaci\'ones, Universidad Antonio Nari\~no, Bogota; Colombia.\\
$^{23}$$^{(a)}$Dipartimento di Fisica e Astronomia, Universit\`a di Bologna, Bologna;$^{(b)}$INFN Sezione di Bologna; Italy.\\
$^{24}$Physikalisches Institut, Universit\"{a}t Bonn, Bonn; Germany.\\
$^{25}$Department of Physics, Boston University, Boston MA; United States of America.\\
$^{26}$Department of Physics, Brandeis University, Waltham MA; United States of America.\\
$^{27}$$^{(a)}$Transilvania University of Brasov, Brasov;$^{(b)}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest;$^{(c)}$Department of Physics, Alexandru Ioan Cuza University of Iasi, Iasi;$^{(d)}$National Institute for Research and Development of Isotopic and Molecular Technologies, Physics Department, Cluj-Napoca;$^{(e)}$University Politehnica Bucharest, Bucharest;$^{(f)}$West University in Timisoara, Timisoara; Romania.\\
$^{28}$$^{(a)}$Faculty of Mathematics, Physics and Informatics, Comenius University, Bratislava;$^{(b)}$Department of Subnuclear Physics, Institute of Experimental Physics of the Slovak Academy of Sciences, Kosice; Slovak Republic.\\
$^{29}$Physics Department, Brookhaven National Laboratory, Upton NY; United States of America.\\
$^{30}$Departamento de F\'isica, Universidad de Buenos Aires, Buenos Aires; Argentina.\\
$^{31}$Cavendish Laboratory, University of Cambridge, Cambridge; United Kingdom.\\
$^{32}$$^{(a)}$Department of Physics, University of Cape Town, Cape Town;$^{(b)}$Department of Mechanical Engineering Science, University of Johannesburg, Johannesburg;$^{(c)}$School of Physics, University of the Witwatersrand, Johannesburg; South Africa.\\
$^{33}$Department of Physics, Carleton University, Ottawa ON; Canada.\\
$^{34}$$^{(a)}$Facult\'e des Sciences Ain Chock, R\'eseau Universitaire de Physique des Hautes Energies - Universit\'e Hassan II, Casablanca;$^{(b)}$Centre National de l'Energie des Sciences Techniques Nucleaires (CNESTEN), Rabat;$^{(c)}$Facult\'e des Sciences Semlalia, Universit\'e Cadi Ayyad, LPHEA-Marrakech;$^{(d)}$Facult\'e des Sciences, Universit\'e Mohamed Premier and LPTPM, Oujda;$^{(e)}$Facult\'e des sciences, Universit\'e Mohammed V, Rabat; Morocco.\\
$^{35}$CERN, Geneva; Switzerland.\\
$^{36}$Enrico Fermi Institute, University of Chicago, Chicago IL; United States of America.\\
$^{37}$LPC, Universit\'e Clermont Auvergne, CNRS/IN2P3, Clermont-Ferrand; France.\\
$^{38}$Nevis Laboratory, Columbia University, Irvington NY; United States of America.\\
$^{39}$Niels Bohr Institute, University of Copenhagen, Copenhagen; Denmark.\\
$^{40}$$^{(a)}$Dipartimento di Fisica, Universit\`a della Calabria, Rende;$^{(b)}$INFN Gruppo Collegato di Cosenza, Laboratori Nazionali di Frascati; Italy.\\
$^{41}$Physics Department, Southern Methodist University, Dallas TX; United States of America.\\
$^{42}$Physics Department, University of Texas at Dallas, Richardson TX; United States of America.\\
$^{43}$$^{(a)}$Department of Physics, Stockholm University;$^{(b)}$Oskar Klein Centre, Stockholm; Sweden.\\
$^{44}$Deutsches Elektronen-Synchrotron DESY, Hamburg and Zeuthen; Germany.\\
$^{45}$Lehrstuhl f{\"u}r Experimentelle Physik IV, Technische Universit{\"a}t Dortmund, Dortmund; Germany.\\
$^{46}$Institut f\"{u}r Kern-~und Teilchenphysik, Technische Universit\"{a}t Dresden, Dresden; Germany.\\
$^{47}$Department of Physics, Duke University, Durham NC; United States of America.\\
$^{48}$SUPA - School of Physics and Astronomy, University of Edinburgh, Edinburgh; United Kingdom.\\
$^{49}$INFN e Laboratori Nazionali di Frascati, Frascati; Italy.\\
$^{50}$Physikalisches Institut, Albert-Ludwigs-Universit\"{a}t Freiburg, Freiburg; Germany.\\
$^{51}$II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"ottingen, G\"ottingen; Germany.\\
$^{52}$D\'epartement de Physique Nucl\'eaire et Corpusculaire, Universit\'e de Gen\`eve, Gen\`eve; Switzerland.\\
$^{53}$$^{(a)}$Dipartimento di Fisica, Universit\`a di Genova, Genova;$^{(b)}$INFN Sezione di Genova; Italy.\\
$^{54}$II. Physikalisches Institut, Justus-Liebig-Universit{\"a}t Giessen, Giessen; Germany.\\
$^{55}$SUPA - School of Physics and Astronomy, University of Glasgow, Glasgow; United Kingdom.\\
$^{56}$LPSC, Universit\'e Grenoble Alpes, CNRS/IN2P3, Grenoble INP, Grenoble; France.\\
$^{57}$Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge MA; United States of America.\\
$^{58}$$^{(a)}$Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei;$^{(b)}$Institute of Frontier and Interdisciplinary Science and Key Laboratory of Particle Physics and Particle Irradiation (MOE), Shandong University, Qingdao;$^{(c)}$School of Physics and Astronomy, Shanghai Jiao Tong University, KLPPAC-MoE, SKLPPC, Shanghai;$^{(d)}$Tsung-Dao Lee Institute, Shanghai; China.\\
$^{59}$$^{(a)}$Kirchhoff-Institut f\"{u}r Physik, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg;$^{(b)}$Physikalisches Institut, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg; Germany.\\
$^{60}$Faculty of Applied Information Science, Hiroshima Institute of Technology, Hiroshima; Japan.\\
$^{61}$$^{(a)}$Department of Physics, Chinese University of Hong Kong, Shatin, N.T., Hong Kong;$^{(b)}$Department of Physics, University of Hong Kong, Hong Kong;$^{(c)}$Department of Physics and Institute for Advanced Study, Hong Kong University of Science and Technology, Clear Water Bay, Kowloon, Hong Kong; China.\\
$^{62}$Department of Physics, National Tsing Hua University, Hsinchu; Taiwan.\\
$^{63}$Department of Physics, Indiana University, Bloomington IN; United States of America.\\
$^{64}$$^{(a)}$INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine;$^{(b)}$ICTP, Trieste;$^{(c)}$Dipartimento di Chimica, Fisica e Ambiente, Universit\`a di Udine, Udine; Italy.\\
$^{65}$$^{(a)}$INFN Sezione di Lecce;$^{(b)}$Dipartimento di Matematica e Fisica, Universit\`a del Salento, Lecce; Italy.\\
$^{66}$$^{(a)}$INFN Sezione di Milano;$^{(b)}$Dipartimento di Fisica, Universit\`a di Milano, Milano; Italy.\\
$^{67}$$^{(a)}$INFN Sezione di Napoli;$^{(b)}$Dipartimento di Fisica, Universit\`a di Napoli, Napoli; Italy.\\
$^{68}$$^{(a)}$INFN Sezione di Pavia;$^{(b)}$Dipartimento di Fisica, Universit\`a di Pavia, Pavia; Italy.\\
$^{69}$$^{(a)}$INFN Sezione di Pisa;$^{(b)}$Dipartimento di Fisica E. Fermi, Universit\`a di Pisa, Pisa; Italy.\\
$^{70}$$^{(a)}$INFN Sezione di Roma;$^{(b)}$Dipartimento di Fisica, Sapienza Universit\`a di Roma, Roma; Italy.\\
$^{71}$$^{(a)}$INFN Sezione di Roma Tor Vergata;$^{(b)}$Dipartimento di Fisica, Universit\`a di Roma Tor Vergata, Roma; Italy.\\
$^{72}$$^{(a)}$INFN Sezione di Roma Tre;$^{(b)}$Dipartimento di Matematica e Fisica, Universit\`a Roma Tre, Roma; Italy.\\
$^{73}$$^{(a)}$INFN-TIFPA;$^{(b)}$Universit\`a degli Studi di Trento, Trento; Italy.\\
$^{74}$Institut f\"{u}r Astro-~und Teilchenphysik, Leopold-Franzens-Universit\"{a}t, Innsbruck; Austria.\\
$^{75}$University of Iowa, Iowa City IA; United States of America.\\
$^{76}$Department of Physics and Astronomy, Iowa State University, Ames IA; United States of America.\\
$^{77}$Joint Institute for Nuclear Research, Dubna; Russia.\\
$^{78}$$^{(a)}$Departamento de Engenharia El\'etrica, Universidade Federal de Juiz de Fora (UFJF), Juiz de Fora;$^{(b)}$Universidade Federal do Rio De Janeiro COPPE/EE/IF, Rio de Janeiro;$^{(c)}$Universidade Federal de S\~ao Jo\~ao del Rei (UFSJ), S\~ao Jo\~ao del Rei;$^{(d)}$Instituto de F\'isica, Universidade de S\~ao Paulo, S\~ao Paulo; Brazil.\\
$^{79}$KEK, High Energy Accelerator Research Organization, Tsukuba; Japan.\\
$^{80}$Graduate School of Science, Kobe University, Kobe; Japan.\\
$^{81}$$^{(a)}$AGH University of Science and Technology, Faculty of Physics and Applied Computer Science, Krakow;$^{(b)}$Marian Smoluchowski Institute of Physics, Jagiellonian University, Krakow; Poland.\\
$^{82}$Institute of Nuclear Physics Polish Academy of Sciences, Krakow; Poland.\\
$^{83}$Faculty of Science, Kyoto University, Kyoto; Japan.\\
$^{84}$Kyoto University of Education, Kyoto; Japan.\\
$^{85}$Research Center for Advanced Particle Physics and Department of Physics, Kyushu University, Fukuoka ; Japan.\\
$^{86}$Instituto de F\'{i}sica La Plata, Universidad Nacional de La Plata and CONICET, La Plata; Argentina.\\
$^{87}$Physics Department, Lancaster University, Lancaster; United Kingdom.\\
$^{88}$Oliver Lodge Laboratory, University of Liverpool, Liverpool; United Kingdom.\\
$^{89}$Department of Experimental Particle Physics, Jo\v{z}ef Stefan Institute and Department of Physics, University of Ljubljana, Ljubljana; Slovenia.\\
$^{90}$School of Physics and Astronomy, Queen Mary University of London, London; United Kingdom.\\
$^{91}$Department of Physics, Royal Holloway University of London, Egham; United Kingdom.\\
$^{92}$Department of Physics and Astronomy, University College London, London; United Kingdom.\\
$^{93}$Louisiana Tech University, Ruston LA; United States of America.\\
$^{94}$Fysiska institutionen, Lunds universitet, Lund; Sweden.\\
$^{95}$Centre de Calcul de l'Institut National de Physique Nucl\'eaire et de Physique des Particules (IN2P3), Villeurbanne; France.\\
$^{96}$Departamento de F\'isica Teorica C-15 and CIAFF, Universidad Aut\'onoma de Madrid, Madrid; Spain.\\
$^{97}$Institut f\"{u}r Physik, Universit\"{a}t Mainz, Mainz; Germany.\\
$^{98}$School of Physics and Astronomy, University of Manchester, Manchester; United Kingdom.\\
$^{99}$CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille; France.\\
$^{100}$Department of Physics, University of Massachusetts, Amherst MA; United States of America.\\
$^{101}$Department of Physics, McGill University, Montreal QC; Canada.\\
$^{102}$School of Physics, University of Melbourne, Victoria; Australia.\\
$^{103}$Department of Physics, University of Michigan, Ann Arbor MI; United States of America.\\
$^{104}$Department of Physics and Astronomy, Michigan State University, East Lansing MI; United States of America.\\
$^{105}$B.I. Stepanov Institute of Physics, National Academy of Sciences of Belarus, Minsk; Belarus.\\
$^{106}$Research Institute for Nuclear Problems of Byelorussian State University, Minsk; Belarus.\\
$^{107}$Group of Particle Physics, University of Montreal, Montreal QC; Canada.\\
$^{108}$P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow; Russia.\\
$^{109}$Institute for Theoretical and Experimental Physics (ITEP), Moscow; Russia.\\
$^{110}$National Research Nuclear University MEPhI, Moscow; Russia.\\
$^{111}$D.V. Skobeltsyn Institute of Nuclear Physics, M.V. Lomonosov Moscow State University, Moscow; Russia.\\
$^{112}$Fakult\"at f\"ur Physik, Ludwig-Maximilians-Universit\"at M\"unchen, M\"unchen; Germany.\\
$^{113}$Max-Planck-Institut f\"ur Physik (Werner-Heisenberg-Institut), M\"unchen; Germany.\\
$^{114}$Nagasaki Institute of Applied Science, Nagasaki; Japan.\\
$^{115}$Graduate School of Science and Kobayashi-Maskawa Institute, Nagoya University, Nagoya; Japan.\\
$^{116}$Department of Physics and Astronomy, University of New Mexico, Albuquerque NM; United States of America.\\
$^{117}$Institute for Mathematics, Astrophysics and Particle Physics, Radboud University Nijmegen/Nikhef, Nijmegen; Netherlands.\\
$^{118}$Nikhef National Institute for Subatomic Physics and University of Amsterdam, Amsterdam; Netherlands.\\
$^{119}$Department of Physics, Northern Illinois University, DeKalb IL; United States of America.\\
$^{120}$$^{(a)}$Budker Institute of Nuclear Physics, SB RAS, Novosibirsk;$^{(b)}$Novosibirsk State University Novosibirsk; Russia.\\
$^{121}$Department of Physics, New York University, New York NY; United States of America.\\
$^{122}$Ohio State University, Columbus OH; United States of America.\\
$^{123}$Faculty of Science, Okayama University, Okayama; Japan.\\
$^{124}$Homer L. Dodge Department of Physics and Astronomy, University of Oklahoma, Norman OK; United States of America.\\
$^{125}$Department of Physics, Oklahoma State University, Stillwater OK; United States of America.\\
$^{126}$Palack\'y University, RCPTM, Joint Laboratory of Optics, Olomouc; Czech Republic.\\
$^{127}$Center for High Energy Physics, University of Oregon, Eugene OR; United States of America.\\
$^{128}$LAL, Universit\'e Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, Orsay; France.\\
$^{129}$Graduate School of Science, Osaka University, Osaka; Japan.\\
$^{130}$Department of Physics, University of Oslo, Oslo; Norway.\\
$^{131}$Department of Physics, Oxford University, Oxford; United Kingdom.\\
$^{132}$LPNHE, Sorbonne Universit\'e, Paris Diderot Sorbonne Paris Cit\'e, CNRS/IN2P3, Paris; France.\\
$^{133}$Department of Physics, University of Pennsylvania, Philadelphia PA; United States of America.\\
$^{134}$Konstantinov Nuclear Physics Institute of National Research Centre "Kurchatov Institute", PNPI, St. Petersburg; Russia.\\
$^{135}$Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh PA; United States of America.\\
$^{136}$$^{(a)}$Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas - LIP;$^{(b)}$Departamento de F\'isica, Faculdade de Ci\^{e}ncias, Universidade de Lisboa, Lisboa;$^{(c)}$Departamento de F\'isica, Universidade de Coimbra, Coimbra;$^{(d)}$Centro de F\'isica Nuclear da Universidade de Lisboa, Lisboa;$^{(e)}$Departamento de F\'isica, Universidade do Minho, Braga;$^{(f)}$Departamento de F\'isica Teorica y del Cosmos, Universidad de Granada, Granada (Spain);$^{(g)}$Dep F\'isica and CEFITEC of Faculdade de Ci\^{e}ncias e Tecnologia, Universidade Nova de Lisboa, Caparica; Portugal.\\
$^{137}$Institute of Physics, Academy of Sciences of the Czech Republic, Prague; Czech Republic.\\
$^{138}$Czech Technical University in Prague, Prague; Czech Republic.\\
$^{139}$Charles University, Faculty of Mathematics and Physics, Prague; Czech Republic.\\
$^{140}$State Research Center Institute for High Energy Physics, NRC KI, Protvino; Russia.\\
$^{141}$Particle Physics Department, Rutherford Appleton Laboratory, Didcot; United Kingdom.\\
$^{142}$IRFU, CEA, Universit\'e Paris-Saclay, Gif-sur-Yvette; France.\\
$^{143}$Santa Cruz Institute for Particle Physics, University of California Santa Cruz, Santa Cruz CA; United States of America.\\
$^{144}$$^{(a)}$Departamento de F\'isica, Pontificia Universidad Cat\'olica de Chile, Santiago;$^{(b)}$Departamento de F\'isica, Universidad T\'ecnica Federico Santa Mar\'ia, Valpara\'iso; Chile.\\
$^{145}$Department of Physics, University of Washington, Seattle WA; United States of America.\\
$^{146}$Department of Physics and Astronomy, University of Sheffield, Sheffield; United Kingdom.\\
$^{147}$Department of Physics, Shinshu University, Nagano; Japan.\\
$^{148}$Department Physik, Universit\"{a}t Siegen, Siegen; Germany.\\
$^{149}$Department of Physics, Simon Fraser University, Burnaby BC; Canada.\\
$^{150}$SLAC National Accelerator Laboratory, Stanford CA; United States of America.\\
$^{151}$Physics Department, Royal Institute of Technology, Stockholm; Sweden.\\
$^{152}$Departments of Physics and Astronomy, Stony Brook University, Stony Brook NY; United States of America.\\
$^{153}$Department of Physics and Astronomy, University of Sussex, Brighton; United Kingdom.\\
$^{154}$School of Physics, University of Sydney, Sydney; Australia.\\
$^{155}$Institute of Physics, Academia Sinica, Taipei; Taiwan.\\
$^{156}$Academia Sinica Grid Computing, Institute of Physics, Academia Sinica, Taipei; Taiwan.\\
$^{157}$$^{(a)}$E. Andronikashvili Institute of Physics, Iv. Javakhishvili Tbilisi State University, Tbilisi;$^{(b)}$High Energy Physics Institute, Tbilisi State University, Tbilisi; Georgia.\\
$^{158}$Department of Physics, Technion, Israel Institute of Technology, Haifa; Israel.\\
$^{159}$Raymond and Beverly Sackler School of Physics and Astronomy, Tel Aviv University, Tel Aviv; Israel.\\
$^{160}$Department of Physics, Aristotle University of Thessaloniki, Thessaloniki; Greece.\\
$^{161}$International Center for Elementary Particle Physics and Department of Physics, University of Tokyo, Tokyo; Japan.\\
$^{162}$Graduate School of Science and Technology, Tokyo Metropolitan University, Tokyo; Japan.\\
$^{163}$Department of Physics, Tokyo Institute of Technology, Tokyo; Japan.\\
$^{164}$Tomsk State University, Tomsk; Russia.\\
$^{165}$Department of Physics, University of Toronto, Toronto ON; Canada.\\
$^{166}$$^{(a)}$TRIUMF, Vancouver BC;$^{(b)}$Department of Physics and Astronomy, York University, Toronto ON; Canada.\\
$^{167}$Division of Physics and Tomonaga Center for the History of the Universe, Faculty of Pure and Applied Sciences, University of Tsukuba, Tsukuba; Japan.\\
$^{168}$Department of Physics and Astronomy, Tufts University, Medford MA; United States of America.\\
$^{169}$Department of Physics and Astronomy, University of California Irvine, Irvine CA; United States of America.\\
$^{170}$Department of Physics and Astronomy, University of Uppsala, Uppsala; Sweden.\\
$^{171}$Department of Physics, University of Illinois, Urbana IL; United States of America.\\
$^{172}$Instituto de F\'isica Corpuscular (IFIC), Centro Mixto Universidad de Valencia - CSIC, Valencia; Spain.\\
$^{173}$Department of Physics, University of British Columbia, Vancouver BC; Canada.\\
$^{174}$Department of Physics and Astronomy, University of Victoria, Victoria BC; Canada.\\
$^{175}$Fakult\"at f\"ur Physik und Astronomie, Julius-Maximilians-Universit\"at W\"urzburg, W\"urzburg; Germany.\\
$^{176}$Department of Physics, University of Warwick, Coventry; United Kingdom.\\
$^{177}$Waseda University, Tokyo; Japan.\\
$^{178}$Department of Particle Physics, Weizmann Institute of Science, Rehovot; Israel.\\
$^{179}$Department of Physics, University of Wisconsin, Madison WI; United States of America.\\
$^{180}$Fakult{\"a}t f{\"u}r Mathematik und Naturwissenschaften, Fachgruppe Physik, Bergische Universit\"{a}t Wuppertal, Wuppertal; Germany.\\
$^{181}$Department of Physics, Yale University, New Haven CT; United States of America.\\
$^{182}$Yerevan Physics Institute, Yerevan; Armenia.\\

$^{a}$ Also at  Department of Physics, University of Malaya, Kuala Lumpur; Malaysia.\\
$^{b}$ Also at Borough of Manhattan Community College, City University of New York, NY; United States of America.\\
$^{c}$ Also at California State University, East Bay; United States of America.\\
$^{d}$ Also at Centre for High Performance Computing, CSIR Campus, Rosebank, Cape Town; South Africa.\\
$^{e}$ Also at CERN, Geneva; Switzerland.\\
$^{f}$ Also at CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3, Marseille; France.\\
$^{g}$ Also at D\'epartement de Physique Nucl\'eaire et Corpusculaire, Universit\'e de Gen\`eve, Gen\`eve; Switzerland.\\
$^{h}$ Also at Departament de Fisica de la Universitat Autonoma de Barcelona, Barcelona; Spain.\\
$^{i}$ Also at Departamento de F\'isica Teorica y del Cosmos, Universidad de Granada, Granada (Spain); Spain.\\
$^{j}$ Also at Department of Applied Physics and Astronomy, University of Sharjah, Sharjah; United Arab Emirates.\\
$^{k}$ Also at Department of Financial and Management Engineering, University of the Aegean, Chios; Greece.\\
$^{l}$ Also at Department of Physics and Astronomy, University of Louisville, Louisville, KY; United States of America.\\
$^{m}$ Also at Department of Physics and Astronomy, University of Sheffield, Sheffield; United Kingdom.\\
$^{n}$ Also at Department of Physics, California State University, Fresno CA; United States of America.\\
$^{o}$ Also at Department of Physics, California State University, Sacramento CA; United States of America.\\
$^{p}$ Also at Department of Physics, King's College London, London; United Kingdom.\\
$^{q}$ Also at Department of Physics, Nanjing University, Nanjing; China.\\
$^{r}$ Also at Department of Physics, St. Petersburg State Polytechnical University, St. Petersburg; Russia.\\
$^{s}$ Also at Department of Physics, Stanford University; United States of America.\\
$^{t}$ Also at Department of Physics, University of Fribourg, Fribourg; Switzerland.\\
$^{u}$ Also at Department of Physics, University of Michigan, Ann Arbor MI; United States of America.\\
$^{v}$ Also at Dipartimento di Fisica E. Fermi, Universit\`a di Pisa, Pisa; Italy.\\
$^{w}$ Also at Giresun University, Faculty of Engineering, Giresun; Turkey.\\
$^{x}$ Also at Graduate School of Science, Osaka University, Osaka; Japan.\\
$^{y}$ Also at Hellenic Open University, Patras; Greece.\\
$^{z}$ Also at Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest; Romania.\\
$^{aa}$ Also at II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"ottingen, G\"ottingen; Germany.\\
$^{ab}$ Also at Institucio Catalana de Recerca i Estudis Avancats, ICREA, Barcelona; Spain.\\
$^{ac}$ Also at Institut de F\'isica d'Altes Energies (IFAE), Barcelona Institute of Science and Technology, Barcelona; Spain.\\
$^{ad}$ Also at Institut f\"{u}r Experimentalphysik, Universit\"{a}t Hamburg, Hamburg; Germany.\\
$^{ae}$ Also at Institute for Mathematics, Astrophysics and Particle Physics, Radboud University Nijmegen/Nikhef, Nijmegen; Netherlands.\\
$^{af}$ Also at Institute for Particle and Nuclear Physics, Wigner Research Centre for Physics, Budapest; Hungary.\\
$^{ag}$ Also at Institute of Particle Physics (IPP); Canada.\\
$^{ah}$ Also at Institute of Physics, Academia Sinica, Taipei; Taiwan.\\
$^{ai}$ Also at Institute of Physics, Azerbaijan Academy of Sciences, Baku; Azerbaijan.\\
$^{aj}$ Also at Institute of Theoretical Physics, Ilia State University, Tbilisi; Georgia.\\
$^{ak}$ Also at LAL, Universit\'e Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, Orsay; France.\\
$^{al}$ Also at Louisiana Tech University, Ruston LA; United States of America.\\
$^{am}$ Also at LPNHE, Sorbonne Universit\'e, Paris Diderot Sorbonne Paris Cit\'e, CNRS/IN2P3, Paris; France.\\
$^{an}$ Also at Manhattan College, New York NY; United States of America.\\
$^{ao}$ Also at Moscow Institute of Physics and Technology State University, Dolgoprudny; Russia.\\
$^{ap}$ Also at National Research Nuclear University MEPhI, Moscow; Russia.\\
$^{aq}$ Also at Near East University, Nicosia, North Cyprus, Mersin; Turkey.\\
$^{ar}$ Also at Ochadai Academic Production, Ochanomizu University, Tokyo; Japan.\\
$^{as}$ Also at Physikalisches Institut, Albert-Ludwigs-Universit\"{a}t Freiburg, Freiburg; Germany.\\
$^{at}$ Also at School of Physics, Sun Yat-sen University, Guangzhou; China.\\
$^{au}$ Also at The City College of New York, New York NY; United States of America.\\
$^{av}$ Also at The Collaborative Innovation Center of Quantum Matter (CICQM), Beijing; China.\\
$^{aw}$ Also at Tomsk State University, Tomsk, and Moscow Institute of Physics and Technology State University, Dolgoprudny; Russia.\\
$^{ax}$ Also at TRIUMF, Vancouver BC; Canada.\\
$^{ay}$ Also at Universita di Napoli Parthenope, Napoli; Italy.\\
$^{*}$ Deceased

\end{flushleft}

% Created with Glance <Atlas.Glance@cern.ch>

